Multi-Rate Planning and Control of Uncertain Nonlinear Systems: Model Predictive Control and Control Lyapunov Functions

Modern control systems must operate in increasingly complex environments subject to safety constraints and input limits, and are often implemented in a hierarchical fashion with different controllers running at multiple time scales. Yet traditional constructive methods for nonlinear controller synthesis typically "flatten" this hierarchy, focusing on a single time scale, and thereby limited the ability to make rigorous guarantees on constraint satisfaction that hold for the entire system. In this work we seek to address the stabilization of constrained nonlinear systems through a \textit{multi-rate} control architecture. This is accomplished by iteratively planning continuous reference trajectories for a nonlinear system using a linearized model and Model Predictive Control (MPC), and tracking said trajectories using the full-order nonlinear model and Control Lyapunov Functions (CLFs). Connecting these two levels of control design in a way that ensures constraint satisfaction is achieved through the use of \textit{B\'{e}zier curves}, which enable planning continuous trajectories respecting constraints by planning a sequence of discrete points. Our framework is encoded via convex optimization problems which may be efficiently solved, as demonstrated in simulation.

==> 1_Introduction.tex <==
\section{Introduction}

% 1-Motivation

% The study and design of nonlinear control systems has long been framed through the lens of stabilization, often in an optimal sense. However in most modern engineering settings, the task of stabilization is complicated by the need to meet safety-critical constraints on the system's state while respecting input limitations. Thus it is necessary to develop efficient control synthesis techniques that provide rigorous guarantees of stability, even in the presence of such constraints.

The study and design of nonlinear control systems has long been framed through the lens of stabilization, often in an optimal sense. This is coupled with the fact that one typically considers a single model, implicitly representing a single time scale. However in most modern engineering settings, especially in the context of autonomous and robotic systems, the task of stabilization is complicated by the need to meet safety-critical constraints on the system's state while respecting input limitations. To address this need, implementations often utilize a hierarchical approach that spans multiple time-scales, from the planning layer---which typically leverages discrete-time models---to the real-time controller layer which often considers continuous-time representations. Thus it is necessary to develop efficient control synthesis techniques that provide rigorous guarantees of stability, even in the presence of such constraints, and across multiple time scales. 

%
%
\par
% 2-Low-level control design
At the level of real-time control design, a rich catalog of methods have been developed for stabilizing nonlinear systems in the presence of unknown disturbances by utilizing underlying structural properties of the system \cite{isidori1995nonlinear, kokotovic2001constructive, khalil2002nonlinear, sepulchre2012constructive}. In particular, the tools of Control Lyapunov Functions (CLFs) \cite{artstein1983stabilization, sontag1989universal} and Input-to-State Stability \cite{Sontag1989smooth} have enabled the joint synthesis of stabilizing controllers and Lyapunov certificates of stability in the presence of disturbances, including through convex optimization \cite{freeman1996robust, ames2013towards, kolathaya2018iss}. These methods for stabilization yield highly structured controllers, and modifying these designs to accommodate state and input constraints may destroy the stability properties guaranteed by the controller. This issue is often circumnavigated theoretically by limiting the domain on which stability is guaranteed, effectively ignoring constraints. 

%
%
\par
% 3-Model predictive control
In contrast, Model Predictive Control (MPC) provides an effective method for addressing constraints \cite{allgower2004nonlinear,allgower2012nonlinear, borrelli2017predictive}. This is achieved by directly incorporating constraints a into controller that iteratively plans a finite sequence of states and inputs that are related through a discrete model of the system dynamics and satisfy required constraints. Although MPC has been successfully demonstrated in several challenging control settings \cite{dicarlo2018dynamic, sleiman2021unified,falcone2007predictive, hrovat2012development, lima2018experimental, bengea2012model, serale2018model, maddalena2020data, rosolia2019learning, liniger2015optimization, hewing2019cautious}, it is rarely implemented in real-time using the full-order continuous time nonlinear dynamics while accounting for unknown disturbances acting on the system. Thus, MPC implementation for nonlinear systems usually lack strong theoretical guarantees on constraint satisfaction in the presence of disturbances. This is because (i) it is typically difficult to find a closed-form expression for the exact temporal discretization of continuous time nonlinear dynamics \cite{nevsic1999sufficient}, (ii) approximating the exact discretization through numerical integration typically yields a non-convex relationship between planned states and inputs, and (iii) exactly propagating disturbances through high-dimensional nonlinear dynamics is often computationally intractable~\cite{bansal2017hamilton}. These challenges often preclude achieving the computational efficiency needed for real-time implementation.

% to the real-time control methods that utilize the full nonlinear dynamics

% ---albeit typically implemented at slower time scales with linear (or linearized) discrete time dynamics. 
% Despite the limitations on control frequency and linearity of the dynamics, this approach

% In contrast to the real-time control methods that utilize the full nonlinear dynamics, Model Predictive Control (MPC) has provided an effective method for incorporating constraints by directly incorporating them into controller design \cite{allgower2004nonlinear,allgower2012nonlinear, borrelli2017predictive}---albeit typically implemented at slower time scales with linear (or linearized) discrete time dynamics. 
% Despite the limitations on control frequency and linearity of the dynamics, this approach has been successfully demonstrated in several challenging control settings \cite{dicarlo2018dynamic, sleiman2021unified,falcone2007predictive, hrovat2012development, lima2018experimental, bengea2012model, serale2018model, maddalena2020data, rosolia2019learning, liniger2015optimization, hewing2019cautious}. Model Predictive Control accomplishes this by iteratively planning a finite sequence of states and inputs that are related through a discrete model of the system dynamics and satisfy required constraints. In practice it can be difficult to find a closed-form expression for the exact discretization of continuous time nonlinear dynamics \cite{nevsic1999sufficient}, and approximating the exact discretization through numerical integration typically yields a non-convex relationship between the planned states and inputs. This often presents difficulties in achieving computationally efficient online planning with guarantees of a solution. 

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/Fig1_v3.pdf}
    \caption{Overview of Multi-Rate Architecture, with discrete planning producing reference trajectories at a mid-level and continuous controllers producing invariant sets at a low-level.}
    \vspace{-5mm}
    \label{fig:my_label}
\end{figure}

%
%
\par
% 4-Approximating and Tubes.  

The difficulty in realizing MPC based controllers at a fast enough rate to allow for real-time implementation 
is often resolved by using an approximate model of the system dynamics that is amenable to efficient planning, typically through reduced-order models or via linearization and temporal discretization of the continuous time nonlinear system dynamics \cite{borrelli2017predictive, rosolia2019learning, liniger2015optimization,carvalho2013predictive, hewing2019cautious}. The use of such approximations creates a gap between the system which is being planned for and the actual evolution of the nonlinear system, requiring an additional measure of robustness to ensure constraint satisfaction. This robustness is often achieved by tightening the constraint sets by the maximum deviation between the approximate model and the continuous time nonlinear system dynamics \cite{gao2014tube, kogel2015discrete, yu2013tube, singh2017robust,kohler2020computationally,herbert2017fastrack, singh2018robust,yin2020optimization}. Approximating worse-case deviations is typically done using properties of the dynamics which may be difficult to compute, such as Lipschitz constants for which over-approximations yield conservativeness, or by solving computationally intensive optimization programs. More recently, hierarchical control frameworks have been proposed that plan with an approximate model, but directly address nonlinear dynamics with a low-level controller \cite{rosolia2020unified, rosolia2021multirate}. However, this work does not address if the low-level controller respects state and input constraints as it follows the planned trajectory under disturbances.



% Furthermore, errors sets should account for inaccuracies introduced by the temporal discretization of the continuous time dynamics, which is needed as the MPC problem plans a sequence of states for a discrete time system\footnote{Notice that even when the MPC problem is introduced using a continuous time formulation, the solution to such problem is computed by discretizing the system dynamics}. Notice that the planned sequence of states is guaranteed to satisfy state constraints, but oftentimes no safety guarantees are given about the evolution of the continuous time dynamics.

%
%
\par
In this work we propose a novel multi-rate control architecture that unifies the planning capabilities of Model Predictive Control with the ability to directly address nonlinear dynamics provided by Control Lyapunov Functions. The fundamental tool that allows our framework to explicitly address the relationship between a planner and controller operating at different time scales are \textit{B\'{e}zier curves} \cite{kamermans2020primer, farin2002curves}. By directly planning over the \textit{control points} that parameterize B\'{e}zier curves, we capitalize on a critical convex hull property to ensure that state and input constraints are met by the nonlinear system evolving under an optimization-based CLF controller. While B\'{e}zier curves have been used in motion planning, or to verify constraint satisfaction after solving an MPC problem \cite{muehlebach2017implementation}, this is to the best of our knowledge the first result directly planning over B\'{e}zier control points in an MPC formulation, and using the resulting continuous trajectories to ensure constraint satisfaction for a nonlinear system with disturbances.

% We begin by reviewing nonlinear dynamics, and how structural properties can be used to synthesize Control Lyapunov Functions and optimization-based controllers for stabilizing a class of \textit{dynamically admissible} reference trajectories. These controllers yield a description of how accurately a reference trajectory is tracked in the presence of disturbances that is amenable to being incorporated into planning. Next, we provide a review of B\'{e}zier curves, and show how they may be used to synthesize reference trajectories for the disturbed nonlinear system such that state constraints are satisfied. We further use the properties of B\'{e}zier curves in conjunction with the structure of the low-level controller to formulate constraints on B\'{e}zier control points that ensure the low-level controller satisfies input constraints. Next, we integrate the preceding constructions into a Model Predictive Control formulation that plans over B\'{e}zier control points and synthesizes continuous reference trajectories using a reduced-order model while ensuring recursive feasibility. We conclude with simulation results and a discussion of future work. Note that proofs of our results are provided in the extended version \cite{csomay2022multirate_extended}.


We begin in Section \ref{sec:lowlevel} by reviewing nonlinear dynamics, and how structural properties can be used to synthesize CLFs and optimization-based controllers for stabilizing a class of \textit{dynamically admissible} reference trajectories. These controllers yield a description of how accurately a reference trajectory is tracked in the presence of disturbances that is amenable to being incorporated into planning. Next, in Section \ref{sec:bezier} we provide a review of B\'{e}zier curves, and show how they may be used to synthesize reference trajectories for the disturbed nonlinear system such that state constraints are satisfied.  Section \ref{sec:input} uses the properties of B\'{e}zier curves in conjunction with the structure of the low-level controller to formulate constraints on B\'{e}zier control points that ensure the low-level controller satisfies input constraints. In Section \ref{sec:multirate} we integrate the preceding constructions into an MPC formulation that plans over B\'{e}zier control points and synthesizes continuous reference trajectories using a locally linearized and discretized model while ensuring recursive feasibility. We conclude in Section \ref{sec:sim} with simulation results.
% Note that proofs of our results are provided in the extended version \cite{csomay2022multirate_extended}.
Space constraints due to the multi-faceted constructions prevent the inclusion of proofs; these can be found in the extended version \cite{csomay2022multirate_extended}.







% In real world applications, achieving stability while satisfying state and input constraints is paramount. Although standard control theoretic techniques provide a powerful set of tools for stabilizing nonlinear systems, they often fail to take state and input constraints into account. While existing methods have sought to directly modify some element of the feedback linearization and Control Lyapunov Function control paradigm, we will instead place the burden of constraint satisfaction on the process of generating reference trajectories. Model predictive control has had a long and fruitful history of planning trajectories or feedback policies while satisfying such constraints; however, this is often done assuming that the control input can only be modified at the frequency which the MPC is running. In this work, we explore the ability of multi-rate controllers, i.e. controllers running at different frequencies, to stabilise mechanical systems while satisfying state and input constraints int he face of disturbances.

% Our proposed approach seeks to utilize the advantages of both nonlinear control tools and MPC to provably achieve stabilization and constraint satisfaction for the nonlinear system \eqref{eqn:openloop_state}. We will accomplish this goal by viewing our control system through a \textit{multi-rate} paradigm. In particular MPC will periodically synthesize continuous reference signals $\mb{x}_d:\R_{\geq 0}\to\R^n$ which are to be tracked using a low-level nonlinear controller $k:\R^n\to\R$ (in continuous time). Moreover, the tracking performance and input requirements of the low-level tracking controller under disturbances will be directly incorporated into the MPC program, ensuring that state and inputs are respected by the tracking controller.






==> 2_LowLevelControllerDesign.tex <==
\section{Low-Level Controller Design}
\label{sec:lowlevel}
In this section we review nonlinear dynamical systems and discuss the design of nonlinear feedback controllers that provide a measure of disturbance rejection. Importantly, these controllers will yield a quantitative description of reference trajectory tracking that is amenable to being directly incorporated into the synthesis of the reference trajectory itself.

%%%%%%%%%%%%%%%% Used to be methodology %%%%%%%%%%%%%%%%%%%%%%%%%%
Consider the nonlinear control-affine system:
% \begin{equation}
%     \label{eqn:openloop_state}
%     \dot{\mb{x}} = \underbrace{\begin{bmatrix} x_2 \\ \vdots \\ x_n \\ f(\mb{x}) \end{bmatrix}}_{ \mb{f}(\mb{x})}+\underbrace{\begin{bmatrix} 0 \\ \vdots \\ 0 \\ g(\mb{x})\end{bmatrix}}_{\mb{g}(\mb{x})}u + \underbrace{\begin{bmatrix} 0 \\ \vdots \\ 0 \\ w(t)\end{bmatrix}}_{\mb{w}(t)},
% \end{equation}
\begin{equation}
    \label{eqn:openloop_state}
    \dot{\mb{x}} = \underbrace{\begin{bmatrix} \mb 0&\mb I\\0&\mb{0}^\top\end{bmatrix}\x+\begin{bmatrix}\mb 0\\ f(\mb{x}) \end{bmatrix}}_{ \mb{f}(\mb{x})}+\underbrace{\begin{bmatrix} \mb 0\\ g(\mb{x})\end{bmatrix}}_{\mb{g}(\mb{x})}u + \mb{w}(t),
\end{equation}
with state $\mb{x}\in\R^n$, input $u\in\R$, piecewise continuous\footnote{This definition is taken as in \cite{khalil2002nonlinear}, with piecewise continuity requiring the existence of one-sided limits at points of discontinuity.} disturbance signal $\mb{w}:\R_{\geq 0}\to\R^n$, and functions $f:\R^n\to\R$ and $g:\R^n\to\R$, assumed to be continuously differentiable on $\R^n$. Furthermore, we make the following assumption:
\begin{assumption}
The function $f$ satisfies $f(\mb{0}) = 0$ and the function $g$ satisfies $g(\state)\ne0$ for all $\x\in\R^n$.
\end{assumption}
\noindent The first assumption takes the origin to be an unforced equilibrium point of the undisturbed system. The second assumption amounts to the system \eqref{eqn:openloop_state} possessing a relative degree \cite{isidori1995nonlinear}. We note that while we consider a single-input, single-output system, this is purely to simplify the presentation of our contributions, and the subsequent developments may be easily extended to the multiple-input, multiple-output setting under an equivalent assumption of a vector relative degree.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Let $\underline{t},\overline{t}\in\R_{\geq 0}$ with $\underline{t}<\overline{t}$, and let $k:\R^n\times\tintc\to\R$ be a feedback controller that is locally Lipschitz continuous with respect to its first argument\footnote{This definition is taken as in \cite{khalil2002nonlinear}, with local Lipschitz continuity holding with a Lipschitz constant that is uniform in the function's second argument.} and piecewise continuous with respect to its second argument on $\R^n\times\tintc$. This controller yields the closed-loop system:
\begin{equation}
    \label{eqn:closedloop_state}
    \dot{\mb{x}} = \mb{f}(\mb{x})+\mb{g}(\mb{x})k(\mb{x},t)+\mb{w}(t).
\end{equation}
As the functions $\mb{f}$, $\mb{g}$, and $k$ are locally Lipschitz continuous with respect to $\mb{x}$ and $k$ is piecewise continuous with respect to $t$, for any initial condition $\mb{x}_0 \in \R^n$ and any piecewise continuous disturbance $\mb{w}:\R_{\geq 0}\to\R^n$, there exists an interval $I(\underline{t},\mb{x}_0,\mb{w})\triangleq[\underline{t},\underline{t}+\delta(\mb{x}_0,\mb{w}))$ with $ \delta(\mb{x}_0,\mb{w})\in\R_{>0}$ such that the system \eqref{eqn:closedloop_state} has a unique piecewise continuously differentiable\footnote{Piecewise continuous differentiability is taken to mean a continuous function with a derivative defined on the open intervals of a finite partition with one-sided limits.} solution $\bs{\varphi}:I(\underline{t},\mb{x}_0,\mb{w})\to\R^n$ satisfying:
\begin{align}
    \dot{\bs{\varphi}}(t) & = \mb{f}(\bs{\varphi}(t)) + \mb{g}(\bs{\varphi}(t))k(\bs{\varphi}(t),t)+\mb{w}(t), \label{eqn:soldiff_state}\\
    \bs{\varphi}(\underline{t}) & = \mb{x}_0, \label{eqn:solic_state}
\end{align}
for almost all $t\in I(\underline{t},\mb{x}_0,\mb{w})$ \cite{khalil2002nonlinear}. 

With a view towards controller design, the system \eqref{eqn:openloop_state} may also be used to define a class of reference trajectories:
\begin{definition}[\textit{Dynamically Admissible Trajectory}]
A piecewise continuously differentiable function $\x_d:[\underline{t},\overline{t}]\to\R^n$ is a \textit{dynamically admissible trajectory} for the system \eqref{eqn:openloop_state} if there is a piecewise continuous function $u_d:[\underline{t},\overline{t}]\to\R$ such that:
\begin{equation}
    \label{eqn:dynadmistraj}
    \dot{\x}_d(t) = \f(\x_d(t))+\g(\x_d(t))u_d(t),
\end{equation}
for almost all $t\in[\underline{t},\overline{t}]$.
\end{definition}
%
Given a dynamically admissible trajectory $\mb{x}_d:[\underline{t},\overline{t}]\to\R^n$ for \eqref{eqn:openloop_state}, let us denote:
% \begin{equation}
%     \dot{\mb{x}}_d(t) = \begin{bmatrix} \dot{x}_{d}^1(t) & \cdots & \dot{x}_{d}^n(t) \end{bmatrix}^\top,
% \end{equation}
$
    \dot{\mb{x}}_d(t) = \begin{bmatrix} \dot{x}_{d}^1(t) & \cdots & \dot{x}_{d}^n(t) \end{bmatrix}^\top,
$
and define a error function $\mb{e}_{\mb{x}_d}:\R^n\times\tintc\to\R^n$: 
\begin{equation}
    \label{eqn:errorfunc}
    \mb{e}_{\mb{x}_d}(\mb{x},t) = \mb{x}-\mb{x}_d(t),
\end{equation}
and its derivative $\dot{\mb{e}}_{\mb{x}_d}:\R^n\times\tintc\times\R\to\R^n$ as:
\begin{align}
    \label{eqn:errorderivfunc}
    \dot{\mb{e}}_{\mb{x}_d}(\mb{x},t,u) = &~\mb{f}(\mb{x})+\mb{g}(\mb{x})u + \mb{w}(t)-\dot{\mb{x}}_d(t).
\end{align}
Denoting:
\begin{equation}
\label{eqn:calFxd}
    \mathcal{F}_{\mb{x}_d}(\mb{x},t) = f(\mb{x})-\dot{x}_d^n(t),
\end{equation}
the structure of the system \eqref{eqn:openloop_state} implies that:
\begin{align}
\label{eqn:errordotdecomp}
    \dot{\mb{e}}_{\mb{x}_d}(\mb{\x},t,u) = & \overbrace{\begin{bmatrix}\mb{0} & \mb{I} \\ 0 & \mb{0}^\top  \end{bmatrix}\mb{e}_{\mb{x}_d}(\mb{x},t)  + \begin{bmatrix} \mb{0} \\ \mathcal{F}_{\mb{x}_d}(\mb{x},t)\end{bmatrix}}^{\mb{f}_{\mb{x}_d}(\mb{x},t)} \\ & \hspace{27.8mm}+ \mb{g}(\mb{x})u + \mb{w}(t). \nonumber
\end{align}
This structure in conjunction with the assumption that $g(\mb{x})\neq 0$ for any $\mb{x}\in\R^n$
enables a controller $k^{\textrm{fbl}}_{{\mb{x}_d}}:\R^n\times\tintc\to\R$:
\begin{equation}
\label{eqn:FBL_CL_gain}
    k^{\rm fbl}_{\mb{x}_d}(\mb{x},t) = g(\mb{x})^{-1}\left(-\mathcal{F}_{\mb{x}_d}(\mb{x},t)-\mb{K}^\top\mb{e}_{\mb{x}_d}(\mb{x},t)\right),
\end{equation}
where $\mb{K}\in\R^{n}$ is selected to yield the relationship:
\begin{equation}
 \dot{\mb{e}}_{\mb{x}_d}(\mb{x},t,k_{\rm fbl}(\mb{x},t)) =  {\mb{F}}\mb{e}_{\mb{x}_d}(\mb{x},t) + \mb{w}(t), \label{eqn:errordotcloop}
\end{equation}
with $\mb{F}\in\R^{n\times n}$ a Hurwitz matrix. For any $\mb{Q}\in\mathbb{S}^n_{\succ 0}$ (symmetric positive definite matrices) there exists a unique $\mb{P}\in\mathbb{S}^n_{\succ 0}$ solving the Continuous Time Lyapunov Equation:
\begin{equation}
    \mb{F}^\top\mb{P}+\mb{PF} = -\mb{Q}.
\end{equation}
For a particular $\mb{Q}$, the corresponding solution $\mb{P}$ may be used to define the following function $V_{\mb{x}_d}:\R^n\times\tintc\to\R_{\geq 0}$:
\begin{equation}
\label{eqn:lyap}
    V_{\mb{x}_d}(\mb{x},t) = \mb{e}_{\mb{x}_d}(\mb{x},t)^\top\mb{P}\mb{e}_{\mb{x}_d}(\mb{x},t).
\end{equation}
Denoting $\grad V_{\mb{x}_d}(\mb{x},t) = 2\mb{e}_{\mb{x}_d}(\mb{x},t)^\top\mb{P}$, we have that:
\begingroup\makeatletter\def\f@size{9}\check@mathfonts
\begin{align}
   &\lambda_{\textrm{min}}(\mb{P})\Vert\mb{e}_{\mb{x}_d}(\mb{x},t)\Vert_2^2 \leq  V_{\mb{x}_d}(\mb{x},t)   \leq  ~\lambda_{\textrm{max}}(\mb{P})\Vert\mb{e}_{\mb{x}_d}(\mb{x},t)\Vert_2^2, \label{eqn:lyapbounds} \\ 
&\grad V_{\mb{x}_d}(\mb{x},t)(\mb{f}_{\mb{x}_d}(\mb{x},t)+\mb{g}(\mb{x})k_{\mb{x}_d}^{\rm fbl}(\mb{x},t)) \label{eqn:lyapdecay} \\ & \qquad\qquad\qquad\qquad\qquad\qquad \leq   -\lambda_{\rm min}(\mb{Q})\Vert\mb{e}_{\mb{x}_d}(\mb{x},t)\Vert_2^2, \nonumber
\end{align}
\endgroup
for all $\mb{x}\in\R^n$ and $t\in\tintc$. Let $\gamma = 4\lambda_{\max}(\mb{P})^3/\lambda_{\rm min}(\mb{Q})^2$ and for a given disturbance signal $\mb{w}:\R_{\geq 0}\to\R^n$ define $\Vert\mb{w}\Vert_\infty = \sup_{t\geq 0}\Vert\mb{w}(t)\Vert_2$. The preceding construction yields the following result:
\begin{lemma}
\label{lem:lowleveliss}
Let $\overline{w}\in\R_{\geq 0}$, and for $t\in\tintc$ define the set:
    \begin{equation}
    \label{eqn:robustInvariant}
        \RobustInvariant_{\mb{x}_d}(t, \overline{w}) = \{\mb{x}\in\R^n ~|~ V_{\mb{x}_d}(\mb{x},t) \leq \gamma\overline{w}^2 \}.
    \end{equation}
Let the controller $k:\R^n\times\tintc\to\R$ satisfy: 
% \begingroup\makeatletter\def\f@size{9}\check@mathfonts
\begin{align}
\label{eqn:cntrllyapreq}
    & \grad V_{\mb{x}_d}(\mb{x},t)(\mb{f}_{\mb{x}_d}(\mb{x},t)+\mb{g}(\mb{x})k(\mb{x},t)) \\ & \qquad\qquad\qquad\qquad\qquad\qquad \leq -\lambda_{\min}(\mb{Q})\Vert\mb{e}_{\mb{x}_d}(\mb{x},t)\Vert^2_2, \nonumber
\end{align}
% \endgroup
for almost all $t\in\tintc$ and all $\mb{x}\in\RobustInvariant_{\mb{x}_d}(t,\overline{w})$. Then for initial time $\underline{t}$, any initial condition $\mb{x}_0\in\RobustInvariant_{\mb{x}_d}(\underline{t},\overline{w})$, and any disturbance signal $\mb{w}$ satisfying $\Vert\mb{w}\Vert_{\infty}\leq \overline{w}$, we have that $I(\underline{t},\mb{x}_0,\mb{w}) = \tinto$, and $\bs{\varphi}(t) \in \RobustInvariant_{\mb{x}_d}(t,\overline{w})$ for all $t\in[\underline{t},\overline{t})$, and $\lim_{t\to\overline{t}}\bs{\varphi}(t)$ exists and satisfies $\lim_{t\to\overline{t}}\bs{\varphi}(t)\in\RobustInvariant_{\mb{x}_d}(\overline{t},\overline{w})$.
\end{lemma}
The preceding result follows by a standard input-to-state stability argument \cite{Sontag1989smooth}. For any $t\in\tintc$, the set $\RobustInvariant_{\mb{x}_d}(t,\overline{w})$ captures how accurately the nonlinear closed-loop system \eqref{eqn:closedloop_state} tracks $\mb{x}_d$ with disturbances. Importantly, for a given $t\in\tintc$ the set $\RobustInvariant_{\mb{x}_d}(t,\overline{w})$ is convex -- as we will see later, this property will allow us to efficiently synthesize a dynamically admissible trajectory $\mb{x}_d$ while knowing how accurately it will be tracked and ensuring state and input constraint satisfaction.

In contrast to cancelling the nonlinear dynamics to achieve linear dynamics as in \eqref{eqn:errordotcloop}, which may be unnecessary and inefficient \cite{freeman1996robust}, Control Lyapunov Functions (CLFs) provide an alternative method for synthesizing stabilizing controllers via convex optimization. In particular, we have that \eqref{eqn:lyapdecay} implies:
\begin{align}
\label{eqn:clfdecay}
&\inf_{u\in\R}\grad V_{\mb{x}_d}(\mb{x},t)(\mb{f}_{\mb{x}_d}(\mb{x},t)+\mb{g}(\mb{x})u) \\ & \qquad\qquad\qquad\qquad\qquad\qquad \leq  -\lambda_{\min}(\mb{Q})\Vert\mb{e}_{\mb{x}_d}(\mb{x},t)\Vert^2_2. \nonumber
\end{align}
for all $\mb{x}\in\R^n$ and $t\in\tintc$. Define a feed-forward controller $k_{\mb{x}_d}^{\rm ff}:\R^n\times\tintc\to\R$ as:
\begin{equation}
\label{eqn:feedforward}
    k_{\mb{x}_d}^{\textrm{ff}}(\mb{x},t) = -g(\mb{x})^{-1}\mathcal{F}_{\mb{x}_d}(\mb{x},t).
\end{equation}
This feed-forward controller is incorporated into the following controller specified via a convex quadratic program (QP):
\begin{align}
\tag{CLF-QP} \label{clf-qp}
    & k_{\mb{x}_d}^\textrm{clf}(\mb{x},t) =  \argmin_{u\in\R} \frac{1}{2}\Vert u-k_{\mb{x}_d}^{\textrm{ff}}(\mb{x},t)\Vert_2^2 \\ & \textrm{s.t.}  ~ \grad V_{\mb{x}_d}(\mb{x},t)(\mb{f}_{\mb{x}_d}(\mb{x},t)+\mb{g}(\mb{x})u) \leq  -\lambda_{\min}(\mb{Q})\Vert\mb{e}_{\mb{x}_d}(\mb{x},t)\Vert^2_2. \nonumber
\end{align}
Note that the constraint in this controller ensures that $k_{\mb{x}_d}^{\rm clf}$ satisfies the condition in \eqref{eqn:cntrllyapreq}.



% \AT{Decide if this goes here or in MPC}
% \begin{align}
%     \Vert \bs{\varphi}_{x}(t) - \mb{x}_d(t) \Vert & = \Vert \bs{\Phi}^{-1}(\bs{\varphi}_{\eta}(t)) - \bs{\Phi}^{-1}(\bs{\eta}_d(t)) \Vert, \nonumber \\
%     & \leq L_{\bs{\Phi}^{-1}}\Vert \bs{\varphi}_{\eta}(t) - \bs{\eta}_d(t) \Vert, \nonumber\\
%     & \leq  L_{\bs{\Phi}^{-1}}\gamma(\Vert\mb{w}\Vert_\infty).
% \end{align}


% \subsection{Input-to-State Stability}
% In many practical engineering settings, there are external disturbances to the dynamics of the system, yielding the following disturbed nonlinear control affine system:
% \begin{equation}
%     \label{eqn:eomdist}
%     \dot{\mb{x}} = \mb{f}(\mb{x}) + \mb{g}(\mb{x})\mb{u} + \mb{d}(t),
% \end{equation}
% with a piecewise continuous disturbance signal $\mb{d}:\R_{\geq 0}\to\R^n$. As before, a state-feedback controller yields a disturbed closed-loop system:
% \begin{equation}
%     \label{eqn:cloopdist}
%     \dot{\mb{x}}= \mb{f}(\mb{x}) + \mb{g}(\mb{x})\mb{k}(\mb{x},t)+\mb{d}(t),
% \end{equation}
% which for any initial time $t_0\in[\underline{t},\overline{t})$ and initial condition in $\mb{x}_0\in\R^n$ there exists a constant $\delta(t_0,\mb{x}_0)>0$ such that \eqref{eqn:closedloop1} has a unique solution $\bs{\varphi}_d:[t_0,t_0+\delta(t_0,\mb{x}_0))\to\R^n$ satisfying:
% \begin{align}
%     \dot{\bs{\varphi}}_d(t) & = \mb{f}(\bs{\varphi}(t)) + \mb{g}(\bs{\varphi}(t))\mb{k}(\bs{\varphi}(t),t)+\mb{d}(t), \label{eqn:distsoldiff}\\
%     \bs{\varphi}_d(t_0) & = \mb{x}_0. \label{eqn:distsolic}
% \end{align}
% for almost all $t\in [t_0,t_0+\delta(t_0,\mb{x}_0))$.

% Given a feedback linearizable system and a dynamically admissible trajectory, the disturbance signal subsequently induces\footnote{The relationship between $\mb{d}$ and $\mb{d}_{\bs{\eta}}$, and their respective bounds, is made explicit in Section \ref{sec:}.} a disturbance signal, denoted $\mb{d}_{\bs{\eta}}:\R_{\geq 0}\to\R^n$, in the dynamics of the error $\mb{e}$ defined in \eqref{eqn:err}:
% \begin{align}
%     \dot{\mb{e}}(\bs{\eta},t,\mb{u}) =&~\mb{f}_{\bs{\eta}}(\bs{\eta})+\mb{g}_{\bs{\eta}}(\bs{\eta})\mb{u} + \mb{d}_{\bs{\eta}}(t) \nonumber \\ &-\derp{\bs{\Phi}}{\mb{x}}(\mb{x}_d(t))(\f(\x_d(t))+\g(\x_d(t))\u_d(t)) \label{eqn:disterrdyn},
% \end{align}

% \blue{Add a comment that if the system is ISS, there exists a sublevel set of the Lyapunov function that is forward invariant.}
% Given the existence of a unique solution to the disturbed closed-loop system, consider the following definition:
% \begin{definition}{\textit{(Time-Varying Forward Invariance)}}
% A set-valued function $\C:\R_{\geq 0}\rightrightarrows\R^n$ defines a \emph{time-varying forward invariant set} if for any initial time $t_0\in[\underline{t},\overline{t}]$ and initial condition ${\mb{x}_0 \in \C(t_0)}$, we have ${\bs{\varphi}_d(t)\in\C(t)}$ for all $t\in[t_0,t_0+\delta(t_0,\mb{x}_0))$. 
% \end{definition}



% , implying that:
% \begin{equation}
%     \Vert \mb{e}(\bs{\Phi}(\bs{\varphi}(t)),t)\Vert_2 \leq -\exp()\Vert \mb{e}(\bs{\Phi}(\bs{\varphi}(0)),0)\Vert_2
% \end{equation}


% a controller $\mb{k}_{\mathrm{fbl}}: \mathcal{\R}^n \times \R^k \to \R^m$, $k\leq m$, and a controllable pair $(\mb{A}, \mb{B}) \in \R^{n \times n} \times \R^{n \times k}$ satisfying:
% \begin{equation}
% \label{eqn:fblindef}
%     D\bs{\Phi}(\mb{x})(\mb{f}(\mb{x}) + \mb{g}(\mb{x})\mb{k}_{\mathrm{fbl}}(\mb{x}, \mb{v})) = \mb{A}\bs{\Phi}(\mb{x}) + \mb{B}\mb{v} ,
% \end{equation}

% Consider a nonlinear control-affine system with state $\mb{x}=\begin{bmatrix} \mb{x}_1^\top \cdots \mb{x}_k^\top \end{bmatrix}^\top \in\R^n$ and dynamics of the form:
% \begin{equation}
%     \dot{\mb{x}}_i  =  \begin{bmatrix}\mb{0}_{n_i} & \mb{I}_{n_i-1 \times n_i-1} \\ 0 & \mb{0}_{n_i}  \end{bmatrix} \mb{x}_i+ \begin{bmatrix} \mb{0}_{n_i-1} \\ f_i(\mb{x})\end{bmatrix} + \begin{bmatrix} \mb{0}_{n_i-1 \times m} \\ \mb{g}_i(\mb{x}) \end{bmatrix} \mb{u}
% \end{equation}
% for $j = 1,\ldots,\gamma_i - 1$ and $i = 1,\ldots k$, where $\mb{f}_i:\R^n\to\R$ and $\mb{g}_i$



% \section{Preliminaries}
% In the following section, we will give the necessary background on Euler-Lagrange mechanics, Control Lyapunov Functions, and will introduce the problem formulation. Consider an Euler-Lagrange system with configuration coordinates $\q\in\Q\subseteq\R^n$ and state vector $\x=(\q,\dot\q)\in\mathcal{X}=T\Q\subseteq\R^{2n}$. Applying D'Alembert's principle to the Euler-Lagrange equations for the system, the dynamics can be written as:
% \begin{align}
%     \D(\q) + \H(\q,\dot \q) = \B\u \label{eq:robotEOM}
% \end{align}
% where $\D(\q)\in\mathbb{R}^{n\times n}$ is the mass-inertia matrix, $\H(\q,\dot\q)\in\R^n$ contains the Coriolis, gravity, and additional non-conservative forces, $\B\in\R^{n\times m}$ is the actuation matrix, and $\u\in\mathcal{U}\subseteq\mathbb{R}^m$ is the control input. The equations of motion in \eqref{eq:robotEOM} can be rearranged into control affine form as:
% \begin{align}
% \label{eq:eom}
%     \dot \x = \underbrace{\begin{bmatrix} \dot \q \\ -\D(\q)^{-1}\H(\q,\dot\q)\end{bmatrix}}_{\f(\x)} + \underbrace{\begin{bmatrix} \mb{0} \\ \D(\q)^{-1} \end{bmatrix}}_{\g(\x)} \u + \w,
% \end{align}
% where the drift vector, $\f:\mathbb{R}^{2n}\to\mathbb{R}^{2n}$, and actuation matrix, $\g:\mathbb{R}^{2n\times m}\to\mathbb{R}^{2n}$, are assumed to be twice continuously differentiable. This is subsumed by the standard assumption that the Lagrangian of the system is smooth. 

% \begin{definition}
% (Feedback Linearizeability) The system \eqref{eq:eom} with $k\in\N$, $k\le m$ time-varying outputs $\y:\mathcal{X}\times \R \to \cal{Y}\subseteq\R^k$ is said to be \textit{feedback linearizeable} of vector relative degree $\gamma\in\N^k$ with $\gamma_i \le 2n$ if there exists a feedback control law $\k:\cal{X}\times\V\times\R$ for an auxiliary control input $\v\in\V\subset\R^m $ such that:
% \begin{align*}
%     \dot \x = \f(\x) + \g(\x)\k(\x,\v,t) \implies \y_i^{(\gamma_i)} = \v_i~ \forall i=1,\dots,k.
% \end{align*}
% \end{definition}
% \begin{assumption}
% Assume that the nonlinear system \eqref{eq:eom} is square $(m=k)$, full state feedback linearizeable with time-varying outputs $\mb{y}:\cal{X}\times\mathbb{R}\to\cal{Y}$ of vector relative degree two $(m = n)$. In other words, the outputs have the structure of $\y(x,t) =\y_a(\q)- \y_d(t)$ for some twice differentiable desired trajectory $\y_d:\mathbb{R}\to\mathbb{R}^k$.
% \end{assumption}
% \noindent
% From the above assumption on feedback linearizeability, there exists a diffeomorphism $\mb{\Phi}:\mathcal{X} \to \cal{Y}$ and output coordinates $\bm{\eta} = \mb{\Phi}(\x)$ satisfying:
% \begin{align}
%     \bm{\eta} \triangleq \begin{bmatrix}\bm{\eta_1} \\ \bm{\eta_2}\end{bmatrix}  = \begin{bmatrix} \y_a(\q)-\y_d(t) \\ \mb{L}_{\f}\y_a(\x) - \dot \y_d(t) \end{bmatrix}.
% \end{align}
% Differentiating, we see:
% \begin{align}
%     \bm{\dot\eta} = \begin{bmatrix}\bm{\dot \eta_1} \\ \bm{\dot \eta_2}\end{bmatrix}  = \begin{bmatrix} \bm{\eta_2} \\ \mb{L}^2_{\f}\y_a(\x) + \mb{L}_\g\mb{L}_{\f}\y_a(\x)\u - \ddot \y_d(t) \end{bmatrix}.
% \end{align}
% Defining $\cal{F}(\x) = \mb{L}^2_{\f}\y_a(\x)$ and $\cal{G}(\x) = \mb{L}_\g\mb{L}_{\f}\y_a(\x)$, applying the following feedback controller $\k:\cal{X}\times\V\times\R\to\mathcal{U}$ results in:
% \begin{align}
% \label{eqn:FL_control}
%     \k= \mathcal{G}^{-1}(\x)(-\mathcal{F}(\x) + \y_d^{\vec \gamma}(t) + \v) \implies \dot \eta = \F\eta + \G\v
% \end{align}
% where the dependence on $(\x,\v,t)$ has been dropped for $\k$, and with $\F\in\R^{2k\times 2k}$, $\G\in\R^{2k\times m}$ defined as:
% % \begin{align*}
% %     \F &= 
% %     \begingroup\setlength\arraycolsep{0pt}\begin{bmatrix} \F_1 &&\mb{0}\\&\ddots&\\\mb{0}&&\F_k\end{bmatrix}\endgroup\F_i = \begin{bmatrix}0&1\\0&0\end{bmatrix}
% %     \G =
% %     \begingroup\setlength\arraycolsep{0pt}\begin{bmatrix} \G_1 &&\mb{0}\\&\ddots&\\\mb{0}&&\G_k\end{bmatrix}\endgroup\G_i &= \begin{bmatrix}0\\1\end{bmatrix}
% % \end{align*}
% \begin{align}
% \label{eq:fg}
%     \F =  \begin{bmatrix}0&1\\0&0\end{bmatrix} \otimes \mb{I}_k,\hspace{5mm}
%     \G = \begin{bmatrix}0\\1\end{bmatrix} \otimes \mb{I}_k
% \end{align}

% \begin{definition} (Input to State Stable Control Lyapunov Function)
% A continuously differentiable function $V:\mathcal{X}\to\mathbb{R}_{+}$ is An \textit{input to state stabilizing control Lyapunov function (ISS-CLF)} if there exist functions $\alpha_1,\alpha_2,\alpha_3,\rho\in\mathcal{K}_\infty$ satisfying:
% \begin{align*}
%     \alpha_1(\|\x\|) \le V(x) \le \alpha_2(\|\x\|) \\
%     \|\x\|\ge\rho(\|\w\|) \implies \inf_{\u\in\mathcal{U}}\dot V(\x,\u,\d) \le -\alpha_3 (\|\x\|)
% \end{align*}
% for all $\x\in\mathcal{X}$ and $\w\in\mathcal{W}$.
% \end{definition}
% \begin{lemma}
% [\red{Find citation}] Given a valid ISS-CLF, the set $\bar B_{\rho(\|\w\|_\infty)}$ is forward invariant.
% \end{lemma}
% Let $\E = \bar B_{\rho(\|\w\|_\infty)}$ represent the set which can be maintained forward invariant by the low-level controller under disturbances $\w$. An ISS-CLF controller can be constructed by solving the continuous algebraic Riccati equation:
% \begin{align*}
%     \F^T\P+\P\F-\P\G\G^T\P = -\mb{Q}
% \end{align*}
% for some $\P\succ 0$ given aby $\mb{Q} \succ0$ and constructing the Lyapunov function $V(\bm{\eta}) = \bm{\eta^TP\eta}$. A solution always exists because the pair $(\F,\G)$ from \eqref{eq:fg} is controllable, and this choise of Lyapunov function was shown to be input to state stable in \red{add reference}. Now, we can construct an ISS-CLF-QP as:
% \begin{equation}
%     \begin{aligned}
%     \k = \min_{\u\in\mathcal{U}} \quad & \|\mathcal{F}(\x) + \mathcal{G}(\x)\u - \y_d^{\vec \gamma}(t) - \v\|\\
% \textrm{s.t.} \quad & L_{\f}V(\x) + L_{\g}V(\x)\u\le -\gamma V + \frac{1}{\epsilon}\|L_{\g}V(\x)\|^2 \notag
% \end{aligned}
% \end{equation}
% Note that this could be replaced with any controller that allows for tracking a desired signal and enforces a robust invariant set $\mathcal{E}$.

% Finally, we remark on the brief background required for B\`ezier polynomials.
% [\red{cite cad book}]
% A B\`ezier polynomial $\Bez:[0,1]\to\mathbb{R}^k$ of degree $N$ is written, given $\b=[\b_0,\dots,\b_N]$ control points where $\b_i\in\R^k$, as $\Bez(\tau) = \b\Xi(\tau)$, where $\bm{\Xi}:\R\to\R^{N+1}$ is a vector-valued function defined as:
% \begin{align*}
%     \bm{\Xi_i}(\tau) = {n \choose i}(1-\tau)^{n-i}\tau^i.
% \end{align*}
% A powerful and well known property of B\`ezier polynomials is that their image is bounded by the convex hull of the control points, i.e. $\Bez(\tau) \in \text{conv}(\b)$ for all $\tau\in[0,1]$. By introducing the control points into the MPC program, we will be able to constraint tighten by the convex hull, and make conclusions about satisfaction of state and input constraints for the continuous time trajectory.




% \begin{align}
%     \bs{\eta} &= \begin{bmatrix}\eta_1 & \cdots & \eta_n \end{bmatrix}^\top, \\ 
%     \mb{f}_{\bs{\eta}}(\bs{\eta}) &= \begin{bmatrix}f_{\bs{\eta},1}(\bs{\eta}) & \cdots & f_{\bs{\eta},n}(\bs{\eta})\end{bmatrix}^\top, \\
%     \mb{g}_{\bs{\eta}}(\bs{\eta}) &= \begin{bmatrix}\mb{g}_{\bs{\eta},1}(\bs{\eta})^\top & \cdots & \mb{g}_{\bs{\eta},n}(\bs{\eta})^\top\end{bmatrix}^\top,
% \end{align}

% diffeomorphism $\bs{\Phi}: \mathcal{D} \to \mathcal{E}$ such that the \textit{transformed state}:
% \begin{equation}
% \label{eqn:transtate}
% \bs{\eta} = \begin{bmatrix}\bs{\eta}_1^\top \cdots \bs{\eta}_k^\top \end{bmatrix}^\top =  \bs{\Phi}(\mb{x}),
% \end{equation}
% with $\bs{\eta}_i\in\R^{n_i}$, $n_1+\ldots +n_k = n$, has dynamics governed by the nonlinear control-affine system:
% \begin{equation}
% \label{eqn:etadot}
% \dot{\bs{\eta}} = \mb{f}_{\bs{\eta}}(\bs{\eta})+\mb{g}_{\bs{\eta}}(\bs{\eta})\mb{u} =  \derp{\bs{\Phi}}{\mb{x}}(\mb{x})(\mb{f}(\mb{x}) + \mb{g}(\mb{x})\mb{u}),
% \end{equation}
% % \begin{equation}
% % \label{eqn:etadot}
% % \dot{\bs{\eta}} = \mb{f}_{\bs{\eta}}(\bs{\eta}) + \mb{g}_{\bs{\eta}}(\bs{\eta})\mb{u} = \derp{\bs{\Phi}}{\mb{x}}(\mb{x})(\mb{f}(\mb{x}) + \mb{g}(\mb{x})\mb{u}),
% % \end{equation}
% with $\mb{f}_{\bs{\eta}}:\mathcal{E}\to\R^n$ and $\mb{g}_{\bs{\eta}}:\mathcal{E}\to\R^{n\times m}$ such that: 
% \begin{equation}
% \label{eqn:etadotdecomp}
%     \dot{\bs{\eta}}_i  =  \begin{bmatrix}\mb{0}_{n_i-1} & \mb{I}_{n_i-1 \times n_i-1} \\ 0 & \mb{0}_{n_i-1}^\top  \end{bmatrix} \bs{\eta}_i+ \begin{bmatrix} \mb{0}_{n_i-1} \\ f_{\bs{\eta},i}(\bs{\eta})\end{bmatrix} + \begin{bmatrix} \mb{0}_{n_i-1 \times m} \\ \mb{g}_{\bs{\eta},i}(\bs{\eta})^\top \end{bmatrix} \mb{u},
% \end{equation}
% for all $\bs{\eta} \in \mathcal{E}$ and $\mb{u}\in\R^m$, with\footnote{Let $r_i = \sum_{j=1}^{i} n_j$. Then $f_{\bs{\eta},i}$ is the $r_i^{\textrm{th}}$ element of $\mb{f}_{\bs{\eta}}$, and $\mb{g}_{\bs{\eta},i}^\top$ the $r_i^{\textrm{th}}$ row of $\mb{g}_{\bs{\eta}}$. } $f_{\bs{\eta},i}:\mathcal{E}\to\R$ and $\mb{g}_{\bs{\eta},i}:\mathcal{E}\to\R^{m}$ for $i = 1,\ldots,k$. Furthermore the matrix:
% \begin{equation}
% \label{eqn:Gmat}
%     \mathcal{G}(\bs{\eta}) = \begin{bmatrix} \mb{g}_{\bs{\eta},1}(\bs{\eta}) & \cdots & \mb{g}_{\bs{\eta},k}(\bs{\eta}) \end{bmatrix}^\top \in \R^{k\times m},
% \end{equation}
% is right-invertible for all transformed states $\bs{\eta} \in \mathcal{E}$.

% \begin{align}
%     \label{eqn:etadotdecomp}
%     \dot{\bs{\eta}}_i  =  \begin{bmatrix}\mb{0}_{\gamma_i-1} & \mb{I}_{\gamma_i-1 \times \gamma_i-1} \\ 0 & \mb{0}_{\gamma_i-1}^\top  \end{bmatrix} \bs{\eta}_i   + \begin{bmatrix} \mb{0}_{\gamma_i-1} \\ f_{\bs{\eta},r_i}(\bs{\eta})\end{bmatrix}  + \begin{bmatrix} \mb{0}_{\gamma_i-1 \times m} \\ \mb{g}_{\bs{\eta},r_i}(\bs{\eta}) \end{bmatrix} \mb{u}.
% \end{align}
% and the error:
% \begin{equation}
% \label{eqn:err}
% \mb{e} = \begin{bmatrix}\mb{e}_{1}^\top \cdots \mb{e}_{k}^\top \end{bmatrix}^\top = \bs{\eta}- \bs{\eta}_{d}(t).
% \end{equation}
% with $\mb{e}_i\in\R^{\gamma_i}$. We have that:
% \begin{align}
%     \dot{\mb{e}} = \mb{f}_{\bs{\eta}}(\bs{\eta})&+\mb{g}_{\bs{\eta}}(\bs{\eta})\mb{u} \nonumber \\ &-\grad\bs{\Phi}(\mb{x}_d(t))(\f(\x_d(t))+\g(\x_d(t))\u_d(t)) \label{eqn:errdyn},
% \end{align}
% where it follows from \eqref{eqn:openloop_eta}-\eqref{eqn:etadotdecomp} that:

% \begin{equation}
%     \label{eqn:transtate}
%     \bs{\eta} = \begin{bmatrix}\bs{\eta}_1^\top \cdots \bs{\eta}_k^\top \end{bmatrix}^\top,\,\bs{\eta}_d(t) = \begin{bmatrix}\bs{\eta}_{d,1}(t)^\top \cdots \bs{\eta}_{d,k}(t)^\top \end{bmatrix}^\top,
% \end{equation}
% with $\bs{\eta}_i\in\R^{\gamma_i}$ and $\bs{\eta}_{d,i}:[\underline{t},\overline{t}]\to\R^{\gamma_i}$,

% \begin{lemma}
% Let $K\subseteq \mathcal{E}$ be a compact set and let a controller $\mb{k}:\mathcal{E}\times[\underline{t},\overline{t}]\to\R^m$ satisfy:
% \begin{align}
% \grad V(\mb{e}(\bs{\eta},t))\dot{\mb{e}}(\bs{\eta},t,\mb{k}(\bs{\eta},t))  \leq &  -\mb{e}(\bs{\eta},t)^\top\mb{Q}\mb{e}(\bs{\eta},t) \nonumber
% \\ & +2\mb{e}(\bs{\eta},t)^\top\mb{P}\mb{w}_{\eta}(\bs{\eta},t) 
% \end{align}
% for all $\bs{\eta}\in\mathcal{E}$ and $t\in[\underline{t},\overline{t}]$.

% Then there exists $w_{\rm max}\in\R_{>0}$ and a class $\mathcal{K}$ function $\gamma:[0,w_{\rm max})\to\R_{\geq 0}$ 

% such that for any $\overline{w}\in[0,w_{\rm max})$ such that the set:
% \begin{equation}
%     \RobustInvariant(t) = \{\bs{\eta}\in\mathcal{E} ~|~ V(\bs{\eta},t) \leq \gamma(\overline{w}) \}
% \end{equation}
% satisfies $\RobustInvariant(t)\subseteq K$ for all $[\underline{t},\overline{t}]$, 

% then for the initial time $\underline{t}$, any initial condition $\bs{\eta}_0\in\RobustInvariant(\underline{t})$, any disturbance $\mb{w}$ satisfying $\Vert\mb{w}\Vert_{\infty}\leq \overline{w}$ and 


% we have that $\bs{\varphi}_{\eta}(t) \in \RobustInvariant(t)$ for all $t\in[\underline{t},\overline{t}]$.
% \end{lemma}

% Before defining Control Lyapunov Functions, we denote a continuous function $\alpha:[0,a)\to\R_{\geq 0}$, with $a>0$, as \textit{class $\K$} ($\alpha\in\K$) if $\alpha(0)=0$ and $\alpha$ is strictly monotonically increasing. If $a=\infty$ and $\lim_{r\to\infty}\alpha(r)=\infty$, then $\alpha$ is \textit{class $\K_\infty$} ($\alpha\in\K_\infty$). More details on these functions may be found in \cite{kellett2014compendium}, but they enable the following definition:

% \begin{definition}[\textit{Control Lyapunov Functions}, \cite{artstein1983stabilization, jankovic2018robust}]
% A continuously differentiable function $V:\R^n\to\R_{\geq 0}$ is a \textit{Control Lyapunov Function (CLF)} for \eqref{eqn:errdyn} if there exist $\alpha_1,\alpha_2,\alpha_3 \in \K_\infty$ such that for all $\bs{\eta}\in\mathcal{E}$, $t\in[\underline{t},\overline{t}]$ and almost all $t'\in[\underline{t},\overline{t}]$:
% \begin{align}
%     \alpha_1(\Vert\mb{e}(\bs{\eta},t)\Vert) \leq V(\mb{e}(\bs{\eta},t)) & \leq \alpha_2(\Vert\mb{e}(\bs{\eta},t)\Vert), \label{eqn:clfbounds} \\ \inf_{\mb{u}\in\R^m}\derp{V}{\mb{e}}(\mb{e}(\bs{\eta},t'))\dot{\mb{e}}(\bs{\eta},t',\mb{u}) & < -\alpha_3(\Vert\mb{e}(\bs{\eta},t')\Vert). \label{eqn:clfdecay}
% \end{align}
% \end{definition}
% The function $V$ defined in \eqref{eqn:lyap} satisfies \eqref{eqn:clfbounds}--\eqref{eqn:clfdecay} with $\alpha_i(r) = k_ir^2$ with $k_1 = \lambda_{\textrm{min}}(\mb{P})$, $k_2 = \lambda_{\textrm{max}}(\mb{P})$, and $k_3 = \lambda_{\textrm{min}}(\mb{Q}')$ for any $\mb{Q}'\in\mathbb{S}^n_{\succ 0}$ such that $\mb{Q}' \prec \mb{Q}$.

%\footnote{More specifically, the piecewise-continuous differentiability of $\mb{x}_d$ implies the existence of a unique finite subdivision $\{t_0,\ldots,t_N\}$, $N\in\mathbb{N}$, with $t_0 = \underline{t}$ and $t_N = \overline{t}$ such that $\mb{x}_d$ is continuously differentiable on the open intervals $(t_i,t_{i+1})$, $i=0,\ldots,N-1$, and is not differentiable at the points $\{t_0,\ldots,t_N\}$. The equality in \eqref{eqn:dynadmistraj} is required to hold on these open intervals.}
%
% \footnote{In the presence of discontinuities of the controller $\mb{k}$ in time, the expression in \eqref{eqn:soldiff} is understood to be satisfied by the solution $\bs{\varphi}$ almost everywhere on the domain $I(\mb{x}_0)$.} 
%
%
% We will use the following definition in characterizing the behavior of a nonlinear system around a dynamically admissible trajectory:
% \begin{definition}{\textit{(Time-Varying Forward Invariance)}}
% A set-valued function $\C:\R_{\geq 0}\rightrightarrows\R^n$ defines a \emph{time-varying forward invariant set} if for any initial time $t_0\in[\underline{t},\overline{t}]$ and initial condition ${\mb{x}_0 \in \C(t_0)}$, we have ${\bs{\varphi}(t)\in\C(t)}$ for all $t\in[t_0,t_0+\delta(t_0,\mb{x}_0))$. 
% \end{definition}
%
% The combination of continuous-time controllers with discrete-time planners yields functions satisfying different differentiability properties. We denote the \textit{right-handed derivative} of a piecewise continuously differentiable function $\bs{\varphi}:\R\to\R^n$ at $t\in\R$ as:
% \begin{equation*}
%     \dot{\bs{\varphi}}^r(t) = \lim_{h\to 0^+}\frac{1}{h}(\bs{\varphi}(t+h)-\bs{\varphi}(h)),
% \end{equation*}
% and note that if $\bs{\varphi}$ is continuously differentiable, we have $\dot{\bs{\varphi}}(t) = c \implies \dot{\bs{\varphi}}^r(t) = c$. Given a continuously differentiable function $\bs{\psi}:\R^n\to\R^p$, a piecewise continuously differentiable function $\bs{\varphi}:\R\to\R^n$, and denoting $\bs{\RobustInvariant}=(\bs{\psi}\circ\bs{\varphi})$, we have that:
% \begin{equation*}
%     \dot{\bs{\RobustInvariant}}^r(t) = \grad\bs{\psi}(\bs{\varphi}(t))\dot{\bs{\varphi}}^r(t)
% \end{equation*}
% where $\grad\bs{\psi}:\R^n\to\R^{p\times n}$ is the standard derivative of $\bs{\psi}$. Lastly, if $\varphi:\R\to\R$ is piecewise continuously differentiable, we have that $\dot{\varphi}^r(t) = c \implies D^+\varphi(t) = c$, where $D^+\varphi:\R\to\R_e$ is the \textit{upper right-hand Dini derivative} \cite{khalil2002nonlinear}.
%
% Feedback linearization offers a tool for the synthesis of stabilizing controllers for nonlinear systems, and will serve an important role in tracking dynamically admissible trajectories generated via model predictive control. In this work we consider the following abbreviated definition, but additional details may be found in \cite{isidori1995nonlinear, sastry1999nonlinear}:
%
% \begin{definition}[\textit{Full-State Feedback Linearizability}]
% The system \eqref{eqn:openloop_state} is \textit{full-state feedback linearizable} if there exist open sets $\mathcal{D},\mathcal{E}\subseteq\R^n$, a diffeomorphism $\bs{\Phi}:\mathcal{D}\to\mathcal{E}$, and $\gamma_1,\ldots,\gamma_k\in\mathbb{Z}_{>0}$ satisfying $\sum_{i=1}^k\gamma_i = n$ such that defining functions $\mb{f}_{\eta}:\mathcal{E}\to\R^n$ and $\mb{g}_{\eta}:\mathcal{E}\to\R^{n\times m}$ as:
% \begin{align}
%   \mb{f}_{\eta}(\bs{\eta}) &= \grad\bs{\Phi}(\bs{\Phi}^{-1}(\bs{\eta}))\mb{f}(\bs{\Phi}^{-1}(\bs{\eta})), \label{eqn:feta} \\  \mb{g}_{\eta}(\bs{\eta}) &= \grad\bs{\Phi}(\bs{\Phi}^{-1}(\bs{\eta}))\mb{g}(\bs{\Phi}^{-1}(\bs{\eta})), \label{eqn:geta}
% \end{align}
% and denoting:
% \begin{equation}
% \label{eqn:etaidx}
%     \bs{\eta} = \begin{bmatrix}\eta_1 \\ \vdots \\ \eta_n \end{bmatrix},\, \mb{f}_{\eta}(\bs{\eta}) = \begin{bmatrix}f_{\eta,1}(\bs{\eta}) \\ \vdots \\ f_{\eta,n}(\bs{\eta})\end{bmatrix},\, \mb{g}_{\eta}(\bs{\eta}) = \begin{bmatrix}\mb{g}_{\eta,1}(\bs{\eta}) \\ \vdots \\ \mb{g}_{\eta,n}(\bs{\eta})\end{bmatrix},
% \end{equation}
% and $r_j = \sum_{i=1}^j \gamma_i$, for $j = 1,\ldots,k$, we have that:
% \begin{enumerate}
% \item The functions $f_{\eta,i}$ and $\mb{g}_{\eta,i}$ satisfy:
% \begin{align}
% \label{eqn:etaintegrator}
%     f_{\eta,i}(\bs{\eta}) = \eta_{i+1}, \qquad
%     \mb{g}_{\eta,i}(\bs{\eta}) = \mb{0}_{1\times m},
% \end{align}
% for all $i\notin\{r_1,\ldots,r_k\}$ and all $\bs{\eta}\in \mathcal{E}$.
% \item The matrix:
%     \begin{equation}
%     \label{eqn:Gmat}
%         \mathcal{G}(\bs{\eta}) = \begin{bmatrix} \mb{g}_{\eta,r_1}(\bs{\eta})^\top & \cdots & \mb{g}_{\eta,r_k}(\bs{\eta})^\top \end{bmatrix}^\top,
%     \end{equation}
%     is right-invertible for all $\bs{\eta} \in \mathcal{E}$.
% \end{enumerate}
% \end{definition}
% Given a disturbance signal $\mb{w}:\R_{\geq 0}\to\mathcal{W}$, define $\mb{w}_{\eta}:\mathcal{E}\times \R_{\geq 0}\to\R^n$ as:
% \begin{equation}
%     \mb{w}_{\eta}(\bs{\eta},t) = \grad\bs{\Phi}(\bs{\Phi}^{-1}(\bs{\eta}))\mb{w}(t),
% \end{equation}
% and consider the nonlinear control-affine system:
% \begin{equation}
% \label{eqn:openloop_eta}
%     \dot{\bs{\eta}} = \mb{f}_{\eta}(\bs{\eta}) + \mb{g}_{\eta}(\bs{\eta})\mb{u} + \mb{w}_{\eta}(\bs{\eta},t).
% \end{equation}
% with state $\bs{\eta}\in\mathcal{E}$. As before, a feedback controller $\mb{k}:\mathcal{E}\times\R_{\geq 0}\to\R^m$ that is locally Lipschitz continuous with respect to its first argument and piecewise continuous with respect to its second argument on $\mathcal{E}\times\R_{\geq 0}$ yields the closed-loop system: 
% \begin{equation}
% \label{eqn:closedloop_eta}
%     \dot{\bs{\eta}} = \mb{f}_{\eta}(\bs{\eta}) + \mb{g}_{\eta}(\bs{\eta})\mb{k}(\bs{\eta},t) + \mb{w}_{\eta}(\bs{\eta},t),
% \end{equation}
% As the function $\bs{\Phi}$ is a diffeomorphism between the sets $\mathcal{D}$ and $\mathcal{E}$, the controller $\mb{k}':\mathcal{D}\times\R_{\geq 0}\to\R^m$ defined as:
% \begin{equation}
% \label{eqn:kprime}
%     \mb{k}'(\mb{x},t) = \mb{k}(\bs{\Phi}(\mb{x}),t),
% \end{equation}
% is locally Lipschitz continuous with respect to its first argument and piecewise continuous with respect to its second argument on $\mathcal{D}\times\R_{\geq 0}$. Consequently, for any initial time $t_0\in\R_{\geq 0}$, initial condition $\bs{\eta}_0 \in \mathcal{E}$ and piecewise continuous $\mb{w}:\R_{\geq 0}\to\mathcal{W}$, there exists an interval $I_{\eta}(t_0,\bs{\eta}_0,\mb{w})\triangleq[t_0,t_0+\delta_{\eta}(t_0,\bs{\eta}_0,\mb{w}))$ with $ \delta_{\eta}(t_0,\bs{\eta}_0,\mb{w})\in\R_{>0}$ such that the system \eqref{eqn:closedloop_eta} has a unique piecewise continuously differentiable solution $\bs{\varphi}_{\eta}:I_{\eta}(t_0,\bs{\eta}_0,\mb{w})\to\mathcal{E}$ satisfying:
% \begin{align}
%     \dot{\bs{\varphi}}_{\eta}(t) & = \mb{f}_{\eta}(\bs{\varphi}_\eta(t)) + \mb{g}(\bs{\varphi}_\eta(t))\mb{k}(\bs{\varphi}_{\eta}(t),t)   +\mb{w}_{\eta}(\bs{\varphi}_{\eta}(t),t), \label{eqn:soldiff_eta} \\
%     \bs{\varphi}_{\eta}(t_0) & = \bs{\eta}_0.  \label{eqn:solic_eta}
% \end{align}
% for almost all $t\in I_{\eta}(t_0,\bs{\eta}_0,\mb{w})$. Moreover, we have that:
% \begin{equation}
%     \bs{\varphi}_{\eta}(t)  =  \bs{\Phi}(\bs{\varphi}_x(t)),
% \end{equation}
% for all $t\in I(t_0,\bs{\eta}_0,\mb{w})$, where $\bs{\varphi}_x:I_{\eta}(t_0,\bs{\eta}_0,\mb{w})\to\mathcal{D}$ is the solution to \eqref{eqn:closedloop_state} defined with the controller $\mb{k}'$ for initial time $t_0$, initial condition $\mb{x}_0 = \bs{\Phi}^{-1}(\bs{\eta}_0)$, and disturbance $\mb{w}$. 
%
% The relationship between the solutions satisfying \eqref{eqn:soldiff_state}--\eqref{eqn:solic_state} and \eqref{eqn:soldiff_eta}--\eqref{eqn:solic_eta} permits us to design controllers directly for the system \eqref{eqn:openloop_eta} rather than the system \eqref{eqn:openloop_state}, a task which is often easier due to the structural properties in \eqref{eqn:etaintegrator}-\eqref{eqn:Gmat}.
%
% Importantly, these properties are not defined with respect to a specific dynamically admissible trajectory, but rather can be used to stabilize the system \eqref{eqn:openloop_state} to \textit{any} dynamically admissible trajectory contained in $\mathcal{D}$. 
%

% Let us denote:
% \begin{align}
%     \mb{e}(\bs{\eta},t) &= \begin{bmatrix}\mb{e}_1(\bs{\eta},t)^\top & \cdots & \mb{e}_k(\bs{\eta},t)^\top \end{bmatrix}^\top, \\
%     \dot{\mb{e}}(\bs{\eta},t,\mb{u}) &= \begin{bmatrix}\dot{\mb{e}}_1(\bs{\eta},t,\mb{u})^\top & \cdots & \dot{\mb{e}}_k(\bs{\eta},t,\mb{u})^\top \end{bmatrix}^\top, \\
%      \mb{w}_{\eta}(\bs{\eta},t) &= \begin{bmatrix}  \mb{w}_{\eta,1}(\bs{\eta},t)^\top & \cdots &  \mb{w}_{\eta,k}(\bs{\eta},t)^\top \end{bmatrix}^\top,
% \end{align}
% with $\mb{e}_i:\mathcal{E}\times[\underline{t},\overline{t}]\to\R^{\gamma_i}$, $\dot{\mb{e}}_i:\mathcal{E}\times[\underline{t},\overline{t}]\times\R^m\to\R^{\gamma_i}$, and $\mb{w}_{\eta,i}:\mathcal{E}\times\R_{\geq 0}\to\R^{\gamma_i}$, and define $\mathcal{F}:\mathcal{E}\times[\underline{t},\overline{t}]\to\R^k$ as:
% \begin{equation}
%     \mathcal{F}(\bs{\eta},t) = \begin{bmatrix} \mathcal{F}_1(\bs{\eta},t) & \cdots & \mathcal{F}_k(\bs{\eta},t)  \end{bmatrix}^\top,
% \end{equation}

==> 3_BezierCurvesStateConstraints.tex <==
\section{B\'{e}zier Curves \& State Constraints}
\label{sec:bezier}
%%%%%%%

% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\linewidth]{Figures/MethodFig_Long.pdf}
%     \caption{A depiction of the proposed method, where the control points of the B\'ezier curve are constraint tightened by the size of the robust invariant tube coming from the low-level controller. \AT{Fix $\Omega$ subscript}}
%     \label{fig:BoundDepiction}
% \end{figure*}

In this section we present the first main contribution of this work by addressing how the properties of the low-level tracking controller can be used to place requirements on a dynamically admissible trajectory $\mb{x}_d$ that ensure state constraint satisfaction by the closed-loop nonlinear system \eqref{eqn:closedloop_state} evolving under controllers such as $k_{\mb{x}_d}^{\rm fbl}$ or $k_{\mb{x}_d}^{\rm clf}$. 

We first make the following assumption regarding the state constraints for the system:
\begin{assumption}
\label{ass:statepolytope}
The state constraint set $\mathcal{X}\subset\mathbb{R}^n$ is a compact, convex polytope, with the existence of $\mb{L}_j\in\R^n$ and $\ell_j\in\R$ for $j=1,\ldots, q$ such that $\mathcal{X} = \{\x \in \R^n ~|~ \forall j,\, \mb L^\top_j\x \leq \ell_j\}$. Furthermore, we have that $\mb{0}\in\textrm{Int}(\mathcal{X})$.
\end{assumption}
\noindent Given the above state constraints, it is not the case -- even for a dynamically admissible trajectory satisfying $\mb{x}_d(t)\in\mathcal{X}$ for all $t\in\tintc$ -- that the state will remain inside the set $\mathcal{X}$, as we may have that $\RobustInvariant_{\mb{x}_d}(t,\overline{w})\nsubseteq\mathcal{X}$ for some $t\in\tintc$. To ensure these constraints are met by the closed-loop system without directly modifying the low-level control design, we will incorporate information about the low-level controller when constructing $\x_d$. The core tool that will enable incorporating this information is \emph{B\'{e}zier curves} \cite{kamermans2020primer}.


Let $T\in\R_{>0}$. A B\'ezier curve  $\BEZc:[0,T]\to\mathbb{R}$ of order $p$ is defined as:
\begin{align}
\label{eqn:bez}
    \BEZc(\tau) = \Bez_0^\top \z(\tau),
\end{align}
where $\Bez_0 = \begin{bmatrix}\bez_{0,0} & \ldots & \bez_{0,p}\end{bmatrix}^\top\in\mathbb{R}^{p+1}$ is a vector with elements consisting of the $p+1$ \textit{control points}, $\bez_{0,i}\in\mathbb{R}$, of the curve and $\z:[0,T]\to\mathbb{R}^{p+1}$ is a Bernstein polynomial defined elementwise as:
\begin{align}
    z_{i}(\tau) = \binom{p}{i} \left(\frac{\tau}{T}\right)^i\left(1-\frac{\tau}{T}\right)^{p-i}, ~~ i=0,\dots, p.
\end{align}
The curve $\BEZc$ is smooth, and there exists a matrix\footnote{The matrices $\mb{H}$ and $\mb{D}$ are uniquely defined by the order of the B\'ezier curve $p$ and can be constructed as shown in the extended version \cite{csomay2022multirate_extended}.\label{HandDfootnote}} $\mb{H}\in\R^{p+1\times p+1}$ such that the $j^{th}$ derivative of $\BEZc$ is given by:
\begin{equation}
\label{eqn:bezjderiv}
    {\BEZc}^{(j)}(\tau) = \frac{1}{T^j}\Bez_0^\top \mb H^j \z (\tau) \triangleq \bs{\xi}_j^\top\mb{z}(\tau).
\end{equation}
Consequently, $\BEZc^{(j)}:[0,T]\to\R$ is a B\'ezier curve of order $p$ with the elements of $\Bez_j$ (which are uniquely and linearly defined by $\bs{\xi}_0$) as control points. Define the function $\BEZC:[0,T]\to\R^n$:
\begin{equation}
\label{eqn:bezpolyvec}
    \BEZC(\tau) = \begin{bmatrix} \BEZc(\tau) & \BEZc^{(1)}(\tau) & \cdots & \BEZc^{(n-1)}(\tau) \end{bmatrix}^\top.
\end{equation}
There exists a matrix\footref{HandDfootnote}
% \footnote{The matrix $\mb{D}$ is uniquely defined by the order of the B\'ezier curve $p$ and can be constructed as shown in the extended version \cite{csomay2022multirate_extended}.}
$\mb D\in\R^{2n\times 2n}$ such that for any two vectors $\x_0,\x_1\in\R^n$, the unique B\'ezier curve $\BEZc$ of order $2n-1$ satisfying $\BEZC(0) = \x_0$ and $\BEZC(T) = \x_1$ with a vector of control points $\Bez_0\in\R^{2n}$ is given by:  
\begin{align}
\label{eqn:bezbndcond}
    \Bez^\top_0 =  \begin{bmatrix} \x_0^\top & \x_1^\top \end{bmatrix}\mb{D}^{-1}.
\end{align}
% where $\mb D\in\mathbb{R}^{2n \times 2n}$.
% \begingroup\makeatletter\def\f@size{9}\check@mathfonts
% \begin{align*}
%     \mb D = \begin{bmatrix}\mb H^0\z(0) & \cdots & \mb H^{n-1}\z(0)& \mb H^0\z(T) & \cdots & \mb H^{n-1}\z(T) \end{bmatrix}.
% \end{align*}
% \endgroup
% \begin{align*}
%     \mb D = \begin{bmatrix}\frac{1}{T^0}\mb H^0\z(0) & \cdots & \frac{1}{T^{n-1}}\mb H^{n-1}\z(0)& \frac{1}{T^0}\mb H^0\z(T) & \cdots & \frac{1}{T^{n-1}}\mb H^{n-1}\z(T) \end{bmatrix}.
% \end{align*}
% \begin{align*}
%     \mb D = \begin{bmatrix}\frac{1}{T^0}\mb H^0\z(0) & \cdots & \frac{1}{T^{n-1}}\mb H^{n-1}\z(0)& \frac{1}{T^0}\mb H^0\z(T) & \cdots & \frac{1}{T^{n-1}}\mb H^{n-1}\z(T) \end{bmatrix}.
% \end{align*}

The following result (proven in \cite{csomay2022multirate_extended}) shows how a sequence of points may be used to construct a set of B\'{e}zier curves that constitute a dynamically admissible trajectory for \eqref{eqn:openloop_state}: 

\begin{lemma}
\label{lem:bezdynadmistraj}
Let $N\in\mathbb{N}$, $\underline{t}\in\R_{\geq 0}$, and define $\overline{t}=\underline{t}+NT$ . For $k = 0,\ldots,N$, consider a collection of points $\{\mb{x}_k\}$
with $\mb{x}_k\in\R^n$ and define $t_k\in\R_{\geq 0}$ as $t_k = \underline t + kT$. For $k=0,\ldots,N-1$, let $\BEZc_k:[0,T]\to\R$ be a B\'{e}zier curve of order $2n-1$ with control points $(\Bez_k)_0 = \begin{bmatrix}(\bez_k)_{0,0} & \ldots & (\bez_k)_{0,2n-1}\end{bmatrix}^\top\in\R^{2n}$ given by:
\begin{equation}
\label{eqn:bezsetctrlpts}
    (\bs{\xi}_k)_0^\top = \begin{bmatrix} \mb{x}_{k}^\top & \mb{x}_{k+1}^\top \end{bmatrix}\mb{D}^{-1}.
\end{equation}
Defining the functions $\BEZC_k:[0,T]\to\R^n$ as in \eqref{eqn:bezpolyvec}, we have that the function $\mb{x}_d:\tintc\to\R^n$ defined as:
\begin{align}
\label{eqn:dyn_admissible_traj}
\mb{x}_d(t) &= \BEZC_k\left(t-t_k\right),\, t\in\left[t_k,t_{k+1} \right), \nonumber \\
\mb{x}_d(\overline{t}) &= \mb{x}_N,
\end{align}
is a dynamically admissible trajectory for the system \eqref{eqn:openloop_state}.
\end{lemma}

We note that the preceding result reduces planning of an (infinite dimensional) continuous time trajectory to planning a finite sequence of points. This aligns with planning dynamically admissible trajectories online in a multi-rate approach. While other classes of functions (such as general polynomials) may similarly be used to construct dynamically admissible trajectories for \eqref{eqn:openloop_state}, the motivation for using B\'{e}zier curves lies in the convex hull relationship between the curve $\BEZC_k$ and the control points $(\Bez_k)_0,\ldots,(\Bez_k)_{n-1}$. More precisely, for $i=0,\ldots,2n-1$ denote:
\begin{equation}
    (\bs{\zeta}_k)_i \triangleq \begin{bmatrix}(\bez_k)_{0,i}&\ldots& (\bez_k)_{n-1,i}\end{bmatrix}^\top\in\R^n.
\end{equation}
% $(\bs{\zeta}_k)_i \triangleq \begin{bmatrix}(\bez_k)_{0,i}&\ldots& (\bez_k)_{n-1,i}\end{bmatrix}^\top\in\R^n$.
The points $(\Bez_k)_j$ can be viewed as the control points in time for the curve $\BEZc_k^{(j)}$, while $(\bs{\zeta}_k)_i$ reflects the control points for the curve $\BEZC_k$ realized in state space. This enables the following:


\begin{fact}[\cite{kamermans2020primer} \S4]
\label{fct:cvxhull}
We have that $\BEZC_k(\tau)\in\textrm{conv}(\{(\bs{\zeta}_k)_i\})$ for all $\tau\in[0,T]$. 
\end{fact}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/MethodFig_v3.pdf}
    \caption{A depiction of the proposed method, where the control points of the B\'ezier curve are constraint tightened by the size of the robust invariant tube coming from the low-level controller.}
    \label{fig:BoundDepiction}
    \vspace{-5mm}
\end{figure}

We may immediately use this property to establish the following result (proven in \cite{csomay2022multirate_extended}) regarding state constraints:

\begin{lemma}
\label{lem:robust_hull}
Define the convex, compact set $\ErrorSet \subseteq \R^n$ as:
\begin{equation}
    \ErrorSet = \{ \mb{v}\in\R^n ~|~ \mb{v}^T \mb P \mb{v} \leq \gamma \overline w^2\}.
\end{equation}
If $(\BEZ_k)_i \in \mathcal{X} \ominus \ErrorSet$ for $i =0,\ldots,2n-1$ and $k=0,\ldots,N-1$, then we have that $\Omega_{\mb{x}_d}(t,\overline{w})\subseteq \mathcal{X}$ for all $t\in\tintc$.
% $\Omega_{\mb{x}_d}(t,\overline{w})\subseteq \mathcal{X}$ for all $t\in\tintc$.
\end{lemma}


% A resulting consequence is that constructing a dynamically admissible trajectory $\mb{x}_d$ as in Lemma \ref{lem:bezdynadmistraj} with control points $(\bs{\xi}_k)_0$ such that the corresponding $(\bs{\zeta}_k)_i$ satisfy $(\BEZ_k)_i \in \mathcal{X} \ominus \ErrorSet$ for $i = 0,\ldots,2n-1$ and $k=0,\ldots,N$, implies the set $\Omega(t,\overline{w})$ defined in Lemma \ref{lem:lowleveliss} satisfies $\Omega(t,\overline{w})\subseteq\mathcal{X}$ for all $t\in\tintc$.
This result states that by constraining the B\'{e}zier curve control points, we can ensure the evolution of the system under the low-level controller satisfies state constraints. The requirement that  $(\BEZ_k)_i \in \mathcal{X} \ominus \ErrorSet$ can be expressed as an affine inequality constraint as in the following result (proven in \cite{csomay2022multirate_extended}):
% \begin{lemma}
% \label{lem:affine_robust}
% Let $\mb{L}_j\in\R^{n}$ and $\ell_j\in\R$ for $j=1,\ldots,q$ be such that $\mathcal{X} = \{\x \in \R^n ~|~ \forall j,\, \mb L^\top_j\x \leq \ell_j\}$. Then we have that:
% \begin{equation}
%     \BEZ_i\in\mathcal{X} \ominus \E \iff \mb L_j^\top\BEZ_i \le \ell_j-\sqrt{\gamma\overline{w}^2\mb L^\top_j \mb P^{-1}\mb L_j},\,\, \forall j.
% \end{equation}
% \end{lemma}

\begin{lemma}
\label{lem:state_bound} 
We have that for $j=1,\ldots,q$:
\begin{align}
    (\BEZ_k)_i\in\mathcal{X} \ominus \E \Leftrightarrow \mb L_j^\top(\BEZ_k)_i \le \ell_j-\sqrt{\gamma\overline{w}^2\mb L^\top_j \mb P^{-1}\mb L_j}.
\end{align}% % % % 
\end{lemma}




% With this fix, the formulation is convex (and even conic for some norm cone), but is not a standard cone constraint as it is a quadratic form of norms. As opposed to \eqref{eqn:M_eq}-\eqref{eqn:s_def}, the benefit of the above constraint is that it can be converted into an SOCP via completion of the square. \red{should we make a comment that this reformulation is not a relaxation?}


% \AT{Motivate convexity vs other polynomials}
% \NCS{As shown above, B\'ezier polynomials allow us to produce continuous dynamically admissible trajectories while only having to reason about a discrete collection of points. B\'ezier polynomials were chosen over any other arbitrary polynomial basis because of another important property: the curve $\BEZC$ is contained in the convex hull of the control points. Stated more formally, consider the control points of a B\'ezier curve $\BEZc$ and its derivatives, $\{\Bez_0,\ldots,\Bez_p\}$. From this collection, we can construct $\bs{\zeta}_i = \begin{bmatrix}\bez_{0,i}&\ldots& \bez_{n-1,i}\end{bmatrix}$ for $i\in\{0,\ldots,2n-1\}$ corresponding to the control points of the curve in state space. Then, we have that $\BEZC(\tau) \in \text{conv}(\{\bs{\zeta}_i\})$ for $i=0,\ldots,2n-1$ and $\tau\in[0,T]$ \cite{BezierBook}. This key property will lay the foundation for the state and input constraint satisfaction guarantees that will be made.}

% \begin{proposition}
% \label{prop:dynFeasTraj}
% Let $\mb{x}_1,\mb{x}_2\in\R^n$, and let the function $\BEZC:[0,1]\to\R^n$ be defined as in \eqref{eqn:bezpolyvec} from a B\'{e}zier curve $\BEZc:[0,1]\to\R$ of order $p$ with control points $\bs{\xi}\in\R^{p+1}$ defined as in \eqref{eqn:bezbndcond}. Then for $\underline{t},\overline{t}\in\R_{\geq 0}$ with $\underline{t}<\overline{t}$, we have that the function $\mb{x}_d:\tintc\to\R^n$ defined as:
% \begin{equation}
% \mb{x}_d(t) = \BEZC\left(\frac{t-\underline{t}}{\overline{t}-\underline{t}}\right),    
% \end{equation}
% is a dynamically admissible trajectory 
% The function $\x_d(t) = \begin{pmatrix} \BEZc(t)&\cdots&\BEZc^{(\gamma)}(t)\end{pmatrix}$ is a dynamically admissible trajectory for the system \ref{eqn:openloop_state} with $\x_d(0) = \x_0$.
% \end{proposition}


% \begin{remark}
% Observe that any trajectory that satisfies the integrator structure in \eqref{eqn:openloop_state} is a dynamically admissible trajectory, as we can always choose an appropriate $u_d$. Additionally, note that there is no restriction on where $\x_k$ can be placed in order for the trajectory to be dynamically admissible. These are both properties of full state feedback linearizable systems. 
% \end{remark}

% Next, consider the matrix $\BEZ = \begin{bmatrix}\Bez_{0} & \ldots & \Bez_{n-1}\end{bmatrix}\in\mathbb{R}^{p+1\times n}$, whose rows $\BEZ_i\in\mathbb{R}^n$ correspond to the control points in state space.  B\'ezier curves enjoy a number of desirable properties; notably, the curve $\BEZC(\tau)$ is contained by the convex hull of the control points, i.e. $\BEZC(\tau) \in \text{conv}(\{\BEZ_i\})$ for $i=0,\ldots p$ and $\tau\in[0,1]$ \cite{BezierBook}. This key property will lay the foundation for the state and input constraint satisfaction guarantees that will be made.


% In this work we assume a fixed and uniform temporal distribution of control points.

% \begin{proposition}
% \label{prop:dynFeasTraj}
% The function $\x_d(t) = \begin{pmatrix} \BEZc(t)&\cdots&\BEZc^{(\gamma)}(t)\end{pmatrix}$ is a dynamically admissible trajectory for the system \ref{eqn:openloop_state} with $\x_d(0) = \x_0$.
% \end{proposition}
% \ifextended
% \begin{proof}
% Let $\mb u(t) = \mathcal{G}^\dagger(\x_d(t))(-\mathcal{F}(\x_d(t)) + \R^{(\gamma)}(t))$; then, it is clear that $\x_d(t)$ is a dynamically admissible trajectory, as it satisfies the dynamics in \eqref{eqn:etadotdecomp}. Furthermore, by observing that $\BEZc^{(\gamma)}(0)$ was exactly set to be $\state^{(\gamma)}(0)$ through the construction of $\mb D$, the initial condition is also met.
% \end{proof}
% \fi

% \NCS{I want $\mb e$ to be a state. Fight me. I want to be able to use $\RobustInvariant$ without needing to discuss time.}
% \subsection{State Bounds}
% Due to the convex hull property of the Bezi\'er polynomials, state constraints only need to be enforced on the control points $\BEZ_i$ of the curve $\BEZC$. This can also be argued in the robust case, as described in the following lemma:

% Define the function $\ErrorSet:\R^{n}\times\R_{\geq 0}\to\mathcal{P}(\R^n)$ as:
% \begin{equation}
%     \ErrorSet(\bs{\zeta},w) = \{ \mb{v}\in\R^n ~|~ (\mb{v}-\bs{\zeta})^\top\mb{P}(\mb{v}-\bs{\zeta}) \leq \gamma w^2\}. 
% \end{equation}



% $\BEZ_i\in\mathcal{X} \ominus \E \iff \BEZ_i$ satisfies $\mb L^T\BEZ_i \le \bs \ell-\sqrt{2}\lambda \mb L^T \mb P^{-1}\mb L$ for $\mathcal{X} = \{\x \in \R^n : \mb L\x \leq \ell\}$ where $\lambda=\gamma\overline{w}^2$ comes from the ISS property of the low-level controller \ref{clf-qp}, as in \eqref{eqn:robustInvariant}.

% In fact, under the assumption \ref{ass:polytopes} the above condition simply adds linear inequality constraints to the MPC program:
% \begin{lemma}
% $\bs b\in\mathcal{X} \ominus \E \iff \bs b$ satisfies $L^T\bs b \le \bs \ell-\sqrt{\gamma} \frac{\mb L^T \mb P^{-1}\mb L}{\sqrt{\mb L^T \mb P^{-1}\mb L}}$ for $(\mb L,\mb \ell)$ defining $\mathcal{X}$ where $\gamma=\frac{1}{2\lambda^2} \mb L^\top \mb P^{-1} \mb L$ and $\lambda$ comes from ISS.
% \end{lemma}

%%%%%%%%
% In order to provide guarantees for the inter-MPC sample times, the disparity between continuous control and discrete planning must be reconciled. The following section introduces B\'ezier polynomials as they are used in addressing this issue, and presents the MPC program that is employed by the planning layer to achieve Problem \ref{prob:IVP}. 

%
% \begin{assumption}
% \label{ass:FSFL}
% The system \eqref{eqn:openloop_state} is full state feedback linearizable.
% \end{assumption}
% \begin{assumption}
% The sets $\mathcal{X}$ and $\mathcal{U}$ are compact and contain the origin in their interior. Additionally, $\mathcal{W}$ is compact, and contains the origin. 
% % \AT{$\mathcal{D}$ can't be compact, its open.} \NCS{Sorry, I was using $\mathcal{D}$ as the disturbance set.}
% % Will need state constraint set $\mathcal{X}$ to be compact.
% \end{assumption}
%

% \ifextended
% \begin{align*}
%     {\R}^{(\gamma)}(\tau) = \Bez {\underbrace{(\mb R \mb S)}_{\mb H}}{}^\gamma  \z (\tau)
% \end{align*}
% where $\mb R \in \mathbb{R}^{p+1\times p+1}$ is defined by:
% \begin{align*}
%     \mb R_{ii} = \frac{p+1-i}{p}, ~~ \mb R_{i+1,i} = \frac{i}{p}
% \end{align*}
% and $\mb S \in \mathbb{R}^{p+1\times p+1}$ by:
% \begin{align*}
%     \mb S_{ii} = -p, ~~\mb S_{i,i+1} = p
% \end{align*}
% for $i=\{0,\ldots,p-1\}$ with all other entries zero \cite{noauthor_primer_2013}. The matrix $\mb S$ simply comes from the equation for differentiating B\'{e}zier curves, and the matrix $\mb R$ from increasing the order of the curve by one.
% \else

% where $\mb H\in\mathbb{R}^{p+1\times p+1}$ is the product of the matrix for differentiating the B\'ezier curve and the matrix for increasing its order by one \cite{noauthor_primer_2013}.
% \fi
%
% where $\mb H\in\mathbb{R}^{p+1\times p+1}$ is defied by:
% \begin{align*}
%     \begin{cases}\mb H_{i,i} = p-2i &\forall i\in\{0,\dots,p\}\\
%     \mb H_{i,i+1} = p-i &\forall i\in\{0,\dots,p-1\}\\
%     \mb H_{i+1,i} = -(i+1) &\forall i\in\{0,\dots,p-1\}.
%     \end{cases}
% \end{align*}
% Note that the matrix $\mb H$ is nilpotent, i.e. ${\mb H}^m\equiv \mb 0$ for $m>p$, as B\'ezier curves have zero derivative for all derivatives greater than $p$.
%

==> 4_InputConstraints.tex <==
\section{Input Constraints}
\label{sec:input}

In this section, we present the second main contribution of this work. We show how the structure of a low-level tracking controller can be used to place requirements on a dynamically admissible trajectory $\mb{x}_d$ to ensure input constraint satisfaction.

We will make the following assumption regarding input constraints for the system:

\begin{assumption}
\label{ass:inputpolytope}
The input constraint set $\mathcal{U}\subset\R$ is given by $\mathcal{U}=[-u_{\rm max}, u_{\rm max}]$ for some $u_{\rm max}\in\mathbb{R}_{>0}$.
\end{assumption}

Neither of the controllers $k_{\mb{x}_d}^{\rm fbl}$ or $k_{\mb{x}_d}^{\rm clf}$ are necessarily required to take values in the set $\mathcal{U}$. Thus, satisfying input constraints may require violating the inequality constraint in \eqref{eqn:cntrllyapreq}, potentially invalidating the claim that $\bs{\varphi}(t)\in\RobustInvariant_{\mb{x}_d}(t,\overline{w})$ for all $t\in\tintc$. To address this limitation, knowledge of how much control action is required by the controller to track the reference trajectory under disturbances should be incorporated when synthesizing $\mb{x}_d$.

To this end, we state the following definitions. For $\alpha,\beta\in\R_{\geq 0}$, define the matrix $\mb{M}_{\alpha,\beta}\in\mathbb{S}_{\succeq 0}^2$ and the functions $\mb{N}_{\alpha,\beta}:\mathcal{X}\to\R^2_{\geq 0}$ and $\Gamma_{\alpha,\beta}:\mathcal{X}\to\R_{\geq 0}$ as:
\begin{align}
    \mb{M}_{\alpha,\beta} &= \bs{\pi}_{\rm PSD}\left(\begin{bmatrix}2\alpha\beta & \beta \\ \beta & 0 \end{bmatrix} \right), \\
    \mb{N}_{\alpha,\beta}(\overline{\mb{x}}) &= \begin{bmatrix} 2\alpha\beta\overline{e}+\alpha\vert g(\overline{\mb{x}})^{-1}\vert+\beta\Vert\mb{K}\Vert_2\overline{e} \\
    \vert g(\overline{\mb{x}})^{-1}\vert + \beta\overline{e} \end{bmatrix}, \\
    \Gamma_{\alpha,\beta}(\overline{\mb{x}}) &=\overline{e}(\beta\overline{e}+\vert g(\overline{\mb{x}})^{-1} \vert)(\alpha+\Vert\mb{K}\Vert_2),
\end{align}
where $\bs{\pi}_{\rm PSD}:\mathbb{S}^2\to\mathbb{S}^2_{\succeq 0}$ denotes the projection from symmetric matrices to symmetric positive semidefinite matrices, $\overline{e} \triangleq \sqrt{\gamma\overline{w}^2 / \lambda_{\rm min}(\mb P)}$, and $\mb{K}$ is defined in \eqref{eqn:FBL_CL_gain}. Given these definitions, we state one of our main results (proven in \cite{csomay2022multirate_extended}):

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{Figures/MethodFig.pdf}
%     \caption{A depiction of the proposed method, where the control points of the B\'ezier curve are constraint tightened by the size of the robust invariant tube coming from the low level controller.}
%     \label{fig:BoundDepiction}
% \end{figure}

\begin{theorem}
\label{thm:fbl_bound}
There exists constants $\underline{\alpha},\underline{\smash{\beta}}\in\R_{\geq 0}$ such that if $\alpha\geq\underline{\alpha}$, $\beta\geq\underline{\smash{\beta}}$, and $\Omega_{\mb{x}_d}(t,\overline{w})\subseteq\mathcal{X}$ for all $t\in[\underline{t},\overline{t}]$, then for any collection of points $\{\overline{\mb{x}}_k\}$ with $\overline{\mb{x}}_k\in\mathcal{X}$ for $k = 0,\ldots,N-1$, we have that for all $t\in[t_k,t_{k+1})$:
\begin{align}
    \label{eqn:M_eq}
    \| k_{\mb{x}_d}^{\textnormal{fbl}}(\state,t)\|_2 \le   
    \frac{1}{2}\bs \sigma_{\mb{x}_d}(t)^\top &{\mb{M}}_{\alpha,\beta}\bs \sigma_{\mb{x}_d}(t)  \\+& {\mb{N}}_{\alpha,\beta}(\overline{\mb{x}}_k)^\top \bs \sigma_{\mb{x}_d}(t) + {\Gamma}_{\alpha,\beta}(\overline{\mb{x}}_k), \nonumber
\end{align}
for all $\mb{x}\in \Omega_{\mb{x}_d}(t,\overline{w})$, where $\bs \sigma_{\mb{x}_d}:\tintc\to\R_{\geq 0}^2$ is defined as:
\begin{align}
   \bs \sigma_{\mb{x}_d}(t) &= \begin{bmatrix}
    \|\mb{x}_d(t)-\overline{\state}_k\|_2 \\
    \|\dot{x}_d^n(t)- f(\overline{\state}_k)\|_2
    \end{bmatrix}, \quad t\in[t_k,t_{k+1}).  \label{eqn:s_def}
\end{align}
\end{theorem}

This result is motivated by the key observation that the upper bound achieved in \eqref{eqn:M_eq} is convex in the quantity $\bs \sigma_{\mb{x}_d}(t)$ for each $t\in\tintc$, such that the constraint:
\begingroup\makeatletter\def\f@size{9}\check@mathfonts
\begin{align}
    \frac{1}{2}\bs \sigma_{\mb{x}_d}(t)^\top {\mb{M}}_{\alpha,\beta}\bs \sigma_{\mb{x}_d}(t) + {\mb{N}}_{\alpha,\beta}(\overline\state_k)^\top \bs \sigma_{\mb{x}_d}(t) + {\Gamma}_{\alpha,\beta}(\overline\state_k) &\le u_{\rm max}. \label{eqn:M_ineq_desired}
\end{align}
\endgroup
is a convex quadratic inequality constraint in the quantity $\bs \sigma_{\mb{x}_d}(t)$. Given that the function $\bs \sigma_{\mb{x}_d}$ is defined by B\'{e}zier control points, we seek to translate this constraint into one on control points.

\begin{remark}
We note that the proof of Theorem \ref{thm:fbl_bound} in \cite{csomay2022multirate_extended} establishes the existence of values of $\underline{\alpha}$ and $\underline{\smash{\beta}}$ through Lipschitz properties of the dynamics. In practice, it may be difficult to compute these values, and they may not necessarily be the minimum values for which this result holds. Moreover, choosing very large values of $\alpha$ and $\beta$ may lead to conservative behavior, as the constraint in \eqref{eqn:M_ineq_desired} will constrain the dynamically admissible trajectory $\mb{x}_d$ to a small neighborhood of $\overline{\mb{x}}_k$. These issues are not unexpected, as the challenge of input constraint satisfaction for general nonlinear systems is known to be quite difficult. Instead, with this result we seek to highlight an important monotonic structural property of the system that permits a well-posed and practical approach for achieving input constraint satisfaction. In particular, one may begin with small values of $\alpha$ and $\beta$ and increase them until the closed-loop nonlinear system meets input constraints. We will demonstrate this type of procedure in Section \ref{sec:sim}. 
\end{remark}


Before relating Theorem \ref{thm:fbl_bound} to the B\'{e}zier control points defining $\mb{x}_d$, we state the following lemma (proven in \cite{csomay2022multirate_extended}):
\begin{lemma}
\label{lem:eq_bound}
For any $\x\in\mathbb{R}^n$, we have that:
\begin{align}
\|\BEZC_k(\tau) - \x\|_2 &\le {\sup}_{i}\|(\BEZ_k)_i-\x\|_2, \\
\|\BEZc_k^{(n)}(\tau) - f(\x)\|_2 &\le {\sup}_{i}\|(\bez_k)_{n,i}-f(\x)\|_2,
\end{align}
for all $\tau\in[0,T]$. 
\end{lemma}

With this result, we now state one of our main results (proven in \cite{csomay2022multirate_extended}) for tractably enforcing input bounds:

\begin{lemma}
\label{lem:input_bounds}
If given a collection of points $\{\overline{\mb{x}}_k\}$ with $\overline{\mb{x}}_k\in\mathcal{X}$ for $k = 0,\ldots,N-1$, there exists $\mb{s}_k\in\R^2_{\geq 0}$ such that:
\begin{align}
    \label{eqn:s_ineq}
  \begin{bmatrix}\|(\BEZ_k)_i - \overline{\mb{x}}_k\|_2 \\ \|(\bez_k)_{n,i}- f(\overline{\mb{x}}_k)\|_2\end{bmatrix} &\le {\mb s}_k,  \\ \label{eqn:t_ineq}
    \frac{1}{2}\mb s_k^\top {\mb{M}}_{\alpha,\beta}\mb s_k + {\mb{N}}_{\alpha,\beta}(\overline{\state}_k)^\top \mb s_k + {\Gamma}_{\alpha,\beta}(\overline{\state}_k) &\le u_{\rm max},
\end{align}
for $i=0,\ldots,2n-1$ and $k=0,\ldots,N-1$, then we have that the inequality \eqref{eqn:M_ineq_desired} is satisfied with $\bs \sigma_{\mb{x}_d}(t)$ defined as in \eqref{eqn:s_def} for all $t\in\tintc$. 
\end{lemma}
A consequence of this result is that for sufficiently high values of $\alpha$ and $\beta$, meeting the conditions of Lemma \ref{lem:input_bounds} implies $\| k_{\mb{x}_d}^{\rm fbl}(\mb{x},t)\|_2 \leq u_{\rm max}$ for all $t\in\tintc$ and $\mb{x}\in\Omega_{\mb{x}_d}(t,\overline{w})$. Moreover, the constraint \eqref{eqn:s_ineq} is a second-order cone constraint and the constraint \eqref{eqn:t_ineq} is a convex quadratic constraint (which may be reformulated as a second-order cone constraint, see \cite{csomay2022multirate_extended}), and thus they may be incorporated into a convex program for determining B\'{e}zier control points. Lastly, we state the following corollary relating bounds on $k_{\mb{x}_d}^{\rm fbl}$ and $k_{\mb{x}_d}^{\rm clf}$:

\begin{corollary}
\label{cor:kclfbd}
If the function $k^{\rm fbl}_{\mb{x}_d}$ is bounded as in \eqref{eqn:M_eq} for all $t\in[t_k,t_{k+1})$ and $\mb{x}\in\Omega_{\mb{x}_d}(t,\overline{w})$, then we have that:
\begin{align}
    \label{eqn:M_eqclf}
    \| k_{\mb{x}_d}^{\textnormal{clf}}(\state,t)\|_2 \le   
    \frac{1}{2}\bs \sigma_{\mb{x}_d}(t)^\top &{\mb{M}}_{\alpha,\beta}\bs \sigma_{\mb{x}_d}(t)  \\+& {\mb{N}}_{\alpha,\beta}(\overline{\mb{x}}_k)^\top \bs \sigma_{\mb{x}_d}(t) + {\Gamma}_{\alpha,\beta}(\overline{\mb{x}}_k), \nonumber
\end{align}
for all $t\in[t_k,t_{k+1})$ and all $\mb{x}\in\Omega_{\mb{x}_d}(t,\overline{w})$.
\end{corollary}

% \AT{
% \begin{theorem}
% Let $\BEZC:[0,T]\to\mathcal{X}$ be a dynamically admissible trajectory for the system \eqref{eqn:openloop_state} such that $\Omega(t,\overline{w})\subseteq\mathcal{X}$ for all $t\in[0,T]$, and let $\Bez_i$ and $\BEZ_i$ denote its associated control points and state space control points, respectively, for $i=1,\ldots,p$. Furthermore, let $\overline{\mb{x}}\in\mathcal{X}$. For sufficiently large $\alpha, \beta\in\R_{\ge0}$, if the following second order cone constraints are enforced:
% \label{thm:input_bounds}
% \begin{align}
%     \label{eqn:s_ineq}
%     \sup_{i\in\{0,\ldots,p\}}\begin{bmatrix}\|\BEZ_i - \bar{\state}\|_2 \\ \|\bez_{n,i}- f(\bar{\state})\|_2\end{bmatrix} &\le {\mb s}  \\
%     \frac{1}{2}\mb s^\top {\mb{M}}_{\alpha,\beta}\mb s + {\mb{N}}_{\alpha,\beta}(\bar\state) \mb s + {\Gamma}_{\alpha,\beta}(\bar\state) &\le u_{max}.
% \end{align}
% % then we have that:
% % \begin{align*}
% %     % \|k_{\textnormal{clf}}(\mb\state, t)\|_2 \le u_{max}.
% %     u(t) = k_{\textnormal{clf}}(\mb\state, t)\in\mathcal{U},~~~\forall t\in\tintc.
% % \end{align*}
% \end{theorem}}


% The set $\mathcal{U}\subset\R$ is a compact, convex polytope, and contain the origin in their interior.
% The set $\mathcal{U}=[-u_{max}, u_{max}]\subset\R$ is a compact and contains the origin in its interior.

% Towards this goal, let $\bar{e}\triangleq\sqrt{\gamma\overline{w}^2 / \lambda_{\rm min}(\mb P)}$, and for notational simplicity, $g^\dagger:\R^n\to\R$ is defined as $g^\dagger(\mb{x}) = g(\mb{x})^{-1}$.
% %
% % Furthermore, let $L_f$, and $L_{g^\dagger}\in\R_{\geq 0}$ represent the Lipschitz constants of $f$ and $g^\dagger$, respectively, 
% %
% Then, given constants $\alpha, \beta \ge 0$, we define ${\mb M}_{\alpha,\beta}\in\mathbb{S}^{2\times 2}$, ${\mb N}_{\alpha,\beta}:\mathcal{X}\to\mathbb{R}_{\ge0}^{2}$, and ${\Gamma}_{\alpha,\beta}:\mathcal{X}\to\mathbb{R}_{\ge0}$ as:
% \begin{align*}
%   {\mb M}_{\alpha, \beta} &= \pi_{PSD}\left(\begin{bmatrix} 2\alpha\beta & \beta\\\beta&0\end{bmatrix}\right)\\
%     % \widetilde{\mb{M}}_\pi(\alpha, \beta) &= \beta\begin{bmatrix} \delta^3 & \delta^2\\\delta^2&\delta\end{bmatrix},
%     % ~~~~\delta = \alpha + \sqrt{1+\alpha^2} \\
%     % \mb{\tilde{M}} &= \beta\begin{bmatrix} (\alpha+\sqrt{1+\alpha^2})^3 & (\alpha+\sqrt{1+\alpha^2})^2\\(\alpha+\sqrt{1+\alpha^2})^2&\alpha+\sqrt{1+\alpha^2}\end{bmatrix}\\
%     {\mb N}_{\alpha, \beta}(\bar \x) &= \begin{bmatrix} 2\alpha\beta\bar{e} +\beta\|g^{\dagger}(\bar\state)\|_2+\alpha\|\mb{K}\|_2\bar{e} \\ \|g^{\dagger}(\bar\state)\|_2 +\alpha\bar{e} \end{bmatrix}^\top \\
%     {\Gamma}_{\alpha, \beta}(\bar \x) &= {\bar{e}}(\alpha{\bar{e}}+\|g^{\dagger}(\bar\state)\|_2)(\beta+\|\mb{K}\|_2). 
% \end{align*}
% where $\pi_{PSD}:\mathbb{S}^2\to\mathbb{S}_{\ge0}^2$ is the unique projection onto the positive semidefinite cone. With these, we have the following statement:

% \begin{theorem}
% \label{lem:fbl_bound}
% Let $\mb{x}_d:\tintc\to\mathcal{X}$ be a dynamically admissible trajectory for the system \eqref{eqn:openloop_state} such that $\Omega(t,\overline{w})\subseteq\mathcal{X}$ for all $t\in[\underline{t},\overline{t}]$, and let $\overline{\mb{x}}\in\mathcal{X}$. There exists functions $\mb{M}:\R_{\geq 0}\times\R_{\geq 0}\to\mathbb{S}_{\succeq 0}^2$, $\mb{N}:\mathcal{X}\times\R_{\geq 0}\times\R_{\geq 0}\to\R^2_{\geq 0}$, and  $\Gamma:\mathcal{X}\times\R_{\geq 0}\times\R_{\geq 0}\to\R_{\geq 0}$, and constants $\underline{\alpha},\underline{\smash{\beta}}\in\mathbb{R}_{\ge 0}$ such that if $\alpha\geq\underline{\alpha}$ and $\beta\geq\underline{\smash{\beta}}$, then for almost all $t\in\tintc$:
% \begin{align}
%     \label{eqn:M_eq}
%     \|k_{\textnormal{fbl}}(\state,t)\|_2 \le &  
%     \frac{1}{2}\mb s^\top {\mb{M}}(\alpha,\beta)\mb s \nonumber \\ & + {\mb{N}}(\bar\state,\alpha,\beta)^\top \mb s + {\Gamma}(\bar\state,\alpha,\beta),
% \end{align}
% for all $\mb{x}\in \Omega(t,\overline{w})$, where:
% \begin{align}
%   \mb s &= \begin{bmatrix}
%     \|\mb{x}_d(t)-\bar{\state}\|_2 \\
%     \|\dot{x}_d^n(t)- f(\bar{\state})\|_2
%     \end{bmatrix}.  \label{eqn:s_def}
% \end{align}
% \end{theorem}

% Given a maximum allowable control input, we would like to enforce a limit on the amount of control action required by the low level controller. Lemma \ref{lem:fbl_bound} hints at how we can achieve this -- namely, through upper bounding the expression in \eqref{eqn:M_eq}:
% \begin{align}
%     \frac{1}{2}\mb s^\top {\mb{M}}_{\alpha,\beta}\mb s + {\mb{N}}_{\alpha,\beta}(\bar\state) \mb s + {\Gamma}_{\alpha,\beta}(\bar\state) &\le u_{max}. \label{eqn:M_ineq_desired}
% \end{align}
%
% \begin{corollary}
% \label{cor:clf_flb}
% Under the same assumptions and the same forms for $\mb M$, $\mb N$, $\Gamma$, and $\mb s$ we have that:
% \begin{align}
%     \|k_{\textnormal{clf}}(\state,t)\|_2 &\le 
%     \frac{1}{2}\mb s^\top \mb M\mb s + \mb N(\bar\state)^\top \mb s + \Gamma(\bar\state),
% \end{align}
% for all $\mb{x}\in \Omega(t,\overline{w}).$
% \end{corollary}
% It is straightforward to see that $\mb{M}\succeq\widetilde{\mb{M}}$, such that:
% \begin{align*}
%     \|k_{\textrm{fbl}}(\mb{x},t)\|_2 &\leq \frac{1}{2}\mb s^\top \mb{M}\mb s + \mb N(\bar\state)^\top \mb s + \Gamma(\bar\state).
% \end{align*}
%
% Being able to enforce this constraint in practice will require a number of additional steps, the first of which is making this efficiently representable via convex programming. Because $\mb M$ 
%
% Although Lemma \ref{lem:fbl_bound} proves the existence of constants $\alpha$ and $\beta$, it provides little insight into how to synthesize them. As such, 
% % As we will only be able to enforce \eqref{eqn:M_ineq_desired} with the above functions, 
% we desire a monotonicity property for choices of $\alpha$ and $\beta$. This is summarized by the following statement:


% \begin{lemma}
% \label{lem:input_bounds}
% Take $\bar\state \in\mathcal{X}$, and $\mb s\in\R^2_{\ge0}$. Then, for all $\alpha \ge \underline{\alpha}$ and $\beta \ge \underline{\smash{\beta}}$:
% \begin{align*}
%     \|k_{\textnormal{clf}}(\bs \state, t)\| &\le \frac{1}{2}\bs s^\top {\mb{M}}^\pi_{\underline{\alpha},\underline{\smash{\beta}}}\bs s + {\mb{N}}_{\underline{\alpha},\underline{\smash{\beta}}}(\bar\state) \bs s + {\Gamma}_{\underline{\alpha},\underline{\smash{\beta}}}(\bar\state)\\
%     &\le \frac{1}{2}\bs s^\top {\mb{M}}^\pi_{\alpha,\beta}\bs s + {\mb{N}}_{\alpha,\beta}(\bar\state) \bs s + {\Gamma}_{\alpha,\beta}(\bar\state).
% \end{align*}
% \end{lemma}



% \begin{remark}
% The above theorem shows that the parameter $c$ can be used as a tuning knob, where the above formulation may exhibit desirable performance at small values of $c$, and past a certain value, i.e. past the Lipschitz constants of the system, theoretical guarantees are maintained.
% \end{remark}


% We begin to see the usefulness of B\'ezier curves: they allow us to bound the desired trajectory in continuous time by enforcing bounds on discrete points. This is demonstrated in the following proposition:


%  $\beta\geq\underline{\smash{\beta}}$, then for a dynamically admissible trajectory $\mb{x}_d:\tintc\to\mathcal{X}$ for the system \eqref{eqn:openloop_state} defined as in Lemma \ref{lem:bezdynadmistraj} from a collection of B\'{e}zier curves $\{r_k\}$, such that

% Let $\mb{x}_d$ be a dynamically admissible trajectory for the system \eqref{eqn:openloop_state} defined as in Lemma \ref{lem:bezdynadmistraj} from a collection of B\'{e}zier curves $\{r_k\}$, such that $\Omega(t,\overline{w})\subseteq\mathcal{X}$ for all $t\in\tintc$.

==> 5_MPC.tex <==
\section{Multi-Rate Control Architecture}
\label{sec:multirate}

Utilizing the developments presented in the previous sections, we now construct a multi-rate control architecture which iteratively produces dynamically admissible trajectories for the system \eqref{eqn:openloop_state} and tracks them with the low-level controller designed in Section \ref{sec:lowlevel}. Importantly, by achieving robustness to disturbances with the low-level controller, the trajectory planning algorithm can reason about a disturbance-free system.

% \begin{figure*}[t]
%     %  \centering
%      \includegraphics[width=0.8\linewidth]{Figures/Combined.png}
%      \caption{A depiction of the proposed method for increasing values of $\alpha$ and $\beta$. Notice that as the parameters increase, the planned MPC points become spatially closer so as to reduce the linearization error, and in doing so the deviation of the low level controller from the planned control input decreases. \red{CLF vs standard MPC with input held constant vs proposed}}
%      \label{fig:AlgoSim}
% \end{figure*}

\subsection{Model Predictive Control}
In this section we establish how to compute the collection of points $\{\mb{x}_k\}$ used to define $\mb{x}_d$ in Lemma \ref{lem:bezdynadmistraj} while meeting the desired constraints on the B\'{e}zier control points. Consider a collection of points $\{\overline\state_{k}\}$ with $\overline\state_{k}\in\mathcal{X}$ and $\{\overline u_{k}\}$ with $\overline{u}_{k}\in\R$ for $k=0,\ldots N-1$. To incorporate information about the system dynamics when synthesizing $\mb{x}_d$ as in Lemma~\ref{lem:bezdynadmistraj}, we will use linearizations of the system dynamics~\eqref{eqn:openloop_state} around these collections of points. This approximation of the dynamics will provide constraints on sequential state points (and the corresponding B\'{e}zier control points as defined by \eqref{eqn:bezsetctrlpts}) defining $\mb{x}_d$. 
We neglect the disturbances $\mb{w}$ in this approximation as the low-level controller rejects these disturbances and provides a robust invariant set around $\mb{x}_d$. More precisely, consider a linear, temporal discretization of \eqref{eqn:openloop_state}:
\begin{align}
    \label{eqn:linearizations}
    \state_{k+1} &= \A(\overline\state_{k}, \overline u_{k}) \state_{k} + \B(\overline\state_{k}) u_{k} + \C(\overline\state_{k}, \overline u_{k}),
\end{align}
where $\A:\mathcal{X}\times\R\to\R^{n\times n}, \B:\mathcal{X}\to\R^n$, and $\C:\mathcal{X}\times\R\to\R^n$ come from linearizing and taking the exact temporal discretization\footnote{See \cite{csomay2022multirate_extended} for a formula for these linearizations and discretizations.} (with sample period $T$) of the dynamics in \eqref{eqn:openloop_state}. For notational simplicity let us define:
\begin{align}
    \mb A_k \triangleq \mb A(\overline\state_k, \overline u_k),~~\mb B_k \triangleq \mb B(\overline\state_k),~~\mb C_k \triangleq \mb C(\overline\state_k, \overline u_k).
\end{align}
Given these, let us denote the state at a time $t\in\R_{\geq 0}$ by $\mb{x}(t)$. Building upon the previous two sections, we propose a Finite Time Optimal Control Problem (FTOCP):
\begin{subequations}
\begin{alignat}{2}
    \hspace{-1mm}\min_{\substack{u_{k}, \state_{k}\\ \mb s_{k}, \Bez_{k}}} \quad & \sum_{k=0}^{N-1} h(\state_{k},u_{k})  + J(\state_{N}) \label{eqn:FTOCP} \tag{FTOCP}\\
\textrm{s.t.}~ \quad & \state_{k+1} = \A_{k}\state_{k} + \B_{k}u_{k} + \C_{k}, \label{eqn:mpclindyn} \\
  & \state_{0} \in \state(t) \oplus \mathcal{E}, \label{eqn:mpcic}\\
  & \state_{N} = \mb{0}, \label{eqn:mpcterminal}\\ %\in \mathcal{X}_F,
  & (\Bez_k) = \begin{bmatrix} \x_{k}^\top &\x_{k+1}^\top \end{bmatrix}\mb{D}^{-1},\label{eqn:mpcbezdef} \\
  & (\BEZ_k)_i \in \mathcal{X} \ominus \E, \hspace{23.7mm} \forall i \in \mathcal{I} \label{eqn:mpccnvxhull}\\
  & \begin{bmatrix}\|(\BEZ_k)_i - \overline{\state}_{k}\|_2 \\ \|(\bez_k)_{n,i}- f(\overline{\state}_{k})\|_2\end{bmatrix} \le \mb s_{k}, \hspace{5mm} \forall i\in\mathcal{I} \label{eqn:mpcconic}\\
  & \frac{1}{2}\mb s_{k}^\top \mb{M}_{\alpha,\beta} \mb s_{k} + {\mb N}_{\alpha,\beta}(\overline \state_k)^\top \mb s_{k} \nonumber \\ & \qquad\qquad\qquad\qquad\qquad + {\Gamma}_{\alpha,\beta}(\overline \state_k) \le u_{\rm max}, \label{eqn:mpcquadratic}
  \end{alignat}
\end{subequations}
where $h:\mathcal{X}\times\R\to\R_{\geq 0}$ is a convex stage cost, $J:\mathcal{X}\to\R_{\geq 0}$ is a convex terminal cost, and $\mathcal{I} = \{0,\ldots,2n-1\}$.
%  and $\mathcal{X}_F\subseteq\mathcal{X}$ is a terminal constraint set.
The constraint in \eqref{eqn:mpclindyn} requires that the sequence of discrete points defining $\mb{x}_d$ satisfy a linear, discrete time approximation of the system dynamics. The constraint in \eqref{eqn:mpcic} requires that the beginning of $\mb{x}_d$ is close to the current state $\mb{x}(t)$, such that $\mb{x}(t)\in\Omega(t,\overline{w})$ as required by Lemma \ref{lem:lowleveliss}. The constraint in \eqref{eqn:mpcterminal} requires the end of $\mb{x}_d$ to be placed at origin. The constraints in \eqref{eqn:mpcbezdef}-\eqref{eqn:mpcquadratic} relate the discrete points $\mb{x}_k$ to B\'{e}zier control points, and consequently the continuous trajectory $\mb{x}_d$ tracked by the low-level controller. Note that as in Fact \ref{fct:cvxhull}, the coefficients $(\bs{\xi})_k$ and $(\bs{\zeta}_k)_i$ are linearly related for $i=0,\ldots,2n-1$, a constraint implicitly assumed in \eqref{eqn:FTOCP}. If $h$ and $J$ are positive definite quadratic functions, \eqref{eqn:FTOCP} is a second-order cone program (SOCP), which can be efficiently solved via standard solvers \cite{mosek}. 

\begin{remark}
Note that we do not explicitly enforce input constraints on the decision variables $u_k$. Instead, constraints are induced on these decision variables through the linear dynamics constraint \eqref{eqn:mpclindyn} and the constraints on the B\'{e}zier coefficients in \eqref{eqn:mpcbezdef} and \eqref{eqn:mpcconic}-\eqref{eqn:mpcquadratic}. Moreover, these constraints ensure that the low-level controller will satisfy input constraints as desired. 
\end{remark}


\subsection{The Multi-Rate Architecture}

\begin{algorithm}[b!]
%   \caption{Multi-Rate Scheme}\label{alg:mpc-fl}
  \caption{$u$ = C-MPC($\state, t$)\label{alg:mpc-fl}}
%   \hspace*{\algorithmicindent}
%   \textbf{Initialize:} $\textbf{Lin}_{-1} = [\A_o, \B_o, \C_{o}], \overline u_{-1} =\mb 0$
%   \textbf{Initialize:} \begin{align*}\A_{-1} &= \A_{origin},\\\R_{-1} &= \R_{origin},\\\C_{-1} &= \C_{origin}\\\overline \u_{-1} &=\mb 0\end{align*}
%   \hspace*{\algorithmicindent} \textbf{Output} 
  \begin{algorithmic}[1]
    % \Procedure{MPC-CLF-Execution}{$\x(t)$} 
    % \If {$t\in\mathcal{T}=\cup_{\mpcindex=0}^\infty\{\mpcindex T\}$}
    \If {$t\in\mathcal{T}=\cup_{\mpcindex=0}^\infty\{\mpcindex T\}$}
        \State Compute $\{\textbf{Lin}_{k|\mpcindex}\}$ in \eqref{eqn:linearizations} about $\{\overline{\x}_{k|\mpcindex}\}$ and $\{\overline u_{k|\mpcindex}\}$;
        \State Solve \eqref{eqn:FTOCP} with $\{\textbf{Lin}_{k|\mpcindex}\}$;
        \If {\eqref{eqn:FTOCP} is infeasible}
        \State $\{\textbf{Lin}_{k|\mpcindex}\} \leftarrow \{\textbf{Lin}_{1|\mpcindex-1},\ldots,\textbf{Lin}_{N-1|\mpcindex-1},\textbf{Lin}_{O}\};$
        % [\textbf{Lin}_{1|\mpcindex-1},\ldots,\textbf{Lin}_{N-1|\mpcindex-1}, \textbf{Lin}_{N|\mpcindex-1]};$
        \State Solve \eqref{eqn:FTOCP}  with $\{\textbf{Lin}_{k|\mpcindex}\}$;
        % \Else
        % \State Jubilee
        \EndIf
        \State $\{\overline\x_{k|\mpcindex+1}\} \leftarrow \{\x_{1|\mpcindex}^*,\ldots,\x^*_{N-1|\mpcindex},\x^*_{N|\mpcindex}\}$;
        \State $\{\overline u_{k|\mpcindex+1}\} \leftarrow \{ u_{1|\mpcindex}^*,\ldots, u_{N-1|\mpcindex}^*,0\}$;
    \EndIf
    \State Calculate $\x_d | \mpcindex$ from $\{\mb x_{k|\mpcindex}^*\}$, as in \eqref{eqn:bezsetctrlpts}--\eqref{eqn:dyn_admissible_traj};
    % \State Compute feedforward $\u_{\textrm{ff}}=\k_{\textrm{ff}}(\x(t), \x_d^*(t), \u_d^*(t))$;
    % \State Compute total input $u(t) = \u_{CLF}(\x(t), t)$;
    \State \Return $u = k^{\textrm{clf}}_{\state_{d}|\mpcindex}(\x, t)$;
    % \Return $u(t) = k_{\textrm{CLF}}(\x(t), \x_d^*(t), \u_d^*(t))$;
    % \EndProcedure
  \end{algorithmic}
\end{algorithm}

We now present the multi-rate architecture that integrates the low-level controller design posed in Section \ref{sec:lowlevel} with the preceding trajectory planner encoded in \eqref{eqn:FTOCP}.

We first recall the role $T$ plays in dynamically admissible trajectories synthesized through B\'{e}zier curves as in Lemma \ref{lem:bezdynadmistraj}, as well as its role as a sampling period for the temporal discretization established in \eqref{eqn:linearizations}. Let us denote $\mathcal{T}=\cup_{\mpcindex=0}^\infty\{\mpcindex T\}$. This set serves to index the discrete points in time (separated by $T$) at which a dynamically admissible trajectory for the system will be replanned by solving the \eqref{eqn:FTOCP}. The multi-rate architecture is initialized at time $t=0$ with collections of points $\{\overline{\mb{x}}_{k|0}\}$ and $\{\overline{u}_{k|0}\}$ with $\overline{\mb{x}}_{k|0}\in\mathcal{X}$ and $\overline{u}_{k|0}\in\R$ for $k=0,\ldots,N-1$. Let us denote the linearized and discretized dynamics computed around these collections by $\{\textbf{Lin}_{k|0}\} = \{(\mb{A}_{k|0},\mb{B}_{k|0},\mb{C}_{k|0})\}$.
\begin{assumption}
Given an initial condition $\mb{x}(0)\in\mathcal{X}$, \eqref{eqn:FTOCP} is feasible using $\{\textbf{Lin}_{k|0}\}$. 
\end{assumption}

We now describe our multi-rate framework as summarized in Algorithm \ref{alg:mpc-fl}. As in Line 1, let $t\in\mathcal{T}$ such that $t=iT$ for some $i\in\mathbb{Z}$. In Line 2, the linearized and discretized dynamics are computed around the collections $\{\overline{\mb{x}}_{k|i}\}$ and $\{\overline{u}_{k|i}\}$, and are denoted by $\{\textbf{Lin}_{k|i}\} = \{(\mb{A}_{k|i},\mb{B}_{k|i},\mb{C}_{k|i})\}$. In Line 3 these dynamics are used to solve the \eqref{eqn:FTOCP} using the state at the current time, $\mb{x}(t)$, in \eqref{eqn:mpcic}. If the \eqref{eqn:FTOCP} is feasible, it returns collections of points $\{\mb{x}^*_{k|i}\}$ with $\mb{x}^*_{k|i}\in\mathcal{X}$ for $k=0,\ldots, N$ and $\{u^*_{k|i}\}$ with $u^*_{k|i}\in\R$ for $k=0,\ldots, N-1$. If \eqref{eqn:FTOCP} is infeasible, in Line 5 we set the linearized and discretized dynamics $\{\textbf{Lin}_{k|i}\}$ to the previous linearization shifted by one and appending the linearization and discretization around the origin, denoted $\textbf{Lin}_O = (\mb{A}(\mb{0},0),\mb{B}(\mb{0}),\mb{C}(\mb{0},0))$. In Line 6 we solve \eqref{eqn:FTOCP} and similarly return collections of points $\{\mb{x}^*_{k|i}\}$ and $\{u^*_{k|i}\}$. As we will show in Theorem \ref{thm:TheBigCahoona}, our assumption about feasibility at time $t=0$ will ensure that switching to this set of linearizations will always ensure \eqref{eqn:FTOCP} is feasible. In Line 8--9 the collection $\{\mb{x}^*_{k|i}\}$ is shifted and the collection $\{u^*_{k|i}\}$ is shifted and appended with $0$ to define collections $\{\overline{\mb{x}}_{k|i+1}\}$ and $\{\overline{u}_{k|i+1}\}$ used for linearization and discretization in the next iteration. In Line 11 the collection $\{\mb{x}^*_{k|i}\}$ is then used to define a dynamically admissible trajectory $\mb{x}_d|i$ as in Lemma \ref{lem:bezdynadmistraj}, which yields a corresponding low-level controller  $k^{\textrm{clf}}_{\state_{d}|\mpcindex}$ that defines the output of our algorithm. We may view our algorithm as a time-varying controller that yields a closed-loop system \eqref{eqn:closedloop_state}. Importantly, our algorithm ensures state and input constraints are satisfied as the continuous time system evolves under this controller, as stated in the following theorem (proven in \cite{csomay2022multirate_extended}): 

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{Figures/Combined_v3.pdf}
    \caption{Comparison of three control methods: only using a low level controller (CLF), applying MPC with no low-level controller, and applying the proposed C-MPC with a CLF at the low-level. In both scenarios, just using the low-level or mid-level controller separately yields both state and input violation.}
    \label{fig:comparison}
\end{figure}

\begin{theorem}
\label{thm:TheBigCahoona}
Suppose that $\alpha\geq\underline{\alpha}$ and $\beta\geq\underline{\smash\beta}$ are such that $\Gamma_{\alpha,\beta}(\mb{0})\leq u_{\rm max}$. Let \eqref{eqn:FTOCP} be defined with $\alpha$ and $\beta$, and consider the closed-loop system \eqref{eqn:closedloop_state} with a feedback controller given by C-MPC in Algorithm \ref{alg:mpc-fl} and a disturbance signal satisfying $\Vert\mb{w}\Vert_{\infty}\leq\overline{w}$. If $\mb{0}\in\mathcal{X}\ominus\ErrorSet$ and \eqref{eqn:FTOCP} is feasible at $t_0=0$ with initial condition $\mb{x}(0)\in\mathcal{X}$, then C-MPC is well-defined for all time, and the closed-loop system \eqref{eqn:closedloop_state} satisfies state and input constraints.
\end{theorem}


% This state-input sequences should not necessary be dynamically feasible and they will affect the Region of Attraction.
% Here we state the multi-rate control architecture as it is used to achieve Problem \ref{prob:StateAndInput}, as is summarized in Algorithm \ref{alg:mpc-fl}. In continuous-time, the \ref{clf-qp} is run, termed the ``low-level" controller, as it is the controller sending input values to the dynamical system. 

% Notice that, if at time $t=0$ the (FTOCP) is not feasible, Algorithm~\ref{alg:mpc-fl} solves an (FTOCP) using the matrices $\A_{\text{origin}}, \B_{\text{origin}}$, and $\C_{\text{origin}}$ that are computed linearizing the system around the origin. Therefore, an inner approximation of the RoA associated with the proposed algorithm is given by the set of states from which the (FTOCP) with matrices $\A_{\text{origin}}, \B_{\text{origin}}$, and $\C_{\text{origin}}$ is feasible. Such regions can be computed explicitly as it is the feasible set of a convex optimization problem.



% In order to generate an initial trajectory, the low-level CLF controller can be simulated forward to generate a collection $(\mb x, \mb u)$, which may not satisfy state or input constraints. Then, the \eqref{eq:mpc} can be run, which if successful would provide a feasible trajectory at time step $0$ that could be used for recursive feasibility. 
% \red{here should go a discussion of how to produce feasible reference trajectories at time step 0, and how to construct robust invariants if you like (i.e. linearizing about the origin and calculating backward reachability) if you like}


% \begin{remark}
%  The terminal constraint set in (FTOCP) is a 
% \end{remark}

% Then, the policy at the low level is given by 
% \begin{align*}
    % u(t) = u^*_{t_k|\tau_k} + k_{NL}(x(t))~\forall t\in[t_k,t_{k+1})
% \end{align*}



% \begin{theorem}
% There exists an $a,b,c\in\mathbb{R}$ such that for all $a < \alpha$ and $b < \beta$, and $c<\gamma$, $\frac{1}{2}\bs t^\top \mb M(L_{\mathcal{G}^\dagger},L_{\bs f_{\bs \eta}})\bs t + \mb N(L_{\mathcal{G}^\dagger},L_{\bs f_{\bs \eta}}) \bs t \le \frac{1}{2}\bs t^\top \mb{\tilde{M}}(\alpha,\beta)\bs t + \mb N(\alpha,\beta) \bs t $ for all $\mb t\in\mathbb{R}^2$.
% \end{theorem}
% \begin{proof}
% \end{proof}


% \begin{theorem}
% The MPC program in \eqref{eq:mpc} satisfies state and input constraints for all time and for all disturbances.
% \end{theorem}

% \begin{lemma}
% The constraint in \eqref{eqn:M_ineq} would lead to the same optimal value as the constraint in \eqref{eqn:M_eq}.
% \end{lemma}
% \ifextended
% \begin{proof}
% Consider a feasible point $\bs\eta_d(t)$ for \eqref{eqn:M_eq} with associated control points $\mb b$. By proposition (?), we know that we can upper bound the path norm by the supremum over the control points
% \end{proof}
% To write the program as an SOCP, the second constraint can be written as:
% \begin{align*}
    % \|\tilde{\mb{M}}^{1/2}\mb t + \frac{1}{2}\tilde{\mb{M}}^{-1/2}\mb N\| \le \left(\frac{1}{4}N^\top \tilde{\mb{M}}^{-1}\mb N +u_max\right)^{\frac{1}{2}}.
% \end{align*}
% \fi
% \begin{lemma}
% \label{lem:stat_and_input}
% Given $\mb b_k^*(t)$ and $\mb u_k^*(t)$ from \ref{eqn:mpc}, $\mb x(t) \in\mathcal{X}$ and $\mb k_{\textrm{clf}}(\bs \eta,t)\in\mathcal{U}$ for all $t\in\mathbb{R}_+$.
% \end{lemma}
% \begin{proof}
% From the ISS property of the low level controller, we know that $\mb x(t) - \mb x_d(t) \in\mathcal{E}$ for all $t\in\mathbb{R}_+$. Furthermore, we have that $x_d(t) \in\mathcal{X} \ominus \mathcal{E}$, as enforced by the MPC program; therefore, $\mb x(t) \in \mathcal{E}$ for all $t\in\mathbb{R}_+$.
% \end{proof}
% 
% \begin{theorem}
% $\|\mb k_{\textrm{clf}}(\bs \eta,t)\|_2 \le u_{max}$
% \end{theorem}
% \begin{proof}
% \NCS{Tie back into Theorem \ref{thm:input_bounds}}
% \end{proof}

% Lemma \ref{lem:stat_and_input} states that, given a solution to the MPC program, the input constrained low level controller is a) feasible, and b) able to keep the system within state and input bounds. Next, we will show that through the application of the low-level controller, the MPC program is recursively feasible. 




==> Leftover.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Notation %%%%%%%%%%%%%%%%%55
% \textit{Notation:} All bolded symbols are multivalued, and all italicized symbols are scalar valued. Let $\v_{k|t}$ represent the decision variable $\v$ at time $t+k\dt$, as planned at time $t$. The closed Ball of radius $r$ around a point $p$ will be written as $\bar B_r(p)$. The Lie derivative of the vector-valued function $y$ with respect to the vector field $f$ will be represented by $L_fy$. The convex hull of a collection of points $\mb{p}$ will be denoted as $\text{conv}(\mb{p})$. Finally, parenthetic matrices denote $(\mb a,\mb b,\ldots) = [\mb a^\top,\mb b^\top,\ldots]^\top$.

% Terms that we need to decide:
% \begin{itemize}
% \item ---- Low Level -----
% \item Dynamics: $\f, \g$
% \item State: $\x\in\mathcal{X}$
% \item Input: $\u\in\mathcal{U}$
% \item Disturbance: $\w\in\mathcal{W}$
% \item Feedback controller: $\k$
% \item Flow: $\bs \varphi_x(t)$ (should be $\bs \varphi_{\x}(t)$)
% \item Desired Trajectory (Low Level): $(\x_d(t), \u_d(t))$
% \item Subindexing output dynamics: $(\cdot)_{\eta,i}$
% \item Error function: $\mb e$ (which is canonically $\bs \eta$)
% \item Dynamics minus feedforward: $\mathcal{F}$
% \item $L_gL_f^{\gamma-1}$: $\mathcal{G}$ \red{(not yet defined)}
% \item Feedback Gains for FL Controller: $\mb K$
% \item Closed Loop linear dynamics from FL: $\mb F$
% \item Feedback Linearizing controller: $\mb k_{\textrm{fbl}}$
% \item Feedforward term: $\mb k_{\textrm{ff}}$
% \item Feedback Linearizing controller: $\mb k_{\textrm{fbl}}$
% \item Compact set to go in $\mathcal{E}$ for Lemma 1: $K$ 
% \item Robust Invariant Set: $\Omega$ (I would like this to be $\mathcal{E}$)
% \item ----- Bezier ---------
% \item Bezier polynomial: $\mb B$
% \item Bezier control points: $\mb b_i$
% \item Collection of Bezier control points: $\mb b$
% \item Bernstein polynomial: $\mb c$
% \item Matrix for increasing order of $\mb B$ by one: $\mb R$ (can be removed)
% \item Matrix for differentiating $\mb B$: $\mb S$ (can be removed)
% \item Matrix for differentiating to same order: $\mb H$
% \item Map from control points to boundary conditions: $\mb D$
% \item --- MPC ---
% \item State and Input constraints: $\mathcal{X}, \mathcal{U}$
% \item Terminal Control Invariant $\mathcal{X_F}$
% \item Linearized dynamics at time step $k$: $\mb{Lin}_k := [\mb A_k, \mb B_k, \mb C_k]$
% \item Stage cost: $h$
% \item Decision variables: $\mb \eta_k$
% \item Intermediate control points: $\mb b_i$ (does this make sense?)
% \item Matrix/Vector/Scalar for input tightening: $\mb M, \tilde{\mb M}, \mb N, \Gamma$
% \item Tuning constants: $\alpha, \beta, \gamma$
% \item Optimal Solution at time $t$: $\bs \eta^*_{t} = [\bs \eta^*_{0|t}, \ldots,\bs \eta^*_{k|t}]$
% \item Sampling time of MPC: $t\in\mathcal{T}=\cup_{i=0}^\infty\{iT\}$
% \item Linearization points: $(\bar{\x},\bar{\u})$

% What do we want to say in this paper:
% \begin{itemize}
%     \item Feedback linearization as a tool to transform from control affine to integrator form
%     \item MPC construction
%     \item Bezier curves
% \end{itemize}
% The novelty:
% \begin{itemize}
%     \item 
% \end{itemize}
% If we want 6 pages:
% \begin{itemize}
%     \item SISO multi stage integrator, disturbance and nonlinear dynamics at last stage
% \end{itemize}

% \end{itemize}


%%%%%%%%%%%%%%%%%%%%%%%% MPC SECTION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

    % \min_{\substack{x_0,\dots,x_N\in\mathbb{R}^n \\ u_0,\dots,u_{N-1}\in\mathbb{R}^m \\ \b_0,\ldots,\bez_N \in \mathbb{R}^{n\gamma},\\ \mb t_0,\ldots,\mb t_N \in \mathbb{R}^{n\gamma}}} \quad & \sum_{i=0}^{N-1} h(x_i,u_i) \tag{FTOCP} \label{eqn:mpc} \\% + V(x_N)\tag{\ref{eq:mpc}} \\
    % \min_{\substack{\u_{k|t} \\ \state_{k|t} \\ \mb s_{k|t}}} \quad & \sum_{i=0}^{N-1} h(x_i,u_i) \tag{FTOCP} \label{eqn:mpc} \\% + V(x_N)\tag{\ref{eq:mpc}} \\
    % \min_{\u_{k|t}, \state_{k|t}, \mb s_{k|t}, \bs \zeta_{k|t}} \quad & \sum_{i=0}^{N-1} h(\state_i,u_i) \tag{FTOCP} \label{eqn:mpc} \\% 
%   & \x_{k|t} \in \mathcal{X}\\%\ominus \E    \\
%   & \u_{k|t} \in \mathcal{U}\ominus \bar B_{\Gamma_k}(0) \\%\ominus L_k(\E\oplus \mb{I}_T\oplus \R)\\
%   & \|\x_{k|t}-\bar \x_{k|t}\|_2 \le L_T \\


% or, more verbosely:
% \begin{subequations}\label{eq:mpc}
% \begin{alignat}{2}
%     \min_{\substack{x_0,\dots,x_N\in\mathbb{R}^n \\ u_0,\dots,u_{N-1}\in\mathbb{R}^m}} \quad & \sum_{i=0}^{N-1} h(x_i,u_i) + V(x_N)\tag{\ref{eq:mpc}} \\
% \textrm{s.t.} \quad & \x_{k+1|t} = \A_{k|t}\x_{k|t} + \R_{k|t}\u_{k|t} + \C_{k|t} \\
%   & -\sqrt{\gamma} \frac{L_i^T P^{-1}L_i}{\sqrt{L_i^T P^{-1}L_i}} \le \ell_i-L_i^T\bs \x_{k|t} \\
%   & \u_{k|t} \in \mathcal{U}_c \ominus L_k(\E\oplus \mb{I}_T\oplus \R)\\
%   & \b(\x_{k|t},\x_{k+1|t}) \in \mathcal{X} \ominus \E \\
%   & \x_{0|t} = \x(t) \oplus \mathcal{E}\\
%   & \x_{N|t} \in \mathcal{X}_f
%   \end{alignat}
% \end{subequations}

% \subsection{Proof of Lemma \ref{lem:input_bounds}}
% \begin{proof}
% We begin by establishing a semidefinite ordering of the matrix $\mb M$.
% \begin{align*}
% \mb{\tilde{M}}(\alpha_2,\beta_2) \succeq \mb M(\alpha_2,\beta_2) \succeq \mb M(\alpha_1,\beta_1)
% \end{align*}
% for all $0\le \alpha_1 \le \alpha_2$ and $0\le\beta\le \beta_2$.

% It is clear from the definition of $\mb{\tilde{M}}$ to see that $\mb M$ and $\mb{\tilde{M}}$ commute (as they share the same eigenbasis). As such, $\mb{\tilde{M}}-\mb M$ has only nonnegative eigenvalues and is therefore a positive semidefinite matrix. As $\mb M$ is linear in $\beta$, we have $\mb M(\alpha_1,\beta_2) \succeq \mb M(\alpha_1,\beta_1)$ for $\beta_1 \le \beta_2$. Finally, consider:
% \begin{align*}
%     \mb M(\alpha_2,\beta_1) - \mb M(\alpha_1, \beta_1) = \begin{bmatrix} 2(\alpha_2-\alpha_1)\beta_1 & 0 \\ 0 & 0\end{bmatrix}
% \end{align*}
% whose eigenvalue is nonnegative for $\alpha_2\ge \alpha_1$.
% \end{proof}
% \begin{proof}

% As demonstrated in Proposition \ref{prop:succ}, by increasing the parameter to $\mb M$, and by taking its projection $\pi_{PSD}$, the quadratic form $\mb s^\top \mb M \mb s$ becomes more positive. Furthermore, as all entries of $\mb N$ and $\mb \Gamma$ are positive, increasing their parameters simply increases there value in the above statement. Therefore, taking $\underoverline c=\min\{L_{\mb{\mathcal{G}}^\dagger}, L_{\mb f},\mathcal{E}\}$, we are done.

% \end{proof}


% As the curve $\BEZc^{(n)}:[0,T]\to\R$ is one dimensional, we no longer need to consider the state space control points $\BEZ_i$, but instead must consider the original control points $\Bez_n$ of $\BEZc$. In other words, we know that $\BEZc^{(n)}\in \text{conv}\{\bez_{n,i}\})$ for $i=1,\ldots,p$. As $\BEZc^{(n)}$ is simply a B\'ezier curve, and $f(\x)\in\R$ is simply a point, we can use the first part of the proof to arrive at the desired result.
% Due to the convex hull property of Bezi\'er curves, we know $\BEZC(\tau)\in \text{conv}(\{\BEZ_i\})$ for $i=0,\ldots,p$ and for all $\tau\in[0,T]$. Taking the curve $\BEZC$ to be the image of $\BEZC(\tau)$ over the interval $[0,T]$, we have that:
% \begin{align*}
%     \|\BEZC(\tau) - \mb x\|_2 \le \sup_{r\in\BEZC}\|r - \mb x\|_2 \le \sup_{\BEZ\in\text{conv}(\{\BEZ_i\})}\|\BEZ-c\|_2.
% \end{align*}
% Furthermore, observe that as $\{\BEZ_i\}$ is a finite collection of points, it represents a bounded, convex polytope. As the two norm is a continuous, convex function, and the constraint set is convex and bounded by the previous argument, we know by the maximum principle that $\|\BEZ-c\|_2$ attains its maximum at an extreme point of the constraint set, i.e. a vertex of the polytope. Therefore, we can instead maximize the function over the vertices of the polytope, giving rise to:
% \begin{align*}
%     \|\BEZC(\tau) - \mb x\|_2 \le \sup_{i} \|\BEZ_i - c\|_2,
% \end{align*}
% as desired. 

% \begin{assumption}
% \label{ass:FSFL}
% The system \eqref{eqn:openloop_state} is full state feedback linearizable.
% \end{assumption}
% \begin{assumption}
% \label{ass:polytopes}
% $\mathcal{X}$, $\mathcal{U}$, and $\mathcal{X}_F$ are convex polytopes.
% \end{assumption}
% \begin{assumption}
% The sets $\mathcal{X}$ and $\mathcal{U}$ are compact and contain the origin in their interior. Additionally, $\mathcal{W}$ is compact, and contains the origin. 
% % \AT{$\mathcal{D}$ can't be compact, its open.} \NCS{Sorry, I was using $\mathcal{D}$ as the disturbance set.}
% \end{assumption}

% The previous sections have demonstrated how to produce continuous time guarantees while only having to reason about a discrete collection of points. This will allow us to develop an algorithm which produces dynamically admissible trajectories in discrete time.

%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%  Consider a linear, discrete time representation of \eqref{eqn:openloop_state} without disturbances as:
% \begin{align}
%     \label{eqn:linearizations}
%     \state_{k+1} & \triangleq \A_k \state_k + \B_k \u_k + \C_k
% \end{align}
% where $\A_k\in\R^{n\times n}, \B_k\in\R^n$, and $\C_k\in\R^n$ are calculated around the point $\overline{\mb{x}}_k \in\mathbb{R}^n$ and come from linearization and then discretization.
%%%%%%%%%%%%%%%%%%%%%%%

% \red{the following discussion will have to change now...}
% \begin{proposition}
% The pair $(\A_k, \R_k)$ is controllable.
% \end{proposition}
% \begin{proof}
% Under assumption \ref{ass:FSFL}, the continuous-time pair $(\A,\R)$ resulting from the linearization of the system about the origin is controllable \cite{isidori_elementary_1995}. One step Euler discretization is used to convert the system from a continuous time linear one to continuous time discrete one, which preserves controllability \cite{ewa_eulers_2007}.
% \end{proof}
% \begin{remark}
% Note that the choice of linearization then Euler discretization was explicit. Discretization of nonlinear systems may destroy feedback linearizeability and therefore controllability of the discrete linear pairs \cite{grizzle_feedback_1988}, and exact discretization of linear systems may similarly destroy controllability \cite{chen_linear_1999}.
% \end{remark}
% This representation could have come from linearizing then discretizing, or discretizing then linearizing, as discussed in \cite{gros_linear_nodate}
% The discretization of this pair, however, is not necessarily controllable unless certain sampling requirements are met \cite{}. Furthermore, if the system is discretized first, the discrete time nonlinear system may no longer be feedback linearizeable \cite{grizzle_feedback_1988}. 
% \subsection{Input Bounds}
% Next consider the input of the combined system for the time interval $t\in[t_k, t_{k+1})$:
% \begin{align*}
%     k_{NL}(\eta(t)) &= k_{NL}(Hx(t) - x^{\vec \gamma}_d(t)) \\
%     &\le L_k\Rig(\underbrace{\|x(t) - x^*(t)\|}_{\text{ISS-CLF}} + \underbrace{\|x^*(t) - x^*_k\|}_{\text{Desired Trajectory}}+\underbrace{\|x^*_k - \overline x_k\|}_{\text{Trust Region}}\Rig) \\
%     &\le L_k\Rig(\rho(\|\w\|_\infty) + \sup_{\b_i}\|\b_i(x_k,x_{k+1}) - x^*_k\|+\|x^*_k - \overline x_k\|\Rig)
% \end{align*}
% where the second line came from Lipschitz and adding and subtracting zero.
%


% and the dependence of ${\mb{{M}}}$, ${\mb N}_k$, and ${\Gamma}_k$ on user parameters $\alpha$ and $\beta$ have been dropped. %{$V:\mathcal{X}\to\R$ is the terminal cost%}
% In the above problem $\mb x_{k|t}$ represents planned state at time $k$ computed by solving the FTOCP at time $t$. 

% By adopting a multi-rate architecture, we are able to tie all the previous results together and make guarantees for the closed loop system \eqref{eqn:closedloop_state} with feedback controller defined in Algorithm \ref{alg:mpc-fl}.

%  Let $T \in \mathbb{R}_+$ denote a sample time whereby our Algorithm~\ref{alg:mpc-fl} calls the \ref{eqn:FTOCP} at discrete intervals $t\in\mathcal{T}=\cup_{\mpcindex=0}^\infty\{\mpcindex T\}$, and


%  consider the time $t=\mpcindex T$ for some $\mpcindex\in\mathbb{Z}$. Let $\state_{k|\mpcindex}$ denote the $k^{th}$ state at time $t=\mpcindex T$. For the collection of points $\{\overline\state_{k|\mpcindex}\}$ and $\{\overline u_{k|\mpcindex}\}$, let $\textbf{Lin}_{k|\mpcindex}$ denote the set of linearizations, i.e. $\textbf{Lin}_{k|\mpcindex} = \{\A_{k|\mpcindex},\B_{k|\mpcindex},\C_{k|\mpcindex}\}$, and let $\textbf{Lin}_o$ denote the linearization about the origin.


% At time $t=0$, Algorithm~\ref{alg:mpc-fl} should be initialized with the initial feasible state-input sequences $\{\overline{\x}_{k|0}\}$ and $\{\overline \u_{k|\mpcindex}\}$. From the solutions $\state_{k|\mpcindex}^*$ of the \eqref{eqn:FTOCP}, 

% a continuous dynamically admissible trajectory for the system \eqref{eqn:openloop_state} can be constructed via \eqref{eqn:bezsetctrlpts}, which then gets passed to the low-level controller in order to generate a control action $u(t)$.

% This is achieved by planning a sequence of states $\{\mb{x}_i\}$ and inputs $\{u_i\}$\footnote{In robust MPC schemes, the control action applied to the system is oftentimes given by the summation the control action from a pre-defined policy and the solution of the MPC optimization problem.} for a disturbance-free nominal model that approximates the mean evolution of uncertain nonlinear system~\eqref{eqn:openloop_state}.

% The multi-rate context, where MPC and a low-level controller are running at different frequencies, has recently received interest due to its practical usefulness [cite Ugo]. In such works, feasiblity of the low level controller was assumed; this work attempts to investigate conditions on when that assumption is valid. In order to make in order to make guarantees about the continuous-time behavior of the system \eqref{eqn:openloop1} despite the discrete-time nature of MPC, the evolution of the system during the inter-sampled time windows must be considered. 
% The most obvious choice is to constraint tighten the MPC state constraints by the possible deviation of the nonlinear and linear system dynamics, as done in \cite{noauthor_tube_nodate}. This bound however is often vacuous, and can lead to extremely conservative behavior. 
% Another option is to use barrier functions to guarantee that the evolution of the system remain in the state constraints, as presented in (??). This has the challenge of specifying a valid barrier function. Instead, we employ B\'ezier curves to achieve the goal of relating discrete time decisions to continuous time behavior. As such, we briefly introduce B\'ezier functions next. \red{cite quad Bezier paper}

% We begin to see the usefulness of B\'ezier curves: they allow us to bound the desired trajectory in continuous time by enforcing bounds on discrete points.

% This work is closely related to the real-time-iteration scheme presented in \cite{diehl_real-time_2005}; however here we assume that there is a controller acting at a faster frequency to maintain the desired outputs for the continuous time system.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This used to be in the Methodology:
% Sorry about messing things up :) I wanted to get a judge of space


% The objective of nonlinear control design is often to stabilize the state of this system to a given goal state $\mb{x}^*\in\R^n$. In the presence of unknown disturbances in the system dynamics this objective is often relaxed to stabilizing the system to a neighborhood of the goal state $\mb{x}^*$. A rich catalog of methods have been developed for achieving this objective that utilize the tools of Control Lyapunov Functions (CLFs) and Input-to-State Stability (ISS)
% \cite{freeman1996robust, kokotovic2001constructive, sepulchre2012constructive}. In most engineering settings, achieving this objective is complicated by the need to meet constraints on the system's state and input. These constraints are captured by sets $\mathcal{X}\subset\R^n$ and $\mathcal{U}\subset\R$ in which the system's state and input, respectively, must remain as the system evolves. The preceding methods for stabilization often yield highly structured controller designs, and modifying these designs to ensure constraint satisfaction often destroys the stability properties guaranteed by the controller. This issue is often circumnavigated by restricting the domain on which stability properties are guaranteed to a small neighborhood of the goal state $\mb{x}^*$, effectively ignoring the constraints. 

% In contrast to these methods, Model Predictive Control (MPC) seeks to constructively address constraints by directly incorporating them into the controller design \cite{allgower2004nonlinear,allgower2012nonlinear}. This is achieved by planning a sequence of states $\{\mb{x}_i\}$ and inputs $\{u_i\}$\footnote{In robust MPC schemes, the control action applied to the system is oftentimes given by the summation the control action from a pre-defined policy and the solution of the MPC optimization problem.} for a disturbance-free nominal model that approximates the mean evolution of uncertain nonlinear system~\eqref{eqn:openloop_state}.
% Safety is ensured tightening the constraint sets by the maximum deviation between the disturbance-free nominal model and the continuous time nonlinear system~\eqref{eqn:openloop_state}. The maximum deviation could be pre-computed or updated online in the MPC problem by scaling error sets computed offline~\cite{gao2014tube, kogel2015discrete, yu2013tube, singh2017robust,kohler2020computationally}.
% % that are consistent with both the system dynamics and the constraints through numerical optimization. Ensuring 
% Computing such error sets requires approximating the dynamics by leveraging often unknown Lipschitz constants or solving computationally intensive optimization programs. Furthermore, errors sets should account for inaccuracies introduced by the temporal discretization of the continuous time dynamics, which is needed as the MPC problem plans a sequence of states for a discrete time system\footnote{Notice that even when the MPC problem is introduced using a continuous time formulation, the solution to such problem is computed by discretizing the system dynamics}. Notice that the planned sequence of states is guaranteed to satisfy state constraints, but oftentimes no safety guarantees are given about the evolution of the continuous time dynamics.

% % \cite{gao2014tube, kogel2015discrete, yu2013tube, singh2017robust,kohler2020computationally}
% \AT{TODO}
% Moreover, disturbances often necessitate performing a reachability analysis to ensure constraint satisfaction, 

% or introducing an auxiliary controller  

% \NCS{I would like to have the problem statement be separate with relevant assumptions on the sets, I like this aspect of MPC literature that it is skimmable in that way}


% \AT{I'm a bit cautious about this, just because we're going to be adding more assumptions in later on those sets, tied to feedback linearizability. I still need to work on this section, just slow going because its high-level.}

% \NCS{I can see the hesitation, what if we move the ssumptions on the sets to the MPC section but keep a block of problem formulation?}

% \AT{It can work, will have to see where we're at as we add more. It can be hard to define the problem statement formally without the technical things we define after it, i.e. an ODE solution. I don't like talking about things we have yet to define, its icky.}
% \NCS{Ya, agreed...}

% Letting $\mathcal{X}\subset\mathbb{R}^n$ and $\mathcal{U}\subset\mathbb{R}^m$ denote the state and input constraint sets, and $\mathcal{X}_F\subset\mathcal{X}$ denote the goal set, the objective can be stated succinctly as:
% \begin{problem}
% % I know that this is confusing because we did not introduce the closed loop system yet, but I think we should save some of the weeds for the background.
% \label{prob:IVP}
% Design a feedback controller $\mb u = \mb k(\mb x, t)$ which guarantees that the system \eqref{eqn:openloop1} satisfies $\mb x(t) \in\mathcal{X}\subset\mathbb{R}^n,~ \mb u(t) \in \mathcal{U}\subset\mathbb{R}^m$ for all time $t\in\mathbb{R}_{\ge 0}$ and for all disturbances $\mb d(t) \in \mathcal{D}$, and that the flow $\mb x(t)$ asymptotically converges to the origin.
% % in finite time to $\cal{X}_F$.
% \end{problem}
% \noindent The following assumptions will be made on the described sets:
% % \noindent Due to the difficulty of solving the general problem, some standard simplifying assumptions will be made:
% % \begin{assumption}
% % $\cal{X}_F$ is a control invariant, i.e. for all $\mb x_0\in\mathcal{X}_f$ there exists a $\mb u(t)\in\mathcal{U}$ such that the solution to the closed loop system $\mb x(t)\in\mathcal{X}_F$ for all $t\in\mathbb{R}_{\ge 0}$. 
% % \end{assumption}

% To achieve Problem \ref{prob:IVP}, a hierarchical multi-rate control architecture will be adopted where low level trajectory tracking controllers running in continuous time need to coordinate with mid level trajectory generating planners running at a slow, time-sampled frequency. Specifically, Control Lyapunov Functions (CLFs) will be employed to track the trajectories on the full nonlinear model that Model Predictive Control (MPC) generates on linearizations of the model. Note that extensions can be made to relax the low level controller to a sampled data paradigm, as in \cite{taylor2021sampled}. 
%%%%%%%%%%% Line of completion

% Furthermore, we require that the system \eqref{eqn:openloop1} satisfy the following state and input constraints:
% \begin{align*}
    % \mb x(t) \in\mathcal{X}\subset\mathbb{R}^n,~ \mb u(t) \in \mathcal{U}\subset\mathbb{R}^m
% \end{align*}
% for all time $t\in\mathbb{R}_{\ge 0}$. 

% \begin{problem}
% % I know that this is confusing because we did not introduce the closed loop system yet, but I think we should save some of the weeds for the background.
% \label{prob:IVP}
% Design a feedback controller $\mb u = \mb k(\mb x, t)$ which guarantees that the system \eqref{eqn:openloop1} satisfies state and input constraints for all time and for all disturbances, and that the flow of the system converges in finite time to the goal set.
% \end{problem}

% Fixing a feedback controller ${\mb{u}=\mb{k}(\mb {x},t)}$ yields the closed loop system:
% \begin{equation}
%     \label{eqn:closedloop1}
%     \dot{\mb{x}} = \mb{f}(\mb{x})+\mb{g}(\mb{x})\mb{k}(\mb{x},t) + \mb{d}(t).
% \end{equation}



% \begin{assumption}
% The sets $\mathcal{U}$ and $\mathcal{W}$ are compact and the set $\mathcal{X}$ is closed.
% \end{assumption}

% Let $x(t)$ be the solution to \eqref{eqn:openloop1} for initial condition $x_0:=x(0)\in\mathbb{R}^n$.
% Our objective is as follows:
% \begin{problem}
% \label{prob:IVP}
% Drive initial conditions $x_0$ to $\mathcal{X}_F$ for the disturbed system \eqref{eqn:openloop1} while enforcing that $\mb x(t) \in\mathcal{X}$ and $\u(t)\in\mathcal{U}$ for all time $t\in\mathbb{R}_{\ge 0}$ and for all disturbances $\mb d(t)\in\mathcal{W}$.
% \end{problem}


%
% While the preceding construction of stabilizing controllers for nonlinear systems via feedback linearization and Control Lyapunov Functions offers a powerful set of tools for directly addressing the nonlinear nature of the system \eqref{eqn:openloop1}, it fails to incorporate state and input constraints. 
%
%
% \subsection{System Dynamics}
%
% Consider 

%



% \begin{problem}
% Let $\mathcal{X},\mathcal{X}_F\subset\R^n$ be polytopes satisfying $\mathcal{X}_F\subseteq\mathcal{X}$, and let $\mathcal{U}\subset\R^m$ be a polytope with $\mb{0}\in\mathcal{U}$.

% \end{problem}




% \begin{definition}[\textit{Constrained Dynamically Admissible Trajectory}]
% Given constants $\underline{t},\overline{t}\in\R_{\ge0}$ with $\underline{t} < \overline{t}$, a piecewise-continuously differentiable function $\x_d:[\underline{t},\overline{t}]\to\mathcal{X}$ is a \textit{constrained dynamically admissible trajectory} for the system \eqref{eqn:openloop1} if there exists a piecewise-continuous function $\u_d:[\underline{t},\overline{t}]\to\mathcal{U}$ such that:
% \begin{equation}
%     \label{eqn:dynadmistraj}
%     \dot{\mb{x}}_d(t) = \f(\x_d(t))+\g(\x_d(t))\u_d(t),
% \end{equation}
% for almost all $t\in[\underline{t},\overline{t}]$.
% \end{definition}


% \begin{align}
% \tag{CLF-QP} \label{clf-qp}
%     \mb{k}_\textrm{clf}(\bs{\eta},t) =  \argmin_{\mb{u}\in\R^m}& \frac{1}{2}\Vert\mb{u}-\mb{k}_{\textrm{ff}}(\bs{\eta},t)\Vert_2^2 \\ \textrm{s.t.}  ~ & \derp{V}{\mb{e}}(\mb{e}(\bs{\eta},t))\dot{\mb{e}}(\bs{\eta},t,\mb{u}) \leq -\alpha_3(\Vert\mb{e}(\bs{\eta},t)\Vert)\nonumber \\
%     &\mb u_{min} \le \mb u \le \mb u_{max}. \nonumber
% \end{align}



==> OLD/BackgroundOLD.tex <==
\section{Background}
This section presents a review of feedback linearization, the synthesis of Control Lyapunov Function (CLF) based controllers via convex optimization, and stability properties in the presence of disturbances. 

\subsection{System Dynamics}

Consider a nonlinear control-affine system: 
\begin{equation}
    \label{eqn:openloop1}
    \dot{\mb{x}} = \mb{f}(\mb{x})+\mb{g}(\mb{x})\mb{u},
\end{equation}
with state $\mb{x}\in\R^n$, input $\mb{u}\in\R^m$ and functions ${\mb{f}:\R^n\to\R^n}$ and ${\mb{g}:\R^n\to\R^{n\times m}}$ assumed to be continuously differentiable on $\R^n$. Let $\underline{t},\overline{t}\in\R_{\geq 0}$ with $\underline{t}<\overline{t}$ and let ${\mb{k}:\R^n\times[\underline{t},\overline{t}]\to\R^m}$ be a state feedback controller that is locally Lipschitz continuous with respect to its first argument and piecewise-continuous with respect to its second argument on $\R^n\times[\underline{t},\overline{t}]$ \footnote{These definitions are taken as in \cite{khalil2002nonlinear}. In particular, local Lipschitz continuity holds with a Lipschitz constant that is uniform in the function's second argument, and piecewise-continuity requires the existence of one-sided limits at points of discontinuity.}. Setting the input ${\mb{u}=\mb{k}(\mb {x},t)}$ yields the closed loop system:
\begin{equation}
    \label{eqn:closedloop1}
    \dot{\mb{x}} = \mb{f}(\mb{x})+\mb{g}(\mb{x})\mb{k}(\mb{x},t).
\end{equation}
As the functions $\mb{f}$, $\mb{g}$, and $\mb{k}$ are locally Lipschitz continuous with respect to $\mb{x}$ and piecewise continuous with respect to $t$, for any initial time $t_0\in[\underline{t},\overline{t})$ and any initial condition $\mb{x}_0 \in \R^n$, there exists a constant\footnote{The dependence on $t_0$ arises from the fact that $\mb{k}$ is not defined for $t>\overline{t}$.} $\delta(t_0,\mb{x}_0)>0$ such that \eqref{eqn:closedloop1} has a unique piecewise-continuously differentiable solution $\bs{\varphi}:[t_0,t_0+\delta(t_0,\mb{x}_0))\to\R^n$ satisfying:
\begin{align}
    \dot{\bs{\varphi}}(t) & = \mb{f}(\bs{\varphi}(t)) + \mb{g}(\bs{\varphi}(t))\mb{k}(\bs{\varphi}(t),t), \label{eqn:soldiff}\\
    \bs{\varphi}(t_0) & = \mb{x}_0. \label{eqn:solic}
\end{align}
for almost all $t\in [t_0,t_0+\delta(t_0,\mb{x}_0))$ \cite{khalil2002nonlinear}. The system \eqref{eqn:openloop1} may also be used to define a class of reference trajectories:
\begin{definition}[\textit{Dynamically Admissible Trajectory}]
Given constants $\underline{t},\overline{t}\in\R_{\ge0}$ with $\underline{t} < \overline{t}$, a piecewise-continuously differentiable function $\x_d:[\underline{t},\overline{t}]\to\R^n$ is a \textit{dynamically admissible trajectory} for the system \eqref{eqn:openloop1} if there exists a piecewise-continuous function $\u_d:[\underline{t},\overline{t}]\to\R^m$ such that:
\begin{equation}
    \label{eqn:dynadmistraj}
    \dot{\mb{x}}_d(t) = \f(\x_d(t))+\g(\x_d(t))\u_d(t),
\end{equation}
for almost all $t\in[\underline{t},\overline{t}]$.
\end{definition}

%\footnote{More specifically, the piecewise-continuous differentiability of $\mb{x}_d$ implies the existence of a unique finite subdivision $\{t_0,\ldots,t_N\}$, $N\in\mathbb{N}$, with $t_0 = \underline{t}$ and $t_N = \overline{t}$ such that $\mb{x}_d$ is continuously differentiable on the open intervals $(t_i,t_{i+1})$, $i=0,\ldots,N-1$, and is not differentiable at the points $\{t_0,\ldots,t_N\}$. The equality in \eqref{eqn:dynadmistraj} is required to hold on these open intervals.}

% \footnote{In the presence of discontinuities of the controller $\mb{k}$ in time, the expression in \eqref{eqn:soldiff} is understood to be satisfied by the solution $\bs{\varphi}$ almost everywhere on the domain $I(\mb{x}_0)$.} 


% We will use the following definition in characterizing the behavior of a nonlinear system around a dynamically admissible trajectory:
% \begin{definition}{\textit{(Time-Varying Forward Invariance)}}
% A set-valued function $\C:\R_{\geq 0}\rightrightarrows\R^n$ defines a \emph{time-varying forward invariant set} if for any initial time $t_0\in[\underline{t},\overline{t}]$ and initial condition ${\mb{x}_0 \in \C(t_0)}$, we have ${\bs{\varphi}(t)\in\C(t)}$ for all $t\in[t_0,t_0+\delta(t_0,\mb{x}_0))$. 
% \end{definition}

% The combination of continuous-time controllers with discrete-time planners yields functions satisfying different differentiability properties. We denote the \textit{right-handed derivative} of a piecewise continuously differentiable function $\bs{\varphi}:\R\to\R^n$ at $t\in\R$ as:
% \begin{equation*}
%     \dot{\bs{\varphi}}^r(t) = \lim_{h\to 0^+}\frac{1}{h}(\bs{\varphi}(t+h)-\bs{\varphi}(h)),
% \end{equation*}
% and note that if $\bs{\varphi}$ is continuously differentiable, we have $\dot{\bs{\varphi}}(t) = c \implies \dot{\bs{\varphi}}^r(t) = c$. Given a continuously differentiable function $\bs{\psi}:\R^n\to\R^p$, a piecewise continuously differentiable function $\bs{\varphi}:\R\to\R^n$, and denoting $\bs{\omega}=(\bs{\psi}\circ\bs{\varphi})$, we have that:
% \begin{equation*}
%     \dot{\bs{\omega}}^r(t) = \grad\bs{\psi}(\bs{\varphi}(t))\dot{\bs{\varphi}}^r(t)
% \end{equation*}
% where $\grad\bs{\psi}:\R^n\to\R^{p\times n}$ is the standard derivative of $\bs{\psi}$. Lastly, if $\varphi:\R\to\R$ is piecewise continuously differentiable, we have that $\dot{\varphi}^r(t) = c \implies D^+\varphi(t) = c$, where $D^+\varphi:\R\to\R_e$ is the \textit{upper right-hand Dini derivative} \cite{khalil2002nonlinear}.

\subsection{Feedback Linearization}

Feedback linearization offers a tool for the synthesis of stabilizing controllers for nonlinear systems, and will serve an important role in tracking dynamically admissible trajectories generated via model predictive control. In this work we consider the following abbreviated definition, but additional details may be found in \cite{sastry1999nonlinear,isidori1995nonlinear}:

\begin{definition}[\textit{Full-State Feedback Linearizability}]
The system \eqref{eqn:openloop1} is \textit{full-state feedback linearizable} if there exist open sets $\mathcal{D},\mathcal{E}\subseteq\R^n$ and a diffeomorphism $\bs{\Phi}: \mathcal{D} \to \mathcal{E}$ such that the \textit{transformed state}:
\begin{equation}
\label{eqn:transtate}
\bs{\eta} = \begin{bmatrix}\bs{\eta}_1^\top \cdots \bs{\eta}_k^\top \end{bmatrix}^\top =  \bs{\Phi}(\mb{x}),
\end{equation}
with $\bs{\eta}_i\in\R^{n_i}$, $n_1+\ldots +n_k = n$, has dynamics governed by the nonlinear control-affine system:
\begin{equation}
\label{eqn:etadot}
\dot{\bs{\eta}} = \mb{f}_{\bs{\eta}}(\bs{\eta})+\mb{g}_{\bs{\eta}}(\bs{\eta})\mb{u} =  \derp{\bs{\Phi}}{\mb{x}}(\mb{x})(\mb{f}(\mb{x}) + \mb{g}(\mb{x})\mb{u}),
\end{equation}
% \begin{equation}
% \label{eqn:etadot}
% \dot{\bs{\eta}} = \mb{f}_{\bs{\eta}}(\bs{\eta}) + \mb{g}_{\bs{\eta}}(\bs{\eta})\mb{u} = \derp{\bs{\Phi}}{\mb{x}}(\mb{x})(\mb{f}(\mb{x}) + \mb{g}(\mb{x})\mb{u}),
% \end{equation}
with $\mb{f}_{\bs{\eta}}:\mathcal{E}\to\R^n$ and $\mb{g}_{\bs{\eta}}:\mathcal{E}\to\R^{n\times m}$ such that: 
\begin{equation}
\label{eqn:etadotdecomp}
    \dot{\bs{\eta}}_i  =  \begin{bmatrix}\mb{0}_{n_i-1} & \mb{I}_{n_i-1 \times n_i-1} \\ 0 & \mb{0}_{n_i-1}^\top  \end{bmatrix} \bs{\eta}_i+ \begin{bmatrix} \mb{0}_{n_i-1} \\ f_{\bs{\eta},i}(\bs{\eta})\end{bmatrix} + \begin{bmatrix} \mb{0}_{n_i-1 \times m} \\ \mb{g}_{\bs{\eta},i}(\bs{\eta})^\top \end{bmatrix} \mb{u},
\end{equation}
for all $\bs{\eta} \in \mathcal{E}$ and $\mb{u}\in\R^m$, with\footnote{Let $r_i = \sum_{j=1}^{i} n_j$. Then $f_{\bs{\eta},i}$ is the $r_i^{\textrm{th}}$ element of $\mb{f}_{\bs{\eta}}$, and $\mb{g}_{\bs{\eta},i}^\top$ the $r_i^{\textrm{th}}$ row of $\mb{g}_{\bs{\eta}}$. } $f_{\bs{\eta},i}:\mathcal{E}\to\R$ and $\mb{g}_{\bs{\eta},i}:\mathcal{E}\to\R^{m}$ for $i = 1,\ldots,k$. Furthermore the matrix:
\begin{equation}
\label{eqn:Gmat}
    \mathcal{G}(\bs{\eta}) = \begin{bmatrix} \mb{g}_{\bs{\eta},1}(\bs{\eta}) & \cdots & \mb{g}_{\bs{\eta},k}(\bs{\eta}) \end{bmatrix}^\top \in \R^{k\times m},
\end{equation}
is right-invertible for all transformed states $\bs{\eta} \in \mathcal{E}$.
\end{definition}





Full-state feedback linearizability can be seen as a property of the system \eqref{eqn:openloop1} on the set $\mathcal{D}$. Importantly, this property may be used to achieve stabilization to dynamically admissible trajectories. Given constants $\underline{t},\overline{t}\in\R_{\geq 0}$ with $\underline{t}<\overline{t}$ and a dynamically admissible trajectory $\mb{x}_d:[\underline{t},\overline{t}]\to\mathcal{D}$ for a full-state feedback linearizable system, define:
\begin{equation}
\bs{\eta}_d(t) = \begin{bmatrix}\bs{\eta}_{d,1}(t)^\top \cdots \bs{\eta}_{d,k}(t)^\top \end{bmatrix}^\top = \bs{\Phi}(\mb{x}_d(t)),
\end{equation}
and the error $\mb{e}:\mathcal{E}\times[\underline{t},\overline{t}]\to\R^n$:
\begin{equation}
\label{eqn:err}
\mb{e}(\bs{\eta},t) = \begin{bmatrix}\mb{e}_{1}(\bs{\eta},t)^\top \cdots \mb{e}_{k}(\bs{\eta},t)^\top \end{bmatrix}^\top = \bs{\eta}- \bs{\eta}_{d}(t).
\end{equation}
We have that:
\begin{align}
    \dot{\mb{e}}(\bs{\eta},t,\mb{u}) =&~\mb{f}_{\bs{\eta}}(\bs{\eta})+\mb{g}_{\bs{\eta}}(\bs{\eta})\mb{u} \label{eqn:errdyn} \\ &-\derp{\bs{\Phi}}{\mb{x}}(\mb{x}_d(t))(\f(\x_d(t))+\g(\x_d(t))\u_d(t)) \nonumber,
\end{align}
where it follows from \eqref{eqn:etadot}-\eqref{eqn:etadotdecomp} that:
\begin{align}
\label{eqn:errordotdecomp}
    \dot{\mb{e}}_i(&\bs{\eta},t,\mb{u})   =  \begin{bmatrix}\mb{0}_{n_i-1} & \mb{I}_{n_i-1 \times n_i-1} \\ 0 & \mb{0}_{n_i-1}^\top  \end{bmatrix} \mb{e}_i(\bs{\eta},t)  + \begin{bmatrix} \mb{0}_{n_i-1 \times m} \\ \mb{g}_{\bs{\eta},i}(\bs{\eta})^\top \end{bmatrix} \mb{u} \nonumber \\ & + \begin{bmatrix} \mb{0}_{n_i-1} \\ f_{\bs{\eta},i}(\bs{\eta})-f_{\bs{\eta},i}(\bs{\eta}_d(t))-\mb{g}_{\bs{\eta},i}(\bs{\eta}_d(t))^\top\mb{u}_d(t)\end{bmatrix},
\end{align}
for all $\bs{\eta}\in\mathcal{E}$, $\mb{u}\in\R^m$, and almost all $t\in[\underline{t},\overline{t}]$. The right invertibility of the matrix $\mathcal{G}(\bs{\eta})$ in \eqref{eqn:Gmat} for all $\bs{\eta}\in\mathcal{E}$ enables a feedback controller $\mb{k}_{\textrm{fbl}}:\mathcal{E}\times[\underline{t},\overline{t}]\to\R^m$ that yields:
% \begin{equation}
%  \dot{\mb{e}}(\bs{\eta},t,\mb{k}_{\textrm{fbl}}(\bs{\eta},t)) = \underbrace{\begin{bmatrix}\mb{F}_1 & \mb{0} & \cdots & \mb{0} \\ \mb{0} & \mb{F}_2 & \cdots & \mb{0} \\ \vdots & \vdots & \ddots & \vdots \\ \mb{0} & \mb{0} & \cdots & \mb{F}_k \end{bmatrix}}_{\mb{F}}\begin{bmatrix} \mb{e}_1(\bs{\eta},t) \\ \vdots \\ \mb{e}_k(\bs{\eta},t) \end{bmatrix}, \label{eqn:errordotcloop}
% \end{equation}
\begin{equation}
 \dot{\mb{e}}(\bs{\eta},t,\mb{k}_{\textrm{fbl}}(\bs{\eta},t)) = \underbrace{\begin{bmatrix}\mb{F}_1 &  & \\  & \ddots &  \\   &  & \mb{F}_k \end{bmatrix}}_{\mb{F}}\begin{bmatrix} \mb{e}_1(\bs{\eta},t) \\ \vdots \\ \mb{e}_k(\bs{\eta},t) \end{bmatrix}, \label{eqn:errordotcloop}
\end{equation}
for all $\bs{\eta}\in\mathcal{E}$ and almost all $t\in[\underline{t},\overline{t}]$, where $\mb{F}_{i}\in\R^{n_i\times n_i}$, and consequently $\mb{F}\in\R^{n\times n}$, are Hurwitz matrices. For any $\mb{Q}\in\mathbb{S}^n_{\succ 0}$ (symmetric positive definite matrices) there exists a unique matrix $\mb{P}\in\mathbb{S}^n_{\succ 0}$ that solves the Continuous Time Lyapunov Equation:
\begin{equation}
    \mb{F}^\top\mb{P}+\mb{PF} = -\mb{Q}.
\end{equation}
The resulting function $V:\R^n\to\R_{\geq 0}$ defined as:
\begin{equation}
\label{eqn:lyap}
    V(\mb{e}(\bs{\eta},t)) = \mb{e}(\bs{\eta},t)^\top\mb{P}\mb{e}(\bs{\eta},t),
\end{equation}
is a Lyapunov function satisfying:
\begin{align}
   \lambda_{\textrm{min}}(\mb{P})\Vert\mb{e}(\bs{\eta},t)\Vert_2^2 \leq  V(\mb{e}(\bs{\eta},t))  & \leq  \lambda_{\textrm{max}}(\mb{P})\Vert\mb{e}(\bs{\eta},t)\Vert_2^2, \label{eqn:lyapbounds} \\ 
\derp{V}{\mb{e}}(\mb{e}(\bs{\eta},t'))\dot{\mb{e}}(\bs{\eta},t',\mb{k}_{\textrm{fbl}}(\bs{\eta},t'))  & =  -\mb{e}(\bs{\eta},t')^\top\mb{Q}\mb{e}(\bs{\eta},t'), \nonumber \\ & \leq - \lambda_{\textrm{min}}(\mb{Q})\Vert\mb{e}(\bs{\eta},t')\Vert_2^2
    , \label{eqn:lyapdecay}
\end{align}
for all $\bs{\eta}\in\mathcal{E}$, all $t\in[\underline{t},\overline{t}]$, and almost all $t'\in[\underline{t},\overline{t}]$.

% , implying:
% \begin{equation}
%     \Vert\mb{e}(\bs{\Phi}(\bs{\varphi}(t)),t)\Vert_2 \leq e^{-\gamma(t-t_0)} \Vert\mb{e}(\bs{\Phi}(\bs{\varphi}(t_0)),t_0)\Vert_2
% \end{equation}



\subsection{Control Lyapunov Functions}
While feedback linearization provides a constructive approach for synthesizing stabilizing controllers, the cancellation of nonlinear dynamics to achieve linear dynamics as in \eqref{eqn:errordotcloop} may be inefficient \cite{freeman1996robust}. Control Lyapunov Functions provide an alternative method for synthesizing stabilizing controllers via convex optimization. 

Before defining Control Lyapunov Functions, we denote a continuous function $\alpha:[0,a)\to\R_{\geq 0}$, with $a>0$, as \textit{class $\K$} ($\alpha\in\K$) if $\alpha(0)=0$ and $\alpha$ is strictly monotonically increasing. If $a=\infty$ and $\lim_{r\to\infty}\alpha(r)=\infty$, then $\alpha$ is \textit{class $\K_\infty$} ($\alpha\in\K_\infty$). More details on these functions may be found in \cite{kellett2014compendium}, but they enable the following definition:

\begin{definition}[\textit{Control Lyapunov Functions}, \cite{artstein1983stabilization, jankovic2018robust}]
A continuously differentiable function $V:\R^n\to\R_{\geq 0}$ is a \textit{Control Lyapunov Function (CLF)} for \eqref{eqn:errdyn} if there exist $\alpha_1,\alpha_2,\alpha_3 \in \K_\infty$ such that for all $\bs{\eta}\in\mathcal{E}$, $t\in[\underline{t},\overline{t}]$ and almost all $t'\in[\underline{t},\overline{t}]$:
\begin{align}
    \alpha_1(\Vert\mb{e}(\bs{\eta},t)\Vert) \leq V(\mb{e}(\bs{\eta},t)) & \leq \alpha_2(\Vert\mb{e}(\bs{\eta},t)\Vert), \label{eqn:clfbounds} \\ \inf_{\mb{u}\in\R^m}\derp{V}{\mb{e}}(\mb{e}(\bs{\eta},t'))\dot{\mb{e}}(\bs{\eta},t',\mb{u}) & < -\alpha_3(\Vert\mb{e}(\bs{\eta},t')\Vert). \label{eqn:clfdecay}
\end{align}
\end{definition}
The function $V$ defined in \eqref{eqn:lyap} satisfies \eqref{eqn:clfbounds}-\eqref{eqn:clfdecay} with $\alpha_i(r) = k_ir^2$ with $k_1 = \lambda_{\textrm{min}}(\mb{P})$, $k_2 = \lambda_{\textrm{max}}(\mb{P})$, and $k_3 = \lambda_{\textrm{min}}(\mb{Q}')$ for any $\mb{Q}'\in\mathbb{S}^n_{\succ 0}$ such that $\mb{Q}' \prec \mb{Q}$. To see how this function can be used to synthesize a stabilizing controller via convex-optimization, first define a function $\bs{\nu}:\mathcal{E}\times[\underline{t},\overline{t}]\to\R^k$:
\begin{equation}
    \bs{\nu}(\bs{\eta},t) = \begin{bmatrix} f_{\bs{\eta},1}(\bs{\eta})-f_{\bs{\eta},1}(\bs{\eta}_d(t))-\mb{g}_{\bs{\eta},1}(\bs{\eta}_d(t))^\top\mb{u}_d(t) \\ \vdots \\ f_{\bs{\eta},k}(\bs{\eta})-f_{\bs{\eta},k}(\bs{\eta}_d(t))-\mb{g}_{\bs{\eta},k}(\bs{\eta}_d(t))^\top\mb{u}_d(t)\end{bmatrix},
\end{equation}
and define the following feed-forward controller:
\begin{equation}
\label{eqn:FL}
    \mb{k}_{\textrm{ff}}(\bs{\eta},t) = -\mathcal{G}(\bs{\eta})^\top(\mathcal{G}(\bs{\eta})\mathcal{G}(\bs{\eta})^\top)^{-1}\bs{\nu}(\bs{\eta},t).
\end{equation}
This feed-forward controller is incorporated into the following controller specified via a convex Quadratic Program (QP):
\begin{align}
\tag{CLF-QP} \label{clf-qp}
    \mb{k}_\textrm{clf}(\bs{\eta},t) =  \argmin_{\mb{u}\in\R^m}& \frac{1}{2}\Vert\mb{u}-\mb{k}_{\textrm{ff}}(\bs{\eta},t)\Vert_2^2 \\ \textrm{s.t.}  ~ & \derp{V}{\mb{e}}(\mb{e}(\bs{\eta},t))\dot{\mb{e}}(\bs{\eta},t,\mb{u}) \leq -\alpha_3(\Vert\mb{e}(\bs{\eta},t)\Vert)\nonumber.
\end{align}
\subsection{Input-to-State Stability}

In many practical engineering settings, there are external disturbances to the dynamics of the system, yielding the following disturbed nonlinear control affine system:
\begin{equation}
    \label{eqn:eomdist}
    \dot{\mb{x}} = \mb{f}(\mb{x}) + \mb{g}(\mb{x})\mb{u} + \mb{d}(t),
\end{equation}
with a piecewise continuous disturbance signal $\mb{d}:\R_{\geq 0}\to\R^n$. As before, a state-feedback controller yields a disturbed closed-loop system:
\begin{equation}
    \label{eqn:cloopdist}
    \dot{\mb{x}}= \mb{f}(\mb{x}) + \mb{g}(\mb{x})\mb{k}(\mb{x},t)+\mb{d}(t),
\end{equation}
which for any initial time $t_0\in[\underline{t},\overline{t})$ and initial condition in $\mb{x}_0\in\R^n$ there exists a constant $\delta(t_0,\mb{x}_0)>0$ such that \eqref{eqn:closedloop1} has a unique solution $\bs{\varphi}_d:[t_0,t_0+\delta(t_0,\mb{x}_0))\to\R^n$ satisfying:
\begin{align}
    \dot{\bs{\varphi}}_d(t) & = \mb{f}(\bs{\varphi}(t)) + \mb{g}(\bs{\varphi}(t))\mb{k}(\bs{\varphi}(t),t)+\mb{d}(t), \label{eqn:distsoldiff}\\
    \bs{\varphi}_d(t_0) & = \mb{x}_0. \label{eqn:distsolic}
\end{align}
for almost all $t\in [t_0,t_0+\delta(t_0,\mb{x}_0))$.

Given a feedback linearizable system and a dynamically admissible trajectory, the disturbance signal subsequently induces\footnote{The relationship between $\mb{d}$ and $\mb{d}_{\bs{\eta}}$, and their respective bounds, is made explicit in Section \ref{sec:}.} a disturbance signal, denoted $\mb{d}_{\bs{\eta}}:\R_{\geq 0}\to\R^n$, in the dynamics of the error $\mb{e}$ defined in \eqref{eqn:err}:
\begin{align}
    \dot{\mb{e}}(\bs{\eta},t,\mb{u}) =&~\mb{f}_{\bs{\eta}}(\bs{\eta})+\mb{g}_{\bs{\eta}}(\bs{\eta})\mb{u} + \mb{d}_{\bs{\eta}}(t) \nonumber \\ &-\derp{\bs{\Phi}}{\mb{x}}(\mb{x}_d(t))(\f(\x_d(t))+\g(\x_d(t))\u_d(t)) \label{eqn:disterrdyn},
\end{align}


Given the existence of a unique solution to the disturbed closed-loop system, consider the following definition:
\begin{definition}{\textit{(Time-Varying Forward Invariance)}}
A set-valued function $\C:\R_{\geq 0}\rightrightarrows\R^n$ defines a \emph{time-varying forward invariant set} if for any initial time $t_0\in[\underline{t},\overline{t}]$ and initial condition ${\mb{x}_0 \in \C(t_0)}$, we have ${\bs{\varphi}_d(t)\in\C(t)}$ for all $t\in[t_0,t_0+\delta(t_0,\mb{x}_0))$. 
\end{definition}


% , implying that:
% \begin{equation}
%     \Vert \mb{e}(\bs{\Phi}(\bs{\varphi}(t)),t)\Vert_2 \leq -\exp()\Vert \mb{e}(\bs{\Phi}(\bs{\varphi}(0)),0)\Vert_2
% \end{equation}


% a controller $\mb{k}_{\mathrm{fbl}}: \mathcal{\R}^n \times \R^k \to \R^m$, $k\leq m$, and a controllable pair $(\mb{A}, \mb{B}) \in \R^{n \times n} \times \R^{n \times k}$ satisfying:
% \begin{equation}
% \label{eqn:fblindef}
%     D\bs{\Phi}(\mb{x})(\mb{f}(\mb{x}) + \mb{g}(\mb{x})\mb{k}_{\mathrm{fbl}}(\mb{x}, \mb{v})) = \mb{A}\bs{\Phi}(\mb{x}) + \mb{B}\mb{v} ,
% \end{equation}

% Consider a nonlinear control-affine system with state $\mb{x}=\begin{bmatrix} \mb{x}_1^\top \cdots \mb{x}_k^\top \end{bmatrix}^\top \in\R^n$ and dynamics of the form:
% \begin{equation}
%     \dot{\mb{x}}_i  =  \begin{bmatrix}\mb{0}_{n_i} & \mb{I}_{n_i-1 \times n_i-1} \\ 0 & \mb{0}_{n_i}  \end{bmatrix} \mb{x}_i+ \begin{bmatrix} \mb{0}_{n_i-1} \\ f_i(\mb{x})\end{bmatrix} + \begin{bmatrix} \mb{0}_{n_i-1 \times m} \\ \mb{g}_i(\mb{x}) \end{bmatrix} \mb{u}
% \end{equation}
% for $j = 1,\ldots,\gamma_i - 1$ and $i = 1,\ldots k$, where $\mb{f}_i:\R^n\to\R$ and $\mb{g}_i$



% \section{Preliminaries}
% In the following section, we will give the necessary background on Euler-Lagrange mechanics, Control Lyapunov Functions, and will introduce the problem formulation. Consider an Euler-Lagrange system with configuration coordinates $\q\in\Q\subseteq\R^n$ and state vector $\x=(\q,\dot\q)\in\mathcal{X}=T\Q\subseteq\R^{2n}$. Applying D'Alembert's principle to the Euler-Lagrange equations for the system, the dynamics can be written as:
% \begin{align}
%     \D(\q) + \H(\q,\dot \q) = \B\u \label{eq:robotEOM}
% \end{align}
% where $\D(\q)\in\mathbb{R}^{n\times n}$ is the mass-inertia matrix, $\H(\q,\dot\q)\in\R^n$ contains the Coriolis, gravity, and additional non-conservative forces, $\B\in\R^{n\times m}$ is the actuation matrix, and $\u\in\mathcal{U}\subseteq\mathbb{R}^m$ is the control input. The equations of motion in \eqref{eq:robotEOM} can be rearranged into control affine form as:
% \begin{align}
% \label{eq:eom}
%     \dot \x = \underbrace{\begin{bmatrix} \dot \q \\ -\D(\q)^{-1}\H(\q,\dot\q)\end{bmatrix}}_{\f(\x)} + \underbrace{\begin{bmatrix} \mb{0} \\ \D(\q)^{-1} \end{bmatrix}}_{\g(\x)} \u + \w,
% \end{align}
% where the drift vector, $\f:\mathbb{R}^{2n}\to\mathbb{R}^{2n}$, and actuation matrix, $\g:\mathbb{R}^{2n\times m}\to\mathbb{R}^{2n}$, are assumed to be twice continuously differentiable. This is subsumed by the standard assumption that the Lagrangian of the system is smooth. 

% \begin{definition}
% (Feedback Linearizeability) The system \eqref{eq:eom} with $k\in\N$, $k\le m$ time-varying outputs $\y:\mathcal{X}\times \R \to \cal{Y}\subseteq\R^k$ is said to be \textit{feedback linearizeable} of vector relative degree $\gamma\in\N^k$ with $\gamma_i \le 2n$ if there exists a feedback control law $\k:\cal{X}\times\V\times\R$ for an auxiliary control input $\v\in\V\subset\R^m $ such that:
% \begin{align*}
%     \dot \x = \f(\x) + \g(\x)\k(\x,\v,t) \implies \y_i^{(\gamma_i)} = \v_i~ \forall i=1,\dots,k.
% \end{align*}
% \end{definition}
% \begin{assumption}
% Assume that the nonlinear system \eqref{eq:eom} is square $(m=k)$, full state feedback linearizeable with time-varying outputs $\mb{y}:\cal{X}\times\mathbb{R}\to\cal{Y}$ of vector relative degree two $(m = n)$. In other words, the outputs have the structure of $\y(x,t) =\y_a(\q)- \y_d(t)$ for some twice differentiable desired trajectory $\y_d:\mathbb{R}\to\mathbb{R}^k$.
% \end{assumption}
% \noindent
% From the above assumption on feedback linearizeability, there exists a diffeomorphism $\mb{\Phi}:\mathcal{X} \to \cal{Y}$ and output coordinates $\bm{\eta} = \mb{\Phi}(\x)$ satisfying:
% \begin{align}
%     \bm{\eta} \triangleq \begin{bmatrix}\bm{\eta_1} \\ \bm{\eta_2}\end{bmatrix}  = \begin{bmatrix} \y_a(\q)-\y_d(t) \\ \mb{L}_{\f}\y_a(\x) - \dot \y_d(t) \end{bmatrix}.
% \end{align}
% Differentiating, we see:
% \begin{align}
%     \bm{\dot\eta} = \begin{bmatrix}\bm{\dot \eta_1} \\ \bm{\dot \eta_2}\end{bmatrix}  = \begin{bmatrix} \bm{\eta_2} \\ \mb{L}^2_{\f}\y_a(\x) + \mb{L}_\g\mb{L}_{\f}\y_a(\x)\u - \ddot \y_d(t) \end{bmatrix}.
% \end{align}
% Defining $\cal{F}(\x) = \mb{L}^2_{\f}\y_a(\x)$ and $\cal{G}(\x) = \mb{L}_\g\mb{L}_{\f}\y_a(\x)$, applying the following feedback controller $\k:\cal{X}\times\V\times\R\to\mathcal{U}$ results in:
% \begin{align}
% \label{eqn:FL_control}
%     \k= \mathcal{G}^{-1}(\x)(-\mathcal{F}(\x) + \y_d^{\vec \gamma}(t) + \v) \implies \dot \eta = \F\eta + \G\v
% \end{align}
% where the dependence on $(\x,\v,t)$ has been dropped for $\k$, and with $\F\in\R^{2k\times 2k}$, $\G\in\R^{2k\times m}$ defined as:
% % \begin{align*}
% %     \F &= 
% %     \begingroup\setlength\arraycolsep{0pt}\begin{bmatrix} \F_1 &&\mb{0}\\&\ddots&\\\mb{0}&&\F_k\end{bmatrix}\endgroup\F_i = \begin{bmatrix}0&1\\0&0\end{bmatrix}
% %     \G =
% %     \begingroup\setlength\arraycolsep{0pt}\begin{bmatrix} \G_1 &&\mb{0}\\&\ddots&\\\mb{0}&&\G_k\end{bmatrix}\endgroup\G_i &= \begin{bmatrix}0\\1\end{bmatrix}
% % \end{align*}
% \begin{align}
% \label{eq:fg}
%     \F =  \begin{bmatrix}0&1\\0&0\end{bmatrix} \otimes \mb{I}_k,\hspace{5mm}
%     \G = \begin{bmatrix}0\\1\end{bmatrix} \otimes \mb{I}_k
% \end{align}

% \begin{definition} (Input to State Stable Control Lyapunov Function)
% A continuously differentiable function $V:\mathcal{X}\to\mathbb{R}_{+}$ is An \textit{input to state stabilizing control Lyapunov function (ISS-CLF)} if there exist functions $\alpha_1,\alpha_2,\alpha_3,\rho\in\mathcal{K}_\infty$ satisfying:
% \begin{align*}
%     \alpha_1(\|\x\|) \le V(x) \le \alpha_2(\|\x\|) \\
%     \|\x\|\ge\rho(\|\w\|) \implies \inf_{\u\in\mathcal{U}}\dot V(\x,\u,\d) \le -\alpha_3 (\|\x\|)
% \end{align*}
% for all $\x\in\mathcal{X}$ and $\w\in\mathcal{W}$.
% \end{definition}
% \begin{lemma}
% [\red{Find citation}] Given a valid ISS-CLF, the set $\bar B_{\rho(\|\w\|_\infty)}$ is forward invariant.
% \end{lemma}
% Let $\E = \bar B_{\rho(\|\w\|_\infty)}$ represent the set which can be maintained forward invariant by the low-level controller under disturbances $\w$. An ISS-CLF controller can be constructed by solving the continuous algebraic Riccati equation:
% \begin{align*}
%     \F^T\P+\P\F-\P\G\G^T\P = -\mb{Q}
% \end{align*}
% for some $\P\succ 0$ given aby $\mb{Q} \succ0$ and constructing the Lyapunov function $V(\bm{\eta}) = \bm{\eta^TP\eta}$. A solution always exists because the pair $(\F,\G)$ from \eqref{eq:fg} is controllable, and this choise of Lyapunov function was shown to be input to state stable in \red{add reference}. Now, we can construct an ISS-CLF-QP as:
% \begin{equation}
%     \begin{aligned}
%     \k = \min_{\u\in\mathcal{U}} \quad & \|\mathcal{F}(\x) + \mathcal{G}(\x)\u - \y_d^{\vec \gamma}(t) - \v\|\\
% \textrm{s.t.} \quad & L_{\f}V(\x) + L_{\g}V(\x)\u\le -\gamma V + \frac{1}{\epsilon}\|L_{\g}V(\x)\|^2 \notag
% \end{aligned}
% \end{equation}
% Note that this could be replaced with any controller that allows for tracking a desired signal and enforces a robust invariant set $\mathcal{E}$.

% Finally, we remark on the brief background required for B\`ezier polynomials.
% [\red{cite cad book}]
% A B\`ezier polynomial $\Bez:[0,1]\to\mathbb{R}^k$ of degree $N$ is written, given $\b=[\b_0,\dots,\b_N]$ control points where $\b_i\in\R^k$, as $\Bez(\tau) = \b\Xi(\tau)$, where $\bm{\Xi}:\R\to\R^{N+1}$ is a vector-valued function defined as:
% \begin{align*}
%     \bm{\Xi_i}(\tau) = {n \choose i}(1-\tau)^{n-i}\tau^i.
% \end{align*}
% A powerful and well known property of B\`ezier polynomials is that their image is bounded by the convex hull of the control points, i.e. $\Bez(\tau) \in \text{conv}(\b)$ for all $\tau\in[0,1]$. By introducing the control points into the MPC program, we will be able to constraint tighten by the convex hull, and make conclusions about satisfaction of state and input constraints for the continuous time trajectory.



==> OLD/MPCOLD.tex <==
\section{Model Predictive Control}
Consider a linear, discrete time representation of \eqref{eq:eom} given by:
\begin{align*}
    \bar \x_{k+1} & \triangleq \A_k \bar \x_k + \B_k \bar \u_k + \C_k,
\end{align*}
and assume that the discretization is exact at the point $(\bar \x_k, \bar \u_k)$. This representation could have come from linearizing then discretizing, or discretizing then linearizing, as discussed in \cite{gros_linear_nodate}.
\subsection{Reconstruction of Continuous Time Trajectory}
Once we have the solution $\x^*=[\x_0^*,\dots \x_N^*], \u^*=[\u_0^*,\dots\u_{N-1}^*]$ to \eqref{eq:mpc}, we next need to construct a continuous time representation of the trajectory $\x(t)$ for $t\in[t_k,t_{k+1})$ for the low level controller to track. As such, the constructed trajectory $x(t)$ must be feasible with respect to the nonlinear dynamics \eqref{eq:eom}, and satisfy state and input constraints. Due to the convex hull property of B\`ezier polynomials, we must simply enforce that the control points satisfy the properties that we desire. The following proposition makes this precise:
\begin{proposition}
$\b\in\mathcal{X}\ominus \cal{E} \implies \B(\tau) \in\mathcal{X}\ominus\cal{E}$ for all $\tau\in[0,1]$.
\end{proposition}
\begin{proof}
Because $\mathcal{X}$ and $\mathcal{E}$ are convex, their minkowski difference is also convex. As such, $\b\in\mathcal{X}\ominus\mathcal{E}$ implies that $\text{conv}(\b)\in\mathcal{X}\ominus\mathcal{E}$. Because of the convex hull property of B\`ezier polynomials, we are done.
\end{proof}

Here, under a slight abuse of notation, we define $\b:\mathcal{X}\times\mathcal{X} \to \mathbb{R}^k$ to take in $x_k$ and $x_{k+1}$ as arguments, and output control points. \blue{If we simply do an admissible interpolation, then this is affine in its inputs. If it is more complicated (like solving an NLP), then it will be nonconvex.}

\begin{corollary}
Under the controller in \eqref{eqn:low_level}, the trajectories of the nonlinear and the linear system are identical.
\end{corollary}
\begin{proof}
Assume that $\x(t_k) = \x^*(t_k)$. Because the trajectory is feasible, the derivatives are identical. Therefore, by uniqueness of solutions, the trajectories must be the same for $t\in[t_k,t_{k+1})$. \correction{Add some limit stuff}. Therefore, $\x(t_{k+1}) = \x^*(t_{k+1})$. Under assumption \ref{ass:IC}, $\x(t_0) = \x^*(t_0)$, and following the same logic as above, $\x(t_1) = \x^*(t_1)$. The result follows from induction.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5 add sim figure here
\begin{figure*}
  \centering
  \begin{tabular}{@{}c@{}c}
    \includegraphics[width=.5\linewidth]{Figures/MPCWithLipschitzBound.png} 
    &\includegraphics[width=.5\linewidth]{Figures/tmp5.png} \\[\abovecaptionskip]
    \small (a) An image & \small (b) Another image
  \end{tabular}
  \vspace{\floatsep}
  \caption{This is a figure caption}\label{fig:myfig}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lemma}
$\x_k\in\mathcal{X}_c \ominus \E \iff \x_k$ satisfies $-\sqrt{\gamma} \frac{F^T P^{-1}F}{\sqrt{F^T P^{-1}F}} \le b-F^T\x_k$ for all $(F_i,b_i)$ defining $\mathcal{X}_c$.
\end{lemma}
\begin{proof}
\begin{align*}
    \x_k\in\mathcal{X}_c\ominus \E &\equiv F_i^T(\x_k+e)\le b_i \forall e\in\E \\
    &= \sup_{e\in\E} F_i^T(\x_k+e)\le b_i
\end{align*}
Noting that $\E=\{e:e^TPe \le \gamma\}$, we can solve the KKT conditions for the above program and achieve the desired result.
\end{proof}

\begin{align*}
    \b_{0,k} &= \q_k \\
    \b_{1,k} &= \frac{1}{3}(\dt\dot\q_k+3\q_k) \\
    \b_{2,k} &= \frac{1}{3}(3\q_{k+1}-\dt\dot\q_{k+1}) \\
    \b_{3,k} &= \q_{k+1}\\
    \Lambda &= \begin{bmatrix}&\mb{I}&&\\-\frac{3}{\dt}&\frac{3}{\dt}&0&0\\0&-\frac{3}{\dt}&\frac{3}{\dt}&0\\0&0&-\frac{3}{\dt}&\frac{3}{\dt}\end{bmatrix},\hspace{5mm}\Lambda\b^T\in\cal{X}_c\ominus\E
\end{align*}
\subsection{Input Bounds}
Next consider the input of the combined system for the time interval $t\in[t_k, t_{k+1})$:
\begin{align*}
    k_{NL}(\eta(t)) &= k_{NL}(Hx(t) - x^{\vec \gamma}_d(t)) \\
    &\le L_k\Big(\underbrace{\|x(t) - x^*(t)\|}_{\text{ISS-CLF}} + \underbrace{\|x^*(t) - x^*_k\|}_{\text{Desired Trajectory}}+\underbrace{\|x^*_k - \bar x_k\|}_{\text{Trust Region}}\Big) \\
    &\le L_k\Big(\rho(\|\w\|_\infty) + \sup_{\b_i}\|\b_i(x_k,x_{k+1}) - x^*_k\|+\|x^*_k - \bar x_k\|\Big)
\end{align*}
where the second line came from Lipschitz and adding and subtracting zero.

\begin{proposition}
There exists a continuous sequence of control inputs $u(t)$ such that $\x^*(t)$ is feasible for the nonlinear system \eqref{eq:eom}.
\end{proposition}
\begin{proof}
Consider an arbitrary interval $t\in [t_k,t_{k+1})$. Note that if $\eta_i = \dot \eta_i = \dots = \eta_i^{(\gamma_i-1)} = 0$ for all $i=1,\dots,k$, then we have that $\x(t) = \x^*(t)$. Therefore, by applying the feedback controller in \eqref{eqn:FL_control}, we know that $\x = \x^*(t)$. From this, we have:
\begin{align*}
    \dot \x^*(t) &= \dot \x(t) = \f(\x(t)) + \g(\x(t))\u^*(t) \\
    &= \f(\x^*(t)) + \g(\x^*(t))\u^*(t).
\end{align*}
Because the choice of $k$ was arbitrary, we are done. \red{wip}.
\end{proof}

The complete MPC program then becomes:
\begin{subequations}\label{eq:mpc}
\begin{alignat}{2}
    \min_{\substack{x_0,\dots,x_N\in\mathbb{R}^n \\ u_0,\dots,u_{N-1}\in\mathbb{R}^m}} \quad & \sum_{i=0}^{N-1} h(x_i,u_i) + V(x_N)\tag{\ref{eq:mpc}} \\
\textrm{s.t.} \quad & \x_{k+1|t} = \A_{k|t}\x_{k|t} + \B_{k|t}\u_{k|t} + \C_{k|t} \\
  & \x_{k|t} \in \mathcal{X}_c\ominus \E    \\
  & \u_{k|t} \in \mathcal{U}_c \ominus L_k(\E\oplus \mb{I}_T\oplus \mb{B})\\
%   & \|\x_{k|t}-\bar \x_{k|t}\|_2 \le L_T \\
  & \b(\x_{k|t},\x_{k+1|t}) \in \mathcal{X} \ominus \E \\
  & \x_{0|t} = \x(t) \oplus \mathcal{E}\\
  & \x_{N|t} \in \mathcal{X}_f
  \end{alignat}
\end{subequations}
where $h:\mathcal{X}\times\mathcal{U}\to\R$ is the stage cost and $V:\mathcal{X}\to\R$ is the terminal cost. Then, the policy at the low level is given by 
\begin{align*}
    u(t) = u^*_{t_k|t_k} + k_{NL}(x(t))~\forall t\in[t_k,t_{k+1})
\end{align*}

\begin{theorem}
The MPC program in \eqref{eq:mpc} satisfies state and input constraints for all time and for all disturbances.
\end{theorem}

==> OLD/ProblemFormulationOLD.tex <==
\section{Problem Formulation}

Consider an Euler-Lagrange system system of the form in \eqref{eq:robotEOM} with bounded additive disturbances $\w\in\W\subset\R^{2n}$ added as:
\begin{align*}
    \dot \x = \f(\x)+\g(\x)\u+\w.
\end{align*}


Next, let $\mathcal{U}_c\subseteq\mathcal{U}$ and $\mathcal{X}_c\subseteq\mathcal{X}$ represent input and output bounds, respectively, to be enforced over the flow of the system, and $\cal{X}_F\subset\cal{X}_c$ be a terminal constraint set.
\begin{assumption}
$\mathcal{X}_c$, $\mathcal{U}_c$, and $\mathcal{X}_F$ are polytopic.
\end{assumption}
\begin{assumption}
The sets $\mathcal{X},\mathcal{U},$ and $\mathcal{W}$ are compact and contain the origin in their interior.
\end{assumption}
% \begin{assumption}
% The sets $\mathcal{U}$ and $\mathcal{W}$ are compact and the set $\mathcal{X}$ is closed.
% \end{assumption}
\begin{assumption}
$\E$ is convex.
\end{assumption}
\begin{assumption}
$\cal{X}_F$ is a control invariant.
\end{assumption}
\noindent
The problem formulation is easily stated as:
\begin{problem}
Drive initial conditions $\y(\x_0,0)$ to $\mathcal{Y}_F$ for the system \eqref{eq:eom} while enforcing that $\y(\x(t),t)\in\mathcal{Y}_c$ and $\u(t)\in\mathcal{U}_c$ for all time $t\in\mathbb{R}_+$ and for all disturbances $\w\in\mathcal{W}$.
\end{problem}
In order to achieve the state objective, the desired trajectory $\y_d(t)$ and it's derivatives will need to be feasible with respect to the dynamics. We make this notion precise with the following definition.

% \begin{definition}[Constrained Dynamically Admissible Trajectory]
% Consider constants $T\in\R_{\ge0}$ and $N\in\mathbb{Z}_{> 0}$. A piecewise continuously differentiable function $\x_d:[0,T]\to\mathcal{X}$ on a finite subdivision $\{t_0, \ldots, t_N\}$ of the interval $[0,T]$ with $t_0 = 0$ and $t_N = T$ is said to be a \textit{feasible trajectory} for the system \eqref{eqn:openloop1} if there exists a right-continuous function $\u_d:[0,T]\to\mathcal{U}$ such that for all $i = 0,\ldots,N$ and $j = 0,\ldots, N-1$:
% \begin{align}
%     \label{eqn:feastraj}
%     \dot{\x}_d(t) &= \f(\x_d(t))+\g(\x_d(t))\u_d(t), ~ t\in(t_i,t_{i+1}), \\
%      \lim_{t\to t_j^+} \dot{\x}_d(t) &= \f(\x_d(t_j))+\g(\x_d(t_j))\u_d(t_j).
% \end{align}
% \end{definition}
\begin{remark}
The following analysis could be performed on any nonlinear control system which satisfies an integrator structure and has valid relative degree outputs. For the sake of simplicity of exposition, the discussion has be restricted to mechanical systems.
\end{remark}


